Resolutions of defining ideals of orbit closures for quivers of type $A_3$

We investigate the properties of coordinate rings of orbit closures for quivers of type $A_3$ by considering the desingularization given by Reineke. We construct explicit minimal free resolutions of the defining ideals of the orbit closures thus giving us a minimal set of generators for the defining ideal. The resolution allows us to read off some geometric properties of the orbit closure. In addition, we give a characterization for the orbit closure to be Gorenstein.

==> old.tex <==
In the case $b \neq 0, ~c \neq 0,~ d\neq 0$, if the condition on the right is satisfied, then applying Bott exchanges to 
\[\bigg( (0^b, (a+b+c)^{d+f}),~~(0^c, (a+b+c)^{d+e}),~((-2d-e-f)^{a+b+c},0^d) \bigg) \] gives the partitions -
\[\bigg( ((a+c)^{d+f}, (d+f)^b),~~((a+b)^{d+e}, (d+e)^c),~((-a-b-c)^{d},(-d-e-f)^{a+b+c}) \bigg) \]
If the orbit closure is Gorenstein, then $F_{top}$ is $1$-dimensional. This implies that the above partitions are rectangles, which means 
\[a+c=d+f, ~~a+b=d+e, ~~ a+b+c=d+e+f\]
When  $a \neq 0, ~e \neq 0,~ f\neq 0$, these conditions imply that $a=d, ~b=e$ and $c=f$.
Applying the same logic to each of the above cases, we get necessary conditions for the orbit closure to be Gorenstein. We list these conditions in the following table. \par \vskip0.5cm


%\advance\leftskip-3.5cm
\begin{center}
      \renewcommand{\arraystretch}{1.2}
\begin{longtable}{|c|cc|c|}
 \hline
Cases & \multicolumn{2}{|c|}{$\bigwedge^{top}\xi$ contributes if..}  & $\overline{O}_V$ is  \\
                                   &&& Gorenstein implies... \\ 
\hline 
\endfirsthead
       \hline 
          \multicolumn{1}{|c|}{Cases} &          
          \multicolumn{2}{|c|}{$\bigwedge^{top}\xi$ contributes if..} &
          \multicolumn{1}{|c|}{ $\overline{O}_V$ is Gorenstein implies..} \\
      \hline 
      \endhead
      \hline 
           \multicolumn{4}{|r|}{{Continued on next page}} \\ \hline
      \endfoot
      \endlastfoot
     
\multirow{3}{*}{$b=0, ~c=0, ~d=0$} & $a \neq 0, ~ e\neq 0, ~ f \neq0 $ &always & no condition     \\
                                                          & $a \neq 0, ~ e= 0, ~ f \neq0 $ &always & no condition     \\   
                                                          & $a \neq 0, ~ e\neq 0, ~ f = 0 $ &always & no condition     \\
 \hline
\multirow{4}{*}{$b\neq 0, ~c=0, ~d=0$}  &  $a \neq 0, ~ e\neq 0, ~ f \neq0 $ & $a \geq f$ & $a=f$     \\
                                                                &  $a \neq 0, ~ e= 0, ~ f \neq0 $ & $a \geq f$ & $a=f$     \\
                                                                &  $a \neq 0, ~ e\neq0, ~ f =0 $ & always & no condition     \\
                                                                &  $a = 0, ~ e\neq 0, ~ f =0 $ & always & no condition     \\
\hline

\multirow{4}{*}{$b=0, ~c\neq0, ~d=0$} &  $a \neq 0, ~ e\neq 0, ~ f \neq0 $ & $a \geq e$ & $a=e$     \\
                                                                &  $a \neq 0, ~ e\neq 0, ~ f =0 $ & $a \geq e$ & $a=e$     \\
                                                                &  $a \neq 0, ~ e=0, ~ f \neq0 $ & always & no condition     \\
                                                                &  $a = 0, ~ e = 0, ~ f \neq 0 $ & always & no condition     \\
\hline
\multirow{4}{*}{$b=0,~ c=0,~ d\neq0$ } &  $a \neq 0, ~ e\neq 0, ~ f \neq0 $ & $d+e+f \geq a$ & $d+e+f=a$     \\
                                                                &  $a \neq 0, ~ e\neq 0, ~ f =0 $ & $d+e \geq a$ & $d+e=a$     \\
                                                                &  $a \neq 0, ~ e=0, ~ f \neq0 $ & $d+f \geq a$ & $d+f=a$     \\
                                                                &  $a \neq 0, ~ e = 0, ~ f = 0 $ & $d \geq a$ & $d=a$   \\
\hline

\multirow{3}{*}{$b=0, ~c\neq0,~ d\neq0$}   & $a \neq 0, ~e \neq 0,~ f\neq 0$ & $a \geq d+e, ~ d+e+f \geq a+c$ & $a=d+e, ~c=f$ \\
                                                                   & $a = 0, ~e \neq 0,~ f\neq 0$ & $f \geq c$ & $c=f$     \\
                                                                   &  $a \neq 0, ~e = 0,~ f \neq 0$ & $a \geq d,~d+f \geq a+c$ & $a=d, ~c=f$    \\
                                                                   
\hline
\multirow{3}{*}{$b\neq 0, ~c=0, ~d\neq0$} & $a \neq 0, ~e \neq 0,~ f\neq 0$ & $a \geq d+f, ~ d+e+f \geq a+b$ & $a=d+f, ~b=e$ \\
                                                                   & $a = 0, ~e \neq 0,~ f\neq 0$ & $e \geq b$ & $b=e$     \\
                                                                   &  $a \neq 0, ~e \neq 0,~ f= 0$ & $a \geq d,~d+e \geq a+b$ & $a=d, ~b=e$    \\
                                                                   
\hline

\multirow{6}{*}{$b\neq 0,~ c\neq0, ~d=0$ }&  $a \neq 0, ~ e\neq 0, ~ f \neq0 $ & $a+b\geq e,~a+c \geq f$ & $a+b=e, ~a+c=f$  \\
                                                                   &  $a =0, ~ e\neq 0, ~ f \neq0 $ & $ b \geq e,~ c \geq f$ & $b=e,~c=f$     \\
                                                                   &  $a \neq 0, ~ e= 0, ~ f \neq0 $ & $a+c \geq f$ & $a+c=f$      \\
                                                                   &  $a \neq 0, ~ e\neq 0, ~ f =0 $ & $a+b\geq e$ & $a+b=e$      \\
                                                                   &  $a = 0, ~ e = 0, ~ f \neq0 $ & $c\geq f$ & $c=f$      \\
                                                                   &  $a = 0, ~ e\neq 0, ~ f =0 $ & $b\geq e$ & $b=e$      \\
\hline
$b\neq0,~c\neq0,~d\neq0$ &  $a \neq 0, ~e \neq 0,~ f\neq 0$ &  $a+c \geq d+f $, ~$a+b \geq d+e $,&  $a=d, ~b=e, ~c=f$   \\
             &&             ~$ d+e+f  \geq a+b+c$ &\\
\hline 

\caption{Cases} \label{table2}
\end{longtable}
\end{center}

\vskip1cm

Now we consider what happens if the conditions on the right are not satisfied in the cases listed in Proposition \ref{Prop4}. In this event, the top exterior power $\bigwedge^{top}\xi$ does not contribute any term to $F_{top}$. For each case, we obtain a description of the term that does contribute to $F_{top}$ (we denote the corresponding exterior power by $\bigwedge^{max}\xi$) and state the necessary condition for the orbit closure to be Gorenstein. \par

\noindent \textbf{Case 1:} $b\neq 0, ~c=0, ~d=0$ - in this case dim $\xi = (a+b)(e+f)$ and codim $\overline{O}_V = ae+af+be$. \par If $a \neq  
   0, ~ e \neq 0, ~f \neq 0$, the weight in $\bigwedge^{top}\xi$ is of the form
   \[ \big( 0^b,(a+b)^f ;~ (a+b)^e ;~(-e-f)^{a+b} \big) \] 
   If $a \geq f$, the above term gives the summand $S_{(a^f,f^b)}V_1 \otimes S_{(a+b)^e}V_2 \otimes S_{(e+f)^{a+b}}V^*_3$ of 
   $F_{top}$ (as noted in Proposition \ref{Prop4}). However, if $a \leq f$, the above term contributes nothing. In this case, it follows from 
   Remark \ref{} that $\bigwedge^{max}\xi$ has a weight of the form  \[ \big( 0^b,(a+b)^k,k^{f-k} ;~(a+b)^e 
   ; - \nu  \big) \] where $k < f$. By Lemma \ref{lemma3} this weight must satisfy the condition $D(\lambda,\mu) = ae+af+be$. Substitution   
   gives
   \begin{eqnarray} \nonumber
   k(a+b+f-k)+(a+b)e-bk&=&ae+af+be \\ \nonumber
   i.e. ~~k^2-k(a+f)+af&=&0   
   \end{eqnarray}  This implies $k=a$ (since $k<f$). So the weight for $\bigwedge^{max}\xi$ is  \[ \big(  
   0^b,(a+b)^a,a^{f-a};~ (a+b)^e ; ~(-a-e)^b,(-e-f)^a  \big) \]  Using this weight it is easy to derive the corresponding weights for remaining 
    cases in the following table  
      \vskip0.5cm
 
      \renewcommand{\arraystretch}{1.5}
      \begin{longtable}[c]{|p{0.08cm}p{0.08cm}p{0.08cm}|p{2cm}|p{6.1cm}|p{6.5cm}|}     
      \hline
      $a$ & $e$ & $f$ &Condition & Weight of $\bigwedge^{max}\xi$& Corresponding summand in $F_{top}$ \\
                                        
      \hline
      \endfirsthead
       \hline 
          \multicolumn{1}{|c}{$a$} &
          \multicolumn{1}{c}{$e$} &
          \multicolumn{1}{c|}{$f$} &
          \multicolumn{1}{|c|}{Condition} &
          \multicolumn{1}{|c|}{Weight of $\wedge^{max}\xi$ }&
          \multicolumn{1}{|c|}{Corresponding summand in  $F_{top}$}\\  
      \hline 
      \endhead
      \hline 
           \multicolumn{6}{|r|}{{Continued on next page}} \\ \hline
      \endfoot
      \endlastfoot

      $*$ & $*$ & $*$ & $a < f$&$\big(0^b, (a+b)^a, a^{f-a};~(a+b)^e;$ &  
      $S_{(a^{b+f})}V_1 \otimes S_{((a+b)^e)}V_2 $\\
      &&&&$(-a-e)^b,(-e-f)^{a} \big)$& $\otimes S_{((-e-a)^b,(-e-f)^{a})}V^*_3$ \\
      \hline
      $0$ & $*$ & $*$ & $a < f$ & $\big( 0^{b+f};~b^e;~-e^b  \big)$ &$S_{(b^e)}V_2 \otimes 
      S_{(-e^b)}V^*_3$ \\
      \hline
      $*$ & $0$ & $*$ & $a < f$ & $\big( 0^b, (a+b)^a,a^{f-a}; ~\phi ;~-a^b,-f^a  \big)$ &$S_{(a^{b+d+f})}V_1 
       \otimes S_{(-a^b,-f^a)}V^*_3$ \\
      \hline
      $*$ & $*$ & $0$ & \multicolumn{2}{|c|}{in this case $\wedge^{top}\xi$ contributes}&$S_{((a+b)^e)}V_2 \otimes 
      S_{(e^{a+b})}V^*_3$  \\
      \hline
      $0$ & $0$ & $*$ & \multicolumn{2}{|c|}{in this case codim $\overline{O}_V = 0$  }& $0$  \\
      \hline
      $0$ & $*$ & $0$ & \multicolumn{2}{|c|}{in this case $\wedge^{top}\xi$ contributes}&$S_{(b^e)}V_2 \otimes 
      S_{(e^b)}V^*_3$ 
      \\
      \hline
      $*$ & $0$ & $0$ & \multicolumn{3}{|c|}{in this case dim $\xi = 0$ } \\
      \hline
      \caption{$b\neq 0, ~c=0, ~d=0$}\label{table3-1}
      \end{longtable}


\vskip1cm
From Table \ref{table2} and Table \ref{table3-1} we can list the candidates for Gorenstein orbits in terms of conditions on multiplicities of indecomposables. We express these orbits in the shape of the AR quiver for easy reading:
\vskip1cm
   \begin{center}
    \includegraphics[scale=0.75, clip]{sec3/Gorenstein1.pdf}
   \end{center}
\vskip0.7cm
  
  
 
We repeat this procedure for the remaining 6 cases. We state only the sub-case $a \neq 0, e\neq 0, f \neq 0$ each time (the remaining subcases can be derived from the above) and the possible candidates for Gorenstein orbits. \par
\newpage
\noindent \textbf{Case 2:} $b=0, ~c\neq0, ~d=0$ 
  
      \renewcommand{\arraystretch}{1.5}
      \begin{table}[h]
      \begin{tabular}{|c|c|c|}     
      \hline
      Condition & Weight of $\wedge^{max}\xi$  & Summand in $F_{top}$ \\
                      
      \hline

      $a \leq f$& $\big( (a+b)^f;~~0^c,(a+c)^a,a^{e-a};~~(-a-f)^c,(-e-f)^{a} \big)$ &  $S_{((a+b)^f)}V_1 \otimes 
      S_{(a^{c+e})}V_2 $\\
       && $\otimes S_{((-a-f)^c,(-e-f)^{a})}V^*_3$ \\
      \hline
     
      \end{tabular} \caption{ $b=0, ~c\neq0, ~d=0$} \label{table3-2}
      \end{table}

   
   \begin{center}
    \includegraphics[scale=0.75, clip]{sec3/Gorenstein2.pdf}
   \end{center}
 \vskip2cm
  
   \noindent \textbf{Case 3:} $b=0,~ c=0,~ d\neq0$ \vskip0.5cm
      \renewcommand{\arraystretch}{1.5}
      \begin{table}[h]
      \begin{tabular}{|c|c|c|}     
      \hline
      Condition & Weight of $\wedge^{max}\xi$  & Summand in $F_{top}$ \\
                      
      \hline
     $d+e+f \leq a$ & $\big( a^{d+f};~ a^{e},(d+e+f)^d;$&  $S_{(a^{d+f})}V_1                
        \otimes S_{(a^{e},(d+e+f)^d)}V_2 $\\
      &$(-d-e-f)^{a-d-e-f},(-2d-e-f)^{d+e+f}, 0^d \big)$ & $\otimes S_{(-d-e-f^a)}V^*_3$ \\

      \hline
     
      \end{tabular} \caption{$b=0,~ c=0,~ d\neq0$} \label{table3-3}
      \end{table}
    
   \begin{center}
    \includegraphics[scale=0.75, clip]{sec3/Gorenstein3.pdf}
   \end{center}      

\newpage
\noindent \textbf{Case 4:} $b=0,~ c\neq 0,~ d\neq0$ \vskip0.5cm
  
      \renewcommand{\arraystretch}{1.5}
      \begin{table}[h]
      \begin{tabular}{|c|c|c|c|} 
    
      \hline
      Condition& cases & Weight of $\wedge^{max}\xi$  & Summand in $F_{top}$ \\
                      
      \hline
       $a \leq d+e,$ & $f \geq c$ & $\big(~(a+c)^{d+f};0^b, (a+c)^a,a^{d+e-a};$ & $S_{((a+c)^{d+f})}V_1 \otimes 
                                                                               S_{(a^{c+d+e})}V_2 $\\
       $ d+e+f \geq a+c$ &&$(-d-f-a)^{c},(-2d-e-f)^{a}, 0^d \big)$& $\otimes S_{((-a-c)^d,(-a-f)^c,(-d-e-f)^a)}V^*_3$ \\
      
      \hline
      &$f \leq c$ &$\big(~(a+c)^{d+f};0^c, (a+c)^a,a^{d+e-a};$ & $S_{((a+c)^{d+f})}V_1\otimes S_{(a^{c+d+e})}V_2 $\\
      &&$(-d-f-a)^{c},(-2d-e-f)^{a}, 0^d \big)$& $ \otimes S_{((-a-c)^d,(-a-f)^c,(-d-e-f)^a)}V^*_3$ \\
      
      \hline
      
      $a \geq d+e$& $f \geq c$ &$\big(~(a+c)^{d+f};0^c, (a+c)^e,(d+e+f)^d;$ & $S_{((a+c)^{d+f})}V_1  $\\
      $d+e+f \leq a+c$ &&$(-d-e-f)^{a+c-d-e-f},(-2d-e-f)^{d+e+f},0^d \big)$& $\otimes 
      S_{(a^e,(d+e+f-c)^d,(d+e)^c)}V_2$ \\
      &&&$\otimes S_{((-d-e-f)^{a+c+d})}V^*_3$\\
      \hline
      & $f \leq c$ &$\big(~(a+c)^{f},(d+e+f)^d;0^c, (a+c)^{d+e};$ & $S_{((a+c)^f,(d+e+f)^d)}V_1 $\\
      &&$(-d-e-f)^{a+c-d-e-f},(-2d-e-f)^{d+e+f}, 0^d \big)$& $\otimes  S_{(a^{d+e},(d+e)^c)}V_2$ \\
      &&&$\otimes S_{((-d-e-f)^{a+c+d})}V^*_3$\\
      \hline
       $a \leq d+e$& $f\leq c$ &$\big(~(a+c)^{f},(a+f)^d;0^c, (a+c)^a,(d+e-a)^d;$ & $S_{((a+c)^{f},(a+f)^d)}V_1 \otimes 
       S_{(a^{c+d+e})}V_2 $\\

      $d+e+f \leq a+c$ &&$(-a-f)^{c-f},(-d-f-a)^{f},(-2d-e-f)^{a},0^d \big)$&$\otimes(-a-f)^{c+d},(-d-e-f)^{a})}V^*_3$ \\
     
      \hline
      \end{tabular} \caption{$b=0,~ c\neq 0,~ d\neq0$} \label{table3-4}
      \end{table}

      
   \begin{center}
    \includegraphics[scale=0.75, clip]{sec3/Gorenstein4.pdf}
   \end{center} 
        
\newpage
\noindent \textbf{Case 5:} $b\neq0,~ c = 0,~ d\neq0$ \par
      \begin{center}
      \renewcommand{\arraystretch}{1.5}
      \begin{table}[h]
      \begin{tabular}{|c|c|c|c|}     
      \hline
      Condition& cases & Weight of $\wedge^{max}\xi$  & Summand in $F_{top}$ \\
                      
      \hline
      $a \leq d+f,$& $e \geq b$ & $\big(0^b, (a+b)^a,a^{d+f-a};~(a+b)^{d+e};$ & $S_{(a^{b+d+f})}V_1 \otimes   
       S_{((a+b)^{d+e})}V_2 $\\
       $ d+e+f \geq a+b$ &&$(-d-e-a)^{b},(-2d-e-f)^{a}, 0^d \big)$& $\otimes S_{((-a-b)^d,(-a-e)^b,(-d-e-f)^a)}V^*_3$ \\
      \hline

      & $e \leq b$ &$\big(0^b, (a+b)^a,a^{d+f-a};~(a+b)^{d+e};$ & $S_{(a^{b+d+f})}V_1 \otimes  
       S_{((a+b)^{d+e})}V_2 $\\
       &&$(-d-e-a)^{b},(-2d-e-f)^{a}, 0^d \big)$& $\otimes S_{((-a-b)^d,(-a-e)^b,(-d-e-f)^a)}V^*_3$ \\
       \hline
       
       $a \geq d+f$& $e \geq b$ &$\big(0^b, (a+b)^f,(d+e+f)^d;~(a+b)^{d+e};$ & $S_{(a^f,(d+e+f-b)^d,(d+f)^b)}V_1 $\\
       $d+e+f < a+b$ &&$(-d-e-f)^{a+b-d-e-f},(-2d-e-f)^{d+e+f},0^d \big)$& $\otimes S_{((a+b)^{d+e})}V_2$ \\
       &&&$\otimes S_{((-d-e-f)^{a+b+d})}V^*_3$\\
       \hline
       & $e \leq b$ &$\big(0^b, (a+b)^{d+f};~(a+b)^{e},(d+e+f)^d;$ & $S_{(a^{d+f},(d+f)^b)}V_1 $\\
       &&$(-d-e-f)^{a+b-d-e-f},(-2d-e-f)^{d+e+f}, 0^d \big)$& $\otimes S_{((a+b)^e,(d+e+f)^d)}V_2 $ \\
       &&&$\otimes  S_{((-d-e-f)^{a+b+d})}V^*_3$\\

       \hline
        $a \leq d+f$& $e \leq b$ &$\big(0^b, (a+b)^a,(d+f-a)^d;~(a+b)^{e},(a+e)^d;$ &  $S_{(a^{b+d+f})}V_1 \otimes 
        S_{((a+b)^{e}, (a+e)^d)}V_2 $\\
       $d+e+f \leq a+b$ &&$(-a-e)^{b-e},(-d-e-a)^{e},(-2d-e-f)^{a},0^d \big)$& $\otimes 
       S_{((-a-e)^{b+d},(-d-e-f)^{a})}V^*_3$ \\
     
      \hline
     
      \end{tabular} \caption{ $b\neq0,~ c = 0,~ d\neq0$} \label{table3-5}
      \end{table}
      \end{center}
      
   \begin{center}
    \includegraphics[scale=0.75, clip]{sec3/Gorenstein5.pdf}
   \end{center}    
     
\newpage
\noindent \textbf{Case 6:} $b\neq0,~ c \neq 0,~ d=0$ \par
      
      \renewcommand{\arraystretch}{1.5}
      \begin{table}[h]
      \begin{tabular}{|c|c|c|c|}     
      \hline
      Condition& cases & Weight of $\wedge^{max}\xi$  & Summand in $F_{top}$ \\
                      
      \hline
      $a+c \leq f$, && $0^b, (a+b+c)^{a+c},(a+c)^{f-a-c};$ & $S_{((a+c)^{b+f})}V_1 \otimes S_{((a+b)^{e},e^c)}V_2 $\\ 
       
      $a+b \geq e$ && $~0^c,(a+b+c)^{e};$ & $\otimes S_{(-a-c-e)^{b},(-e-f)^{a+c} )}V^*_3$\\
      &&$(-a-c-e)^{b},(-e-f)^{a+c} $ & \\
      \hline
      $a+c \geq f$,  && $0^b, (a+b+c)^f;$ & $S_{((a+c)^{f},f^b)}V_1 \otimes S_{((a+b)^{c+e})}V_2 $\\
      $ a+b \leq e$ &&$~0^c,(a+b+c)^{a+b},(a+b)^{e-a-b};$  & $\otimes S_{(-a-b-f)^{c},(-e-f)^{a+b} )}V^*_3$ \\
      && $(-a-b-f)^{c},(-e-f)^{a+b}$ &\\
      \hline
      $a+c \leq f,$ & $c \geq b$ & $ 0^b, (a+b+c)^{a+c},(a+c)^{f-a-c};$ &  
                                                 $S_{((a+c)^{b+f})}V_1 \otimes S_{((a+b)^{e},e^c)}V_2 $\\
      $ a+b \leq e$ &&$ 0^c,(a+b+c)^{a+b},(a+b)^{e-a-b};$& $\otimes 
      S_{((-2a-b-c)^{b},(-a-b-f)^{c-b},(-e-f)^{a+b} )}V^*_3$ \\
      &&$(-2a-b-c)^{b},(-a-b-f)^{c-b},(-e-f)^{a+b} $&\\
      \hline
      &$c \leq b$ & $ 0^b, (a+b+c)^{a+c},(a+c)^{f-a-c};$ & $S_{((a+c)^{b+f})}V_1 \otimes 
                                                                               S_{((a+b)^{e},e^c)}V_2 $\\
       & & $~0^c,(a+b+c)^{a+b},(a+b)^{e-a-b}; $& $\otimes 
      S_{((-2a-b-c)^{b},(-a-c-e)^{b-c},(-e-f)^{a+b} )}V^*_3$ \\ 
      & & $(-2a-b-c)^{b},(-a-c-e)^{b-c},(-e-f)^{a+b} $& \\ \hline
      \end{tabular} \caption{$b\neq0,~ c \neq 0,~ d=0$} \label{table3-6}
      \end{table}
      
   \begin{center}
    \includegraphics[scale=0.75, clip]{sec3/Gorenstein6.pdf}
   \end{center}      
 
\newpage      
\noindent \textbf{Case 7:} $b\neq0,~ c \neq 0,~ d \neq 0$ \par
      
      \renewcommand{\arraystretch}{1.5}
     
      \begin{longtable}{|c|c|c|c|}     
      \hline
      Condition& cases & Weight of $\wedge^{max}\xi$  & Summand in $F_{top}$ \\
      \hline
\endfirsthead
       \hline 
          \multicolumn{1}{|c|}{Condition} &
          \multicolumn{1}{|c|}{cases} &
          \multicolumn{1}{|c|}{Weight of $\wedge^{max}\xi$ }&
          \multicolumn{1}{|c|}{Summand in $F_{top}$}\\  
      \hline 
      \endhead
      \hline 
           \multicolumn{4}{|r|}{{Continued on next page}} \\ \hline
      \endfoot
      \endlastfoot 
      
                      
   
      $a+c \leq d+f$ & $e \geq b$& $0^b, (a+b+c)^{a+c},(a+c)^{d+f-a-c};$ & $S_{((a+c)^{b+d+f})}V_1 \otimes 
      S_{((a+b)^{d+e},(d+e)^c)}V_2 $\\ 
      $a+b \geq d+e$ && $~0^c,(a+b+c)^{d+e};$ & $\otimes S_{(-a-b-c)^d,(-a-c-e)^{b},(-d-e-f)^{a+c} )}V^*_3$\\
      $d+e+f \geq a+b+c$ &&$(-d-a-c-e)^{b},(-2d-e-f)^{a+c},0^d $ & \\
      \hline
      
      &$e \leq b$ & $0^b, (a+b+c)^{a+c},(a+c)^{d+f-a-c};$ & $S_{((a+c)^{b+d+f})}V_1 $\\
      &$a \geq d$&$~0^c,(a+b+c)^{e},(a+c+e)^{d};$  & $ \otimes 
      S_{((a+b)^{e},(a+e)^d,(d+e)^c)}V_2$ \\
      && $(-a-c-e)^{b-e},(-d-e-a-c)^{e},$ &$\otimes S_{(-a-c-e)^{b+d},(-d-e-f)^{a+c} )}V^*_3$\\
      &&$(-2d-e-f)^{a+c},0^d$&\\
      \hline
      
      &$e \leq b$ & $0^b, (a+b+c)^{a+c},(a+c)^{d+f-a-c};$ & $S_{((a+c)^{b+d+f})}V_1  $\\
      &$a \leq d$&$~0^c,(a+b+c)^{e},(a+c+e)^{a},(a+e)^{d-a};$  & $\otimes S_{((a+b)^{e},(a+e)^{c+d})}V_2$ \\
      && $(-a-c-e)^{b-e},(-d-e-a-c)^{e},$ & $\otimes  
      S_{(-a-c-e)^{b+d},(-a-e-f)^{c},(-d-e-f)^{a})}V^*_3$\\
      &&$(-a-d-e-f)^{c},(-2d-e-f)^{a},0^d$&\\
      \hline
      $a+c \geq d+f$  & $e \geq b$ & $0^b,(a+b+c)^{f},(d+e+f)^d;$ & $S_{(a+c)^{f},(d+e+f-b)^d,(d+f)^b}V_1$ \\
      $a+b \geq d+e$ & $f \leq c$ & $0^c,(a+b+c)^{d+e};$ & $\otimes S_{(a+b)^{d+e},(d+e)^c}V_2$ \\
      $d+e+f \leq a+b+c$ &  & $(-d-e-f)^{a+b+c-d-e-f},(-2d-e-f)^{d+e+f},0^d$ & $\otimes S_{(-d-e-f)^{a+b+c+d}}V^*_3$ \\
      \hline
      & $e \leq b$ & $0^b,(a+b+c)^{d+f};$ & $S_{(a+c)^{d+f},(d+f)^b}V_1$ \\
      & $f \geq c$ & $0^c,(a+b+c)^{e},(d+e+f)^d$ & $\otimes S_{(a+b)^{e},(d+e+f-c)^d,(d+e)^c}V_2$ \\
      & & $(-d-e-f)^{a+b+c-d-e-f},(-2d-e-f)^{d+e+f},0^d$ & $S_{(-d-e-f)^{a+b+c+d}}V^*_3$ \\
      \hline
      & $e \leq b$ & $0^b,(a+b+c)^f,(a+b+f)^d;$ & $S_{(a+c)^f,(a+f)^{b+d}}V_1$ \\
      & $f \leq c$ & $0^c,(a+b+c)^{e},(c+d+e)^{d}$ & $\otimes S_{(a+b)^{e},(d+e)^{c+d}}V_2$ \\
      & $a \geq d$& $(-d-e-f)^{a+b+c-d-e-f},(-2d-e-f)^{d+e+f},0^d$ & $S_{(-d-e-f)^{a+b+c+d}}V^*_3$  \\
      \hline
      & $e \leq b$ & $0^b,(a+b+c)^f,(a+b+f)^a,(a+f)^{d-a};$ & $S_{(a+c)^f,(a+f)^{b+d}}V_1$ \\
      & $f \leq c$ & $0^c,(a+b+c)^{e},(a+c+e)^{a},(a+e)^{d-a}$ & $\otimes S_{(a+b)^{e},(a+e)^{c+d}}V_2$ \\
      & $a \leq d$& $(-a-e-f)^{b+c-e-f},(-d-e-f-a)^{e+f},(-2d-e-f)^{a},0^d$ & $S_{(-a-e-f)^{b+c+d},(-d-e-f)^{a}}V^*_3$\\
      \hline

      $a+c \leq d+f$  & $a \geq d$ & $0^b,(a+b+c)^{a+c},(a+c)^{d+f-a-c};$ & $S_{(a+c)^{b+d+f}}V_1$ \\
      $a+b \geq d+e$ &  & $0^c,(a+b+c)^{e},(a+c+e)^{d};$ & $\otimes S_{(a+b)^{e},(a+e)^{d},(d+e)^{c}}V_2$ \\
      $d+e+f \leq a+b+c$ &  & $(-a-c-e)^{b-e},(-d-a-c-e)^{e},(-2d-e-f)^{a+c},0^d$ & $\otimes 
      S_{(-a-c-e)^{a+b+c},(-d-e-f)^{d}}V^*_3$ \\
      \hline
      & $a \leq d$ & $0^b,(a+b+c)^f,(a+b+f)^a,(a+f)^{d-a};$ & $S_{(a+c)^f,(a+f)^d,(d+f)^b}V_1$ \\
      & $f \leq c$ & $0^c,(a+b+c)^{e},(a+c+e)^a,(a+e)^{d-a}$ & $\otimes S_{(a+b)^e,(a+e)^{c+d}}V_2$ \\
      & & $(-a-e-f)^{b+c-e-f},(-d-e-f-a)^{e+f},(-2d-e-f)^{a},0^d$ & $S_{(-a-e-f)^{b+c+d},(-d-e-f)^{a}}V^*_3$ \\
      \hline
      & $a \leq d$ & $0^b,(a+b+c)^{a+c},(a+c)^{d+f-a-c};$ & $S_{(a+c)^{b+d+f}}V_1$ \\
      & $f \geq c$ & $0^c,(a+b+c)^{e},(a+c+e)^{a},(a+e)^{d-a}$ & $\otimes S_{(a+b)^{e},(a+e)^{c+d}}V_2$ \\
      & & $(-a-c-e)^{b-e},(-d-a-c-e)^{e},$ & $S_{(-a-c-e)^{b+d},(-a-e-f)^{c},(-d-e-f)^{a}}V^*_3$ \\
      & &$(-d-e-f-a)^{c},(-2d-e-f)^{a},0^d$  &\\
      \hline

      $a+c \geq d+f$  & $a \geq d$ & $0^b,(a+b+c)^{f},(a+b+f)^{d};$ & $S_{(a+c)^{f},(a+f)^d,(d+f)^b}V_1$ \\
      $a+b \leq d+e$ &  & $0^c,(a+b+c)^{a+b},(a+b)^{d+e-a-b};$ & $\otimes S_{(a+b)^{c+d+e}}V_2$ \\
      $d+e+f \leq a+b+c$ &  & $(-a-b-f)^{c-f},(-d-a-b-f)^{f},(-2d-e-f)^{a+b},0^d$ & $\otimes 
      S_{(-a-b-f)^{c+d},(-d-e-f)^{a+b}}V^*_3$ \\
      \hline
      & $a \leq d$ & $0^b,(a+b+c)^f,(a+b+f)^a,(a+f)^{d-a};$ & $S_{(a+c)^f,(a+f)^{b+d}}V_1$ \\
      & $e \leq b$ & $0^c,(a+b+c)^{e},(a+c+e)^a,(a+e)^{d-a}$ & $\otimes S_{(a+b)^e,(a+e)^{c+d}}V_2$ \\
      & & $(-a-e-f)^{b+c-e-f},(-d-e-f-a)^{e+f},(-2d-e-f)^{a},0^d$ & $S_{(-a-e-f)^{b+c+d},(-d-e-f)^{a}}V^*_3$ \\
      \hline
      & $a \leq d$ & $0^b,(a+b+c)^{f},(a+b+f)^a,(a+f)^{d-a};$  & $S_{(a+c)^{f},(a+f)^{b+d}}V_1$ \\
      & $e \geq b$ & $0^c,(a+b+c)^{a+b},(a+b)^{d+e-a-b}$ & $\otimes S_{(a+b)^{c+d+e}}V_2$ \\
      & & $(-a-b-f)^{c-f},(-d-a-b-f)^{f},$ & $S_{(-a-b-f)^{c+d},(-a-e-f)^{b},(-d-e-f)^{a}}V^*_3$ \\
      &&$(-d-e-f-a)^{b},(-2d-e-f)^{a},0^d$  &\\
      \hline

      $a+c \leq d+f$  & $a \geq d$ & $0^b,(a+b+c)^{a+c},(a+c)^{d+f-a-c};$ & $S_{(a+c)^{b+d+f}}V_1$ \\
      $a+b \leq d+e$ & $c \geq b$ & $0^c,(a+b+c)^{a+b},(a+b)^{d+e-a-b};$ & $\otimes S_{(a+b)^{c+d+e}}V_2$ \\
      $d+e+f \geq a+b+c$ &  & $(-2a-b-c)^{b},(-d-a-b-f)^{c-b},(-2d-e-f)^{a+b},0^d$ & $\otimes         
      S_{(-a-b-c)^{d},(-2a-b-c-d)^{b},(-a-b-f)^{c-b},(-d-e-f)^{a+c}}V^*_3$ \\
      \hline
      & $a \geq d$ & $0^b,(a+b+c)^{a+c},(a+c)^{d+f-a-c};$ & $S_{(a+c)^{b+d+f}}V_1$ \\
      & $c \leq b$ & $0^c,(a+b+c)^{a+b},(a+b)^{d+e-a-b};$ & $\otimes S_{(a+b)^{c+d+e}}V_2$ \\
      &  & $(-2a-b-c)^{c},(-d-a-c-e)^{b-c},(-2d-e-f)^{a+b},0^d$ & $\otimes 
      S_{(-a-b-c)^{d},(-2a-b-c-d)^{c},(-a-c-e)^{b-c},(-d-e-f)^{a+c}}V^*_3$ \\
      \hline
      & $a \leq d$ & $0^b,(a+b+c)^f,(a+b+f)^a,(a+f)^{d-a};$ & $S_{(a+c)^f,(a+f)^{b+d}}V_1$ \\
      & $e \leq b$ & $0^c,(a+b+c)^{e},(a+c+e)^a,(a+e)^{d-a}$ & $\otimes S_{(a+b)^e,(a+e)^{c+d}}V_2$ \\
      & & $(-a-e-f)^{b+c-e-f},(-d-e-f-a)^{e+f},(-2d-e-f)^{a},0^d$ & $S_{(-a-e-f)^{b+c+d},(-d-e-f)^{a}}V^*_3$ \\
      \hline
      & $a \leq d$ & $0^b,(a+b+c)^{f},(a+b+f)^a,(a+f)^{d-a};$  & $S_{(a+c)^{f},(a+f)^{b+d}}V_1$ \\
      & $e \geq b$ & $0^c,(a+b+c)^{a+b},(a+b)^{d+e-a-b}$ & $\otimes S_{(a+b)^{c+d+e}}V_2$ \\
      & & $(-a-b-f)^{c-f},(-d-a-b-f)^{f},$ & $S_{(-a-b-f)^{c+d},(-a-e-f)^{b},(-d-e-f)^{a}}V^*_3$ \\
      &&$(-d-e-f-a)^{b},(-2d-e-f)^{a},0^d$  &\\
      \hline

      \caption{$b\neq0,~ c \neq 0,~ d\neq 0$} \label{table3-7}
      \end{longtable} 
      
      
   \begin{center}
    \includegraphics[scale=0.75, clip]{sec3/Gorenstein7.pdf}
   \end{center}
     
\begin{center}
\begin{table}[h]
\caption{Candidates for Gorenstein orbits}  \label{table4}
\begin{tabular}{|c|c|c|c|c|c|}
\hline
$a$  & $b$  & $c$ &  $d$  &  $e$  &  $f$ \\
\hline
$*$  & $*$  & $0$ &  $0$  &  $*$  &  $a$ \\
$0$  & $*$  & $0$ &  $0$  &  $*$  &  $*$ \\
$*$  & $*$  & $0$ &  $0$  &  $*$  &  $0$ \\
%$0$  & $*$  & $0$ &  $0$  &  $*$  &  $0$ \\
\hline
$*$  & $0$  & $*$ &  $0$  &  $a$  &  $*$ \\
$0$  & $0$  & $*$ &  $0$  &  $*$  &  $*$ \\
$*$  & $0$  & $*$ &  $0$  &  $0$  &  $*$ \\
%$0$  & $0$  & $*$ &  $0$  &  $*$  &  $*$ \\
\hline
$d+e+f$  & $0$  & $0$ &  $*$  &  $*$  &  $*$ \\
$*$      & $0$  & $0$ &  $*$  &  $0$  &  $*$ \\
$*$      & $0$  & $0$ &  $*$  &  $*$  &  $0$ \\
\hline
$d+e$  & $0$  & $*$ &  $*$  &  $*$  &  $c$ \\
$d+e$  & $0$  & $*$ &  $*$  &  $*$  &  $0$ \\
$0$  & $0$  & $*$ &  $*$  &  $*$  &  $c$ \\
$*$  & $0$  & $*$ &  $*$  &  $0$  &  $c$ \\
$d$  & $0$  & $*$ &  $*$  &  $0$  &  $0$ \\
%$0$  & $0$  & $*$ &  $*$  &  $0$  &  $c$ \\
\hline
$d+f$  & $*$  & $0$ &  $*$  &  $b$  &  $*$ \\
$d+f$  & $*$  & $0$ &  $*$  &  $0$  &  $*$ \\
$0$  & $*$  & $0$ &  $*$  &  $b$  &  $*$ \\
$*$  & $*$  & $0$ &  $*$  &  $b$  &  $0$ \\
$d$  & $*$  & $0$ &  $*$  &  $0$  &  $0$ \\
%$0$  & $*$  & $0$ &  $*$  &  $b$  &  $0$ \\
\hline
$*$  & $*$  & $*$ &  $0$  &  $a+b$  &  $a+c$ \\
$*$  & $*$  & $*$ &  $0$  &  $b$  &  $c$ \\
$*$  & $*$  & $*$ &  $0$  &  $0$  &  $a+c$ \\
$*$  & $*$  & $*$ &  $0$  &  $a+b$  &  $0$ \\
\hline
$0$  & $*$  & $*$ &  $*$  &  $b$  &  $c$ \\
%$*$  & $*$  & $*$ &  $a$  &  $0$  &  $c$ \\
%$*$  & $*$  & $*$ &  $a$  &  $b$  &  $0$ \\
$*$  & $*$  & $*$ &  $a$  &  $b$  &  $c$ \\
%$0$  & $*$  & $*$ &  $*$  &  $b$  &  $0$ \\
%$0$  & $*$  & $*$ &  $*$  &  $0$  &  $c$ \\
\hline
\end{tabular}
\end{table}
\end{center}
     
\bc{corollary3} For non-equioriented quiver $A_3$, let $V$ be a representation for which all indecomposables occur as summands of $V$ with non-zero multiplicities. The orbit closure $\overline{O_V}$ is Gorenstein iff the Coxeter orbits ($\tau$-orbits of the Auslander-Reiten quiver) are constant. 
\ec
\bpr
Sufficiency follows from Proposition \ref{Prop6}. Necessity follows from Case $7$.
\qed 
\newpage



==> sec2.tex <==
\section{Preliminaries}
First, we recall some basic facts about representations of quivers.
Gabriel \cite{MR0332887} proved that the set of isomorphism classes of indecomposable representations of $Q$ is in bijective correspondence with the set of positive roots $R^+$ of the corresponding root systems. Under this correspondence, simple roots correspond to simple objects. Every representation of $Q$ can be written uniquely (upto permutation of factors) as a direct sum of indecomposable representations
  \[ V= \bigoplus_{\alpha \in R^+}m_{\alpha} X_{\alpha} \](where $m_{\alpha}=$ multiplicity of $X_{\alpha}$ in $V$). The indecomposable representations can be obtained as the vertices of the Auslander-Reiten quiver of $Q$. \par

Given a quiver $Q$, one can define an Euler form on the dimension vectors of $Q$ as follows -
\begin{definition} Let $x=(x_1,\cdots, x_n)$ and $y=(y_1,\cdots,y_n)$ be two elements of $\mathbb{N}^{Q_0}$ ($|Q_0|=n$).
The the \emph{Euler form} $\left\langle . , . \right\rangle$ is \[\left\langle x , y \right\rangle=\sum_{i \in Q_0}x_iy_i - \sum_{a \in Q_1} x_{ta} y_{ha}\]
\end{definition}
 
\brem{remarks}
    \begin{enumerate}
     \item The Euler form can also be expressed in terms of the Cartan matrix $C_Q$ of $Q$ as \[\left\langle x , y   
     \right\rangle =x^t (C_Q^{-1})^t y\]
     \item We have the following useful dimension formula in terms of the Euler form (refer \cite{MR2197389}) : if $V,W 
     \in Rep(Q, 
     \underline{d})$, then
     \[ \left\langle \hbox{dim}~V ,~\hbox{dim}~ W \right\rangle= \hbox{dim}_K \hbox{Hom}_{KQ}(V,W)-\hbox{dim}_K 
      \hbox{Ext}^1_{KQ}(V,W) 
     \]
    \end{enumerate}
\erem

%------------------------------------------------------------------
\subsection{Orbit closures} The group $\displaystyle{\prod_{x \in Q_0}}$GL$(d(x))$ acts on Rep$(Q, \underline{d})$ by- \[((g_x)_{x \in Q_0}, (V(a))_{a \in Q_1})\longmapsto (g_{ha}V(a) g_{ta}^{-1})_{a \in Q_1} . \] The orbits of this action are the isomorphism classes of representations of $Q$.

Let $V, W \in$ Rep$(Q, \underline{d})$. We say that $V \leq_{deg} W$ (i.e. $V$ is a degeneration of $W$) if the orbit of $W$ is contained in the closure of the orbit of $V$ (i.e.$O_{W} \subset \overline{O}_V$). This introduces a partial order on the orbits. There is also Riedtmann's rank criterion: $V \leq W$ if dim Hom$_Q(X,V) \leq $ dim Hom$_Q(X,W)$ for all indecomposables $X$ in $Rep(Q,\underline{d})$. The connection between these two partial orders is given by-

\bt{Bongartz' theorem}(Bongartz \cite{MR1402728}) If $A$ is a representation-directed, finite dimensional, associative $K$-algebra then the partial orders $\leq_{deg}$ and $\leq$ coincide.
\et

Since $Rep(Q,\underline{d})$ satisfies the hypotheses of this theorem, the orbit of $V \in$ $Rep(Q,\underline{d})$ is given by 
  \begin{equation}
    O_V= \{W \in Rep(Q, \underline{d}) |~ \hbox{dim Hom}_Q(X,V) = \hbox{ dim Hom}_Q(X,W) \} 
  \end{equation}
and the corresponding orbit closure is 
  \begin{equation}
    \overline{O}_V= \{W \in Rep(Q, \underline{d}) |~\hbox{dim Hom}_Q(X,V) \leq \hbox{ dim Hom}_Q(X,W) \}
  \end{equation}
where $X$ varies over all indecomposables in $Rep(Q,\underline{d})$.
%-----------------------------------------------------------------
\subsection{Desingularization}
In \cite{MR1985731}, Reineke describes an explicit method of constructing desingularizations of orbit closures of representations of $Q$. The desingularizations depend on certain directed partitions of the isomorphism classes of indecomposable objects-

\bd{Defn1} A partition $\I_*=(\I_1, \cdots , \I_s)$, where $R^+=\I_1 \cup \cdots \cup \I_s$, is called directed if:
   \begin{enumerate}
     \item $Ext^1_Q(X_{\alpha}, X_{\beta})=0$ for all $\alpha, \beta \in \I_t$ for $t=1,\cdots ,s$.
     \item $Hom_Q(X_{\beta}, X_{\alpha})=0= Ext^1_Q(X_{\alpha}, X_{\beta})$ for all $\alpha \in \I_t, \beta \in \I_u,          t < u$
   \end{enumerate} 
\ed 

These conditions can be expressed in terms of the Euler form as-
   \begin{enumerate}
     \item $\left\langle\alpha, \beta \right\rangle=0$ for $\alpha, \beta \in \I_t$ for $t= 1, \cdots, s$
     \item $\left\langle \alpha, \beta \right\rangle \hspace{0.1cm} \geq \hspace{0.1cm} 0 \hspace{0.1cm} \geq        
            \left\langle \beta, \alpha \right\rangle$ for $\alpha \in \I_t, \beta \in \I_u, t<u$
   \end{enumerate}
 
Let $Q$ be a Dynkin quiver and let $AR(Q)$ denote its corresponding Auslander-Reiten quiver. A partition of indecomposables exists because the category of finite-dimensional representations is directed; in particular, we can choose a sectional tilting module and let $\I_t$ be its Coxeter translates.  We fix a partition $\I_*$ of $AR(Q)$. Then the indecomposable representations $X_{\alpha}$ are the vertices of $AR(Q)$. For a representation $V= \oplus_{\alpha \in R^+}m_{\alpha} X_{\alpha}$, we define representations \[ V_{(t)}:=\oplus_{\alpha \in \I_t}m_{\alpha} X_{\alpha}, ~~~~ t=1,\cdots,s \] Then $V=V_{(1)}\oplus \cdots \oplus V_{(s)}$. Let $\underline{d}_t =$ dim $V_{(t)}$. We consider the incidence variety \[Z_{\I_*, V} \subset \prod_{x \in Q_0} Flag(d_s(x),d_{s-1}(x)+d_s(x), \cdots , d_1(x)+ \cdots +d_s(x), K^{d(x)} ) \times Rep_K(Q,\underline{d}) \] defined as \[ Z_{\I_*, V} = \{((R_s(x) \subset R_{s-1}(x) \subset \cdots \subset R_1(x) \subset K^{d(x)}), V) | \forall a \in Q_1, \forall t, V(a)(R_t(ta)) \subset R_t(ha) \}. \]
In this case we say that $Z$ is a $s$-step desingularization.
\bt{Thm 1}(Reineke \cite{MR1985731}) Let $Q$ be a Dynkin quiver, $\I_*$ a directed partition of $R^+$. Then the second projection \[ q:Z_{\I_*, V} \longrightarrow Rep_K(Q, \underline{d})\] makes $Z_{\I_*, V}$ a desingularization of the orbit closure $\overline{O}_V$. More precisely, the image of $q$ equals $\overline{O}_V$ and $q$ is a proper birational isomorphism of $Z_{\I_*, V}$ and $\overline{O}_V$.
\et 

In the next section, we will realize $Z_{\I_*, V}$ as the total space of a vector bundle over \newline $\displaystyle{\prod_{x \in Q_0} Flag(d_s(x),d_{s-1}(x)+d_s(x), \cdots , d_1(x)+ \cdots +d_s(x), K^{d(x)} )}$ and calculate its cohomology to find a resolution of $\overline{O}_V$.
%===============================================================================================================================================================================================================================================
\section{Geometry of orbit closures} 
We use the desingularization described above to extract useful information about orbit closures. The idea is to apply the geometric construction described in \cite{MR1988690} to calculate syzygies. We will construct a resolution $\textbf{F}_{ \bullet}$ of the coordinate ring of the orbit closure under consideration. Then using results from \cite{MR1988690} we can recover the normality of this orbit closure (we refer to \cite{MR1885816} for a different proof of the general case). In the case of $1$-step desingularization, the vector bundle $\xi$ defined below is semisimple and we get an algorithm for calculating the resolution. Also, using this resolution, we give an explicit description of the minimal set of generators for the defining ideal of the orbit closure . 
%-------------------------------------------------------------------------------------------------------------------
\subsection{The geometric setup} The varieties of type $Z_{\I_*, V}$ are the total spaces of homogeneous vector bundles on the product of flag varieties. We will use shorthand notation \[Z_{\underline{d}_*} \subset \prod_{x \in Q_0} Flag(\underline{d}_*{(x)}, K^{d(x)})\times Rep(Q, \underline{d}) \] to denote our incidence varieties.
%be a sequence of dimension vectors. We define \[ Z_{\underline{d}_1, \cdots ,\underline{d}_s} \subset \prod_{x \in Q_0} Flag(d_s(x),d_{s-1}(x)+d_s(x), \cdots , d_2(x)+ \cdots +d_s(x), K^{d(x)} ) \times Rep_K(Q,\underline{d}) \]

The space $Rep(Q,\underline{d})$ has the structure of an affine variety. Let $A$ be the coordinate ring of $Rep(Q,\underline{d})$.
%use language of vector bundles
Let $\r_t(x)$ denote the tautological subbundle and $\q_t(x)$ the tautological factor bundle on $Flag(\underline{d}_*{(x)}, K^{d(x)})$. We define the following vector bundles: \[ \xi(a) = \sum_{t=1}^s \r_t(ta)\otimes \q_t(ha)^* \subset  V(d(ta))\otimes V(d(ha))^* \] and \[\eta(a)= V(d(ta))\otimes V(d(ha))^*/ \xi(a)\]
We set \[\eta := \bigoplus_{a \in Q_1}\eta(a), ~~~ \xi:=\bigoplus_{a \in Q_1}\xi(a)\]
Then $Z=Z_{\underline{d}_*}$ is the total space of $\eta^*$. \newline

\noindent We have: 
    \begin{center}
    \includegraphics[scale=0.7, clip]{sec2/setting.pdf}
    \end{center}

We resolve the structure sheaf $\mathcal{O}_Z$ using vector bundle $\xi$ over $\displaystyle{\prod_{x \in Q_0} Flag(\underline{d}_*{(x)},K^{d(x)})}$; this is a Koszul complex of sheaves on $Rep(Q,\underline{d}) \times \prod_{x \in Q_0}Flag(\underline{d}_*{(x)},K^{d(x)})$ -
\[ 0 \longrightarrow \bigwedge^t(p^* \xi) \longrightarrow \cdots \longrightarrow \bigwedge^2(p^* \xi) \longrightarrow p^* \xi \stackrel{\delta}{\longrightarrow} \mathcal{O}_{ Rep(Q,\underline{d}) \times \prod_{x \in Q_0}Flag(\underline{d}_*{(x)},K^{d(x)})}\]

We apply the direct image functor $R^iq_*$ to this complex to get a free resolution $\textbf{F}_{\bullet}$ of $K[\overline{O}_V]$ in terms of cohomology bundles on $V$. By Bott's theorem for general linear groups (\cite{MR1988690}, Theorem 4....), the terms of this resolution are given by - \[ \textbf{F}_i = \bigoplus_{j \geq 0}H^j(\prod_{x \in Q_0}{Flag(d_*(x), V(d(x)), \bigwedge^{i+j}\xi)})\otimes A[-i-j] \]We identify $A$ with the symmetric algebra \[ \displaystyle \bigotimes_{a \in Q_1} Sym (V(ta) \otimes V(ha)^*)\]

\bt{Thm 2} \cite{MR1988690} The normalization of $\overline{O}_V$ has rational singularities if and only if $\textbf{F}_i = 0$ for $i < 0$. The orbit closure $\overline{O}_V$ is normal with rational singularities if and only if $\textbf{F}_i = 0$ for $i < 0$ and $\textbf{F}_0 = A$. 
\et

In the next section, we apply the above tool for calculations on the case of non-equioriented quiver of type $A_3$. We will consider a family of incidence varieties which is more general in the sense that we take arbitrary dimension vectors $\underline{d}_1, \cdots , \underline{d}_s$ in place of the dimension vectors described by the partition above; on the other hand we will restrict to $1$-step desingularizations. In this case, $\xi$ is semisimple and has the form \[\displaystyle{\xi = \bigoplus_{a \in Q_1} \r_t(ta)\otimes \q_t(ha)^*}\]
%explain

==> sec3.tex <==


%-------------------------------------------------------------------------------------------------------------------
\subsection{Minimal generators of the defining ideal}
Let $V \in Rep({Q, \underline{d}})$, $V=a(0K0)+b(0KK)+c(KK0)+d(KKK)+e(K00)+f(00K)$ as before. 

%    \begin{center}
 %   \includegraphics[scale=0.6, clip]{A3nequi2.pdf}
   % \end{center}
\noindent In terms of multiplicities of indecomposables $a,b,c,d,e,f$, we have \[\hbox{rank}~\phi = b+d,~ \hbox{rank}~\psi = c+d,~ \hbox{rank}~(\phi+\psi) = b+c+d\] Also, $r_1=b$, $r_2=c$ and $q_3=d$. Hence $N=ub+vc+wd$.

\bl{lemma1} The terms in $F_1$ come from $\bigwedge^{rank(\phi)+1} \xi$, $\bigwedge^{rank(\psi)+1} \xi$ and $\bigwedge^{rank(\phi+\psi)+1} \xi$.
\el
\bpr From proposition 4.1, we have that \[F_1 = \bigoplus_{t=1}^{dim \xi}\bigoplus_{|\lambda|+|\mu|=t}c_{\lambda',\mu'}^{\nu} (S_{[0^{q_1},\lambda]}V_1 \otimes S_{[0^{q_2},\mu]}V_2 \otimes S_{[0^{r_3},\nu]}V_3^* )\] where $S_{\nu}\subset S_{\lambda'} \otimes S_{\mu'} $ and $D(\lambda,\mu)=1$. 
By proposition \ref{Prop2}, we must have- 
   \begin{eqnarray}
   D(\lambda,\mu) &\geq& \left\langle (u, v, w),(u, v, w) \right\rangle \nonumber \\
   1 &\geq& \left\langle (u, v, w),(u, v, w) \right\rangle \nonumber  
   \end{eqnarray}
Since $\left\langle (u, v, w),(u, v, w) \right\rangle > 0$, we must have
\[\left\langle (u, v, w),(u, v, w) \right\rangle =1 \]
Thus the options for $(u,v,w)$ are $(1,0,0), (0,1,0),(0,0,1),(1,0,1),(0,1,1),(1,1,1)$. (Of these, the first 3 are of no interest to us since they).
This together with the fact that $|\lambda|+|\mu|- N =1$ implies that $|\lambda|+|\mu|$ equals one of-
   \begin{itemize}
   \item $b+d+1$- this occurs for $(u,v,w)=(1,0,1)$. In this case, $\mu=0$ and $\nu=\lambda'$. 
   \item $c+d+1$- this occurs for $(u,v,w)=(0,1,1)$. In this case, $\lambda=0$ and $\nu=\mu'$. 
   \item $b+c+d+1$- this occurs for $(u,v,w)=(1,1,1)$. In this case, both $\lambda$ and $\mu$ can be non-zero.
   \end{itemize}
Hence, in order to find terms occuring in $F_1$, it is enough to look at $\bigwedge^{rank( \phi)+1} \xi$, $\bigwedge^{rank(\psi)+1} \xi$ and $\bigwedge^{rank(\phi+\psi)+1} \xi$.\qed


\noindent Let us denote the terms contributed by $\bigwedge^{rank(\phi)+1} \xi$, $\bigwedge^{rank(\psi)+1} \xi$ and $\bigwedge^{rank(\phi+\psi)+1} \xi$ to $F_1$ by $F(1,0,1), F(0,1,1)$ and $F(1,1,1)$ respectively. Then lemma \ref{lemma1} says that \[F_1=F(1,0,1) \oplus F(0,1,1) \oplus F(1,1,1)\]

\noindent The next proposition gives an explicit description of these $F(u,v,w)$-
\bp{Prop3}  
   \begin{enumerate}
   \item $F(1,0,1)= \bigwedge^{rank(\phi)+1}V_1 \otimes \bigwedge^{rank(\phi)+1}V_3^*$
   \item $F(0,1,1)= \bigwedge^{rank(\psi)+1}V_2 \otimes \bigwedge^{rank(\psi)+1}V_3^*$
   \item $F(1,1,1)= \bigoplus c^{\nu}_{\lambda',\mu'}(\bigwedge^{b+k+1}V_1 \otimes \bigwedge^{c+l+1}V_2 \otimes 
   \bigwedge^{rank(\phi+\psi)+1}V_3^*),~\hbox{where}~ k+l=d-1 $
   \end{enumerate}
\ep 
\bpr %Recall that if we consider the weight $(0^t,\lambda)$, suppose we need move the first $u$ terms to $\lambda$ to the left to bring this weight to decreasing order using Bott's algorithm, then after $ut$ exchanges the weight is  $(\lambda_1-t,\lambda_2-t,\cdots,\lambda_t-t,u^t,\lambda_{u+1},\cdots)$; so $\lambda_i-t \geq u$ for $i=1,\cdots u$.
%In order to describe the terms appearing in $F(u,v,w)$, lets first make the following observations:
%  \begin{enumerate}
 % \item
 % \end{enumerate}
\noindent For ease of notation, lets denote $\hbox{rank}(\phi),~ \hbox{rank}(\psi)$ and $\hbox{rank}(\phi+\psi)$ by $p, q, r$ respectively. \newline
\noindent $\textbf{F(1,0,1)}$: dim $Q_1=b$ so we consider weight $(0^b,\lambda)$, with $|\lambda|=p+1=b+d+1$. (here dim $R_1=d+f$)\newline 
\noindent $u=1$ implies $\lambda$ is a hook i.e. $\lambda=(\lambda_1,1^k,0,\cdots)$.
So we consider the weights:
\[(0^b,\lambda)=(0^b,\underbrace{\lambda_1,1^k,0,\cdots}_{d+f}) ~~\hbox{and}~~ (0^d,\nu)=(0^d,\underbrace{\nu_1,1^l,0,\cdots}_{a+b+c})\]
satisfying $b+1+k=p+1=d+1+l$. These equations imply $k=d$, $l=b$ and $\lambda_1=b+1$, $\nu_1=d+1$. Now if either $f=0$ or $a=c=0$, then rank $\phi=b+d=$ dim $V_1$ (resp. dim $V_3$). In this case, there is no contribution to $F_1$ from $\bigwedge^{p+1}\xi$. In all other cases, $\bigwedge^{p+1}\xi$ contributes the term $\bigwedge^{p+1}V_1 \otimes \bigwedge^{p+1}V_3^*$ to $F_1$. By Cauchy's formula \cite{MR1988690}, this term is a direct summand of $\bigwedge^{p+1}(V_1 \otimes V_3^*)$. \vskip0.3cm

\noindent $\textbf{F(0,1,1)}$: this case is similar to the above, we are looking at weights: \[(0^c,\mu)=(0^c,\underbrace{c+1,1^k,0,\cdots}_{d+e}) ~~\hbox{and}~~ (0^d,\nu)=(0^d,\underbrace{d+1,1^l,0,\cdots}_{a+b+c})\] satisfying $c+1+k=q+1=d+1+l$ which imply $k=d$ and $l=c$.
If either $e=0$ or $a=b=0$, then rank $\psi=c+d=$ dim $V_2$ (resp. dim $V_3$). In this case, there is no contribution to $F_1$ from $\bigwedge^{q+1}\xi$. In all other cases, $\bigwedge^{q+1}\xi$ contributes the term $\bigwedge^{q+1}V_2 \otimes \bigwedge^{q+1}V_3^*$ to $F_1$. This term is a direct summand of $\bigwedge^{q+1}(V_2 \otimes V_3^*)$. \vskip0.3cm

\noindent $\textbf{F(1,1,1)}$: in this case, $\lambda$ and $\mu$ are hooks of the form: \[\lambda=(b+1,1^k,0\cdots) ~~~~ \mu=(c+1,1^l,0\cdots) \]
Since $\nu$ is such that $S_{\nu}\subset S_{\lambda'} \otimes S_{\mu'}$, $\nu$ is also a hook of the form \[(d+1,1^m,0,\cdots)~~~\hbox{where}~m=b+c~ \hbox{or}~ m=b+c \]
Since $|\lambda|+|\mu|=|\nu|=r+1=b+c+d+1$, we must have $k+l=d-1$ and $m=b+c$.
Thus we have weights:\[(0^b,\lambda)=(0^b,\underbrace{b+1,1^k,0,\cdots}_{d+f}),~~(0^c,\mu)=(0^c,\underbrace{c+1,1^l,0,\cdots}_{d+e}),~~(0^d,\nu)=(0^d,\underbrace{d+1,1^{b+c},0,\cdots}_{a+b+c})  \]
If $a=0$, then rank$(\phi+\psi)=b+c+d$ dim $V_3$, so in this case $\bigwedge^{r+1}\xi$ does not contribute to $F_1$.\newline
\noindent If $d=0$, then $r+1=b+c+1$; so either
   \begin{itemize}
   \item $(0^b,\lambda)=(0^b,b+1,0,0,\cdots)$ and $(0^c,\mu)=(0^c,c,0,0,\cdots)$ or 
   \item $(0^b,\lambda)=(0^b,b,0,0,\cdots)$ and $(0^c,\mu)=(0^c,c+1,0,0,\cdots)$
   \end{itemize}
In both cases, there is no contribution (by Bott's algorithm).\newline
\noindent In all other cases,  $\bigwedge^{r+1}\xi$ contributes the term $\bigwedge^{b+k+1}V_1 \otimes \bigwedge^{c+l+1}V_2 \otimes \bigwedge^{r+1}V_3^*$ (where $k+l=d-1$) with multiplicity $c^{\nu}_{\lambda',\mu'}$ to $F_1$. Again by Cauchy's formula, this term is a direct summand of $\bigwedge^{r+1}([V_1 \oplus V_2] \otimes V_3^*)$.\qed


\bc{corollary2} Let rank$(\phi)=p$, rank$(\psi)=q$, rank$(\phi+\psi)=r$. The minimal generators of the defining ideal are determinantal: $(p+1) \times (p+1)$ minors of $\phi$, the $(q+1) \times (q+1)$ minors of $\psi$ and the $(r+1) \times (r+1)$ minors of $\phi+\psi$, taken by choosing $b+k+1$ columns of $\phi$ and $c+l+1$ columns of $\psi$.
\ec
\bpr The defining ideal of the orbit closure $\overline{O}_V$ is generated by the image of the map $F_1 \stackrel{\delta}{\longrightarrow} A$. Since $F_1=F(1,0,1) \oplus F(0,1,1) \oplus F(1,1,1)$, the image of the differential map $\delta$ is generated by $(p+1)\times (p+1)$-minors of the matrix corresponding to the linear map $\phi$, $(q+1)\times (q+1)$-minors of the matrix corresponding to the linear map $\psi$ and $(r+1)\times (r+1)$-minors of the matrix corresponding to the linear map $\phi+\psi$. \qed


\be{example2} Continuing example \ref{example1}, we calculate $F_1$ and the minimal generators of the defining ideal-
\ee
%-------------------------------------------------------------------------------------------------------------------
\subsection{$F_{top}$ and classification of Gorenstein orbits}
%In this section, we investigate classes of orbit closures that are Gorenstein. For the case of non-equioriented A_3, we also give a description of the last (top) term occuring in the resolution. 
%By \cite{MR1988690}, an orbit closure is Gorenstein if and only if the top module occuring in its resolution is irreducible and 1-dimensional. \par

Lets consider a Dynkin quiver $Q$. The top exterior power of $\xi(a)$ is 
\begin{eqnarray}  S_{[0^{d_1(ta)}, d_1(ha)^{d_2(ta)}, \cdots, (d_1(ha)+\cdots+d_{s-1}(ha))^{d_s(ta)}]}(ta) \\ \nonumber \otimes S_{[(-d_2(ta)-\cdots-d_s(ta))^{d_1(ha)}, \cdots, -d_s(ta)^{d_{s-1}(ha)}, 0^{d_s(ha)}]}(ha)^*\end{eqnarray}
%\[ S_{[0^{d_1(ta)}, d_1(ha)^{d_2(ta)}, \cdots, (d_1(ha)+\cdots+d_{s-1}(ha))^{d_s(ta)}]}(ta) \otimes S_{[(-d_2(ta)-\cdots-d_s(ta))^{d_1(ha)}, \cdots, -d_s(ta)^{d_{s-1}(ha)}, 0^{d_s(ha)}]}(ha) \]
Thus the top exterior power of $\xi$ is given by 
   \begin{equation} \bigwedge^{top} \xi= \bigotimes_{x \in Q_0} S(x)(k_1(x)^{d_1(x)},\cdots,k_s(x)^{d_s(x)} )   
   \label{topterm}
   \end{equation}
where 
   \begin{equation} k_t(x)= \sum_{a \in Q_1; ta=x} \sum_{u<t} d_u(ha)-\sum_{a \in Q_1; ha=x} \sum_{u>t} d_u(ta)
   \end{equation} \par

First, we give sufficient conditions for the orbit closure $\overline{O}_V$ to be Gorenstein in case of any Dynkin quiver $Q$. 
By \cite{MR1988690}, we have that if for every $x \in Q_0$, the number 
   \begin{equation} k_t(x)-\sum_{u<t}d_u(x)+\sum_{u>t}d_u(x) \label{condition}
   \end{equation} 
is independent of $t$, $(t=1,2, \cdots, s)$, then the corresponding orbit closure is Gorenstein.
The following lemma shows that this condition means that the $\tau$-orbits in the Auslander-Reiten quiver are constant- 
\bl{lemma4} Let $\tau$ denote the Auslander-Reiten translate and suppose $\underline{d}(x)=(d_u(x))_{u=1,2,\cdots, s}$ are dimensions of the flag at vertex $x$ in the desingularization $Z$. Then
\[ \langle \underline{e}_x, \underline{d}_t(x) \rangle = -\langle \underline{d}_{t+1}(x), \underline{e}_x \rangle  \] 
for all $x \in Q_0$ and $t=1,2,\cdots, s-1$, where $\underline{e}_x$ is the dimension vector of the simple representation supported at $x$.
\el 
\bpr (\ref{condition}) translates to the equations- 
   \begin{equation} k_{t+1}(x)-k_t(x)=d_t(x)+d_{t+1}(x)
   \end{equation}
for $x \in Q_0$ and $t=1,2,\cdots, s-1$. This is equivalent to-   
   \begin{equation} \sum_{a \in Q_1;ta=x}d_t(ha)+\sum_{a \in Q_1; ha=x}d_{t+1}(ta)=d_{t+1}(x)+d_t(x)
   \end{equation}
for all $x \in Q_0$ and $t=1,2,\cdots, s-1$. These conditions can be expressed in terms of Euler form as follows-
   \begin{eqnarray} \nonumber
   \langle \underline{e}_x, \underline{d}_t \rangle &=& d_t(x)-\sum_{a \in Q_1;ta=x}d_t(ha) \\ \nonumber
   &=& \sum_{a \in Q_1;ha=x}d_{t+1}(ta)-d_{t+1}(x) \\ \nonumber
   &=& -\langle \underline{d}_{t+1}, \underline{e}_x \rangle
   \end{eqnarray} 
   Thus, 
   \begin{equation} \langle \underline{e}_x, \underline{d}_t \rangle = -\langle \underline{d}_{t+1}, \underline{e}_x
    \rangle \label{euler}
   \end{equation}
where $\underline{e}_x$ is the dimension vector of the simple representation supported at $x$.    \qed   


\bp{Prop6} Assume that for each $t=1,2, \cdots, s-1$ we have $\underline{d}_{t+1}=\tau^+ \underline{d}_t$. Then the complex $F_{\bullet}$ is self-dual. If the incidence variety comes from Reineke desingularization and the corresponding orbit closure is normal with rational singularities, then it is also Gorenstein. 
\ep

Next, we investigate necessary conditions for for the orbit closure $\overline{O}_V$ to be Gorenstein in case of non-equioriented $A_3$. 
Evidence suggests that the maximal contributing exterior power of $\xi$ contributes to the last term of the resolution $F_{top}$. In this section we investigate whether this is true in general. This leads to a description of $F_{top}$ and a classification of Gorenstein orbits.\\

\noindent \textbf{Notation}: We will denote the topmost exterior power of $\xi$ by $\bigwedge^{top} \xi$. In cases when $\bigwedge^{top} \xi$ does not contribute to $F_{top}$, we denote the maximal contributing exterior power by $\bigwedge^{max} \xi$. \\

\noindent For the case of non-equioriented $A_3$, we investigate the following questions:
\begin{enumerate}
\item In what cases does $\bigwedge^{top}\xi$ contribute? To which term $F_i$ does $\bigwedge^{top}\xi$ contribute?  
\item In cases not covered by $(1)$ what is the $\bigwedge^{max}\xi$ which contributes? Does it contribute to $F_{top}$? 
\end{enumerate}
In each case, we give a description of $F_{top}$. Recall that for our case of non-equioriented $A_3$, we have desingularization-
  \begin{center}
  \includegraphics[scale=0.5, clip]{sec3/desing.pdf}
  \end{center}
As before, let $V=a(0K0)+b(0KK)+c(KK0)+d(KKK)+e(K00)+f(00K)$ be a representation of $A_3$.   
Then \[d_1=(b, ~a+b+c,~ c) ;~~ d_2=(d+f, ~d,~ d+e)\]  
From (\ref{topterm}) the weights for $\bigwedge^{top}\xi$ are:
\[(0^b, (a+b+c)^{d+f}),~~(0^c, (a+b+c)^{d+e}),~((-2d-e-f)^{a+b+c},0^d) \]  
\bl{lemma3} For a weight $(0^b, \lambda;~ 0^c, \mu;-\nu, 0^d)$ of $\bigwedge^{|\lambda|+|\mu|}\xi$, $D(\lambda,\mu)=$ codim $\overline{O}_V$ implies that the partition (if any) arising from $(0^b, \lambda; ~0^c, \mu; -\nu, 0^d)$ corresponds to a summand of $F_{top}$.
\el
\bpr...
\qed \par
We show that a contribution from $\bigwedge^{top} \xi$, if any, always goes to $F_{top}$.
\bl{lemma4} If the weight of the $\bigwedge^{top}\xi$ gives a non-zero partition after Bott exchanges, then the corresponding representation is a summand of $F_{top}$.
%If $\bigwedge^{top} \xi$ contributes, it always contributes to $F_{top}$. 
\el
\bpr We apply Bott's algorithm to each weight to get:
 \[[0^b, (a+b+c)^{d+f}] = ((a+c)^{d+f}, (d+f)^b) ~\hbox{after}~  b(d+f) ~\hbox{Bott exchanges}\]
 \[[0^c, (a+b+c)^{d+e}] = ((a+b)^{d+e}, (d+e)^c) ~\hbox{after}~ c(d+e) ~\hbox{Bott exchanges}\]
 \[[(-2d-e-f)^{a+b+c},0^d] = ((-a-b-c)^d, (-d-e-f)^{a+b+c}) ~\hbox{after}~ d(a+b+c) ~\hbox{Bott exchanges}\]
 
   \begin{eqnarray} \nonumber
   D(\lambda, \mu)&=&[(d+f)(a+b+c)]+[(d+e)(a+b+c)]\\ \nonumber
   &&-[b(d+f)+c(d+e)+d(a+b+c)] \\ \nonumber
   &=&ad+ae+af+be+cf \\ \nonumber
   &=&\hbox{codim}~ \overline{O}_V 
   \end{eqnarray} \qed

Next, we investigate when $\bigwedge^{top}\xi$ contributes. Observe that a contribution will occur whenever the Bott exchanges give a non-increasing sequence for every term of
\[\bigg( (0^b, (a+b+c)^{d+f}),~~(0^c, (a+b+c)^{d+e}),~((-2d-e-f)^{a+b+c},0^d) \bigg) \]
Also, note that if any of $b,c$ or $d$ are zero, then there are no exchanges for the corresponding term in the weight. We base our cases on this observation.
\bp{Prop4} $\bigwedge^{top}\xi$ contributes to $F_{top}$ in the following cases when the corresponding conditions are satisfied:
\begin{table}[h]
\centering
      \renewcommand{\arraystretch}{1.3}
\begin{tabular}{|c|ccc|}
\hline
Cases & \multicolumn{3}{|c|}{Conditions}\\
\hline
$b=0, ~c=0, ~d=0$ &   no condition &&      \\
\hline
$b\neq 0, ~c=0, ~d=0$ &  $a+c \geq d+f$ &  &      \\
\hline
$b=0, ~c\neq0, ~d=0$ &  & $a+b \geq d+e$ &  \\
\hline
$b=0,~ c=0,~ d\neq0$ &  &  &$ d+e+f \geq a+b+c  $      \\
\hline
$b=0, ~c\neq0,~ d\neq0$ &  & $a+b \geq d+e$ ,&~ $d+e+f \geq a+b+c$  \\
\hline
$b\neq 0, ~c=0, ~d\neq0$ & $a+c \geq d+f$ ,& & $ d+e+f \geq a+b+c $       \\
\hline
$b\neq 0,~ c\neq0, ~d=0$ &$ a+c \geq d+f$, &~$a+b \geq d+e$ & \\
\hline
$b\neq0,~c\neq0,~d\neq0$ & $a+c \geq d+f $, & ~$a+b \geq d+e $, &~$ d+e+f \geq a+b+c$ \\
\hline
\end{tabular}
\caption{}
\label{table1}
\end{table}
\ep

In the case $b \neq 0, ~c \neq 0,~ d\neq 0$, if the condition on the right is satisfied, then applying Bott exchanges to 
\[\bigg( (0^b, (a+b+c)^{d+f}),~~(0^c, (a+b+c)^{d+e}),~((-2d-e-f)^{a+b+c},0^d) \bigg) \] gives the partitions -
\[\bigg( ((a+c)^{d+f}, (d+f)^b),~~((a+b)^{d+e}, (d+e)^c),~((-a-b-c)^{d},(-d-e-f)^{a+b+c}) \bigg) \]
If the orbit closure is Gorenstein, then $F_{top}$ is $1$-dimensional. This implies that the above partitions are rectangles, which means 
\[a+c=d+f, ~~a+b=d+e, ~~ a+b+c=d+e+f\]
When  $a \neq 0, ~e \neq 0,~ f\neq 0$, these conditions imply that $a=d, ~b=e$ and $c=f$.
Applying the same logic to each of the above cases, we get necessary conditions for the orbit closure to be Gorenstein. We list these conditions in the following table. \par \vskip0.5cm


%\advance\leftskip-3.5cm
\begin{center}
      \renewcommand{\arraystretch}{1.2}
\begin{longtable}{|c|cc|c|}
 \hline
Cases & \multicolumn{2}{|c|}{$\bigwedge^{top}\xi$ contributes if..}  & $\overline{O}_V$ is  \\
                                   &&& Gorenstein implies... \\ 
\hline 
\endfirsthead
       \hline 
          \multicolumn{1}{|c|}{Cases} &          
          \multicolumn{2}{|c|}{$\bigwedge^{top}\xi$ contributes if..} &
          \multicolumn{1}{|c|}{ $\overline{O}_V$ is Gorenstein implies..} \\
      \hline 
      \endhead
      \hline 
           \multicolumn{4}{|r|}{{Continued on next page}} \\ \hline
      \endfoot
      \endlastfoot
     
\multirow{3}{*}{$b=0, ~c=0, ~d=0$} & $a \neq 0, ~ e\neq 0, ~ f \neq0 $ &always & no condition     \\
                                                          & $a \neq 0, ~ e= 0, ~ f \neq0 $ &always & no condition     \\   
                                                          & $a \neq 0, ~ e\neq 0, ~ f = 0 $ &always & no condition     \\
 \hline
\multirow{4}{*}{$b\neq 0, ~c=0, ~d=0$}  &  $a \neq 0, ~ e\neq 0, ~ f \neq0 $ & $a \geq f$ & $a=f$     \\
                                                                &  $a \neq 0, ~ e= 0, ~ f \neq0 $ & $a \geq f$ & $a=f$     \\
                                                                &  $a \neq 0, ~ e\neq0, ~ f =0 $ & always & no condition     \\
                                                                &  $a = 0, ~ e\neq 0, ~ f =0 $ & always & no condition     \\
\hline

\multirow{4}{*}{$b=0, ~c\neq0, ~d=0$} &  $a \neq 0, ~ e\neq 0, ~ f \neq0 $ & $a \geq e$ & $a=e$     \\
                                                                &  $a \neq 0, ~ e\neq 0, ~ f =0 $ & $a \geq e$ & $a=e$     \\
                                                                &  $a \neq 0, ~ e=0, ~ f \neq0 $ & always & no condition     \\
                                                                &  $a = 0, ~ e = 0, ~ f \neq 0 $ & always & no condition     \\
\hline
\multirow{4}{*}{$b=0,~ c=0,~ d\neq0$ } &  $a \neq 0, ~ e\neq 0, ~ f \neq0 $ & $d+e+f \geq a$ & $d+e+f=a$     \\
                                                                &  $a \neq 0, ~ e\neq 0, ~ f =0 $ & $d+e \geq a$ & $d+e=a$     \\
                                                                &  $a \neq 0, ~ e=0, ~ f \neq0 $ & $d+f \geq a$ & $d+f=a$     \\
                                                                &  $a \neq 0, ~ e = 0, ~ f = 0 $ & $d \geq a$ & $d=a$   \\
\hline

\multirow{3}{*}{$b=0, ~c\neq0,~ d\neq0$}   & $a \neq 0, ~e \neq 0,~ f\neq 0$ & $a \geq d+e, ~ d+e+f \geq a+c$ & $a=d+e, ~c=f$ \\
                                                                   & $a = 0, ~e \neq 0,~ f\neq 0$ & $f \geq c$ & $c=f$     \\
                                                                   &  $a \neq 0, ~e = 0,~ f \neq 0$ & $a \geq d,~d+f \geq a+c$ & $a=d, ~c=f$    \\
                                                                   
\hline
\multirow{3}{*}{$b\neq 0, ~c=0, ~d\neq0$} & $a \neq 0, ~e \neq 0,~ f\neq 0$ & $a \geq d+f, ~ d+e+f \geq a+b$ & $a=d+f, ~b=e$ \\
                                                                   & $a = 0, ~e \neq 0,~ f\neq 0$ & $e \geq b$ & $b=e$     \\
                                                                   &  $a \neq 0, ~e \neq 0,~ f= 0$ & $a \geq d,~d+e \geq a+b$ & $a=d, ~b=e$    \\
                                                                   
\hline

\multirow{6}{*}{$b\neq 0,~ c\neq0, ~d=0$ }&  $a \neq 0, ~ e\neq 0, ~ f \neq0 $ & $a+b\geq e,~a+c \geq f$ & $a+b=e, ~a+c=f$  \\
                                                                   &  $a =0, ~ e\neq 0, ~ f \neq0 $ & $ b \geq e,~ c \geq f$ & $b=e,~c=f$     \\
                                                                   &  $a \neq 0, ~ e= 0, ~ f \neq0 $ & $a+c \geq f$ & $a+c=f$      \\
                                                                   &  $a \neq 0, ~ e\neq 0, ~ f =0 $ & $a+b\geq e$ & $a+b=e$      \\
                                                                   &  $a = 0, ~ e = 0, ~ f \neq0 $ & $c\geq f$ & $c=f$      \\
                                                                   &  $a = 0, ~ e\neq 0, ~ f =0 $ & $b\geq e$ & $b=e$      \\
\hline
$b\neq0,~c\neq0,~d\neq0$ &  $a \neq 0, ~e \neq 0,~ f\neq 0$ &  $a+c \geq d+f $, ~$a+b \geq d+e $,&  $a=d, ~b=e, ~c=f$   \\
             &&             ~$ d+e+f  \geq a+b+c$ &\\
\hline 

\caption{Cases} \label{table2}
\end{longtable}
\end{center}

\vskip1cm

Now we consider what happens if the conditions on the right are not satisfied in the cases listed in Proposition \ref{Prop4}. In this event, the top exterior power $\bigwedge^{top}\xi$ does not contribute any term to $F_{top}$. For each case, we obtain a description of the term that does contribute to $F_{top}$ (we denote the corresponding exterior power by $\bigwedge^{max}\xi$) and state the necessary condition for the orbit closure to be Gorenstein. \par

\noindent \textbf{Case 1:} $b\neq 0, ~c=0, ~d=0$ - in this case dim $\xi = (a+b)(e+f)$ and codim $\overline{O}_V = ae+af+be$. \par If $a \neq  
   0, ~ e \neq 0, ~f \neq 0$, the weight in $\bigwedge^{top}\xi$ is of the form
   \[ \big( 0^b,(a+b)^f ;~ (a+b)^e ;~(-e-f)^{a+b} \big) \] 
   If $a \geq f$, the above term gives the summand $S_{(a^f,f^b)}V_1 \otimes S_{(a+b)^e}V_2 \otimes S_{(e+f)^{a+b}}V^*_3$ of 
   $F_{top}$ (as noted in Proposition \ref{Prop4}). However, if $a \leq f$, the above term contributes nothing. In this case, it follows from 
   Remark \ref{} that $\bigwedge^{max}\xi$ has a weight of the form  \[ \big( 0^b,(a+b)^k,k^{f-k} ;~(a+b)^e 
   ; - \nu  \big) \] where $k < f$. By Lemma \ref{lemma3} this weight must satisfy the condition $D(\lambda,\mu) = ae+af+be$. Substitution   
   gives
   \begin{eqnarray} \nonumber
   k(a+b+f-k)+(a+b)e-bk&=&ae+af+be \\ \nonumber
   i.e. ~~k^2-k(a+f)+af&=&0   
   \end{eqnarray}  This implies $k=a$ (since $k<f$). So the weight for $\bigwedge^{max}\xi$ is  \[ \big(  
   0^b,(a+b)^a,a^{f-a};~ (a+b)^e ; ~(-a-e)^b,(-e-f)^a  \big) \]  Using this weight it is easy to derive the corresponding weights for remaining 
    cases in the following table  
      \vskip0.5cm
 
      \renewcommand{\arraystretch}{1.5}
      \begin{longtable}[c]{|p{0.08cm}p{0.08cm}p{0.08cm}|p{2cm}|p{6.1cm}|p{6.5cm}|}     
      \hline
      $a$ & $e$ & $f$ &Condition & Weight of $\bigwedge^{max}\xi$& Corresponding summand in $F_{top}$ \\
                                        
      \hline
      \endfirsthead
       \hline 
          \multicolumn{1}{|c}{$a$} &
          \multicolumn{1}{c}{$e$} &
          \multicolumn{1}{c|}{$f$} &
          \multicolumn{1}{|c|}{Condition} &
          \multicolumn{1}{|c|}{Weight of $\wedge^{max}\xi$ }&
          \multicolumn{1}{|c|}{Corresponding summand in  $F_{top}$}\\  
      \hline 
      \endhead
      \hline 
           \multicolumn{6}{|r|}{{Continued on next page}} \\ \hline
      \endfoot
      \endlastfoot

      $*$ & $*$ & $*$ & $a < f$&$\big(0^b, (a+b)^a, a^{f-a};~(a+b)^e;$ &  
      $S_{(a^{b+f})}V_1 \otimes S_{((a+b)^e)}V_2 $\\
      &&&&$(-a-e)^b,(-e-f)^{a} \big)$& $\otimes S_{((-e-a)^b,(-e-f)^{a})}V^*_3$ \\
      \hline
      $0$ & $*$ & $*$ & $a < f$ & $\big( 0^{b+f};~b^e;~-e^b  \big)$ &$S_{(b^e)}V_2 \otimes 
      S_{(-e^b)}V^*_3$ \\
      \hline
      $*$ & $0$ & $*$ & $a < f$ & $\big( 0^b, (a+b)^a,a^{f-a}; ~\phi ;~-a^b,-f^a  \big)$ &$S_{(a^{b+d+f})}V_1 
       \otimes S_{(-a^b,-f^a)}V^*_3$ \\
      \hline
      $*$ & $*$ & $0$ & \multicolumn{2}{|c|}{in this case $\wedge^{top}\xi$ contributes}&$S_{((a+b)^e)}V_2 \otimes 
      S_{(e^{a+b})}V^*_3$  \\
      \hline
      $0$ & $0$ & $*$ & \multicolumn{2}{|c|}{in this case codim $\overline{O}_V = 0$  }& $0$  \\
      \hline
      $0$ & $*$ & $0$ & \multicolumn{2}{|c|}{in this case $\wedge^{top}\xi$ contributes}&$S_{(b^e)}V_2 \otimes 
      S_{(e^b)}V^*_3$ 
      \\
      \hline
      $*$ & $0$ & $0$ & \multicolumn{3}{|c|}{in this case dim $\xi = 0$ } \\
      \hline
      \caption{$b\neq 0, ~c=0, ~d=0$}\label{table3-1}
      \end{longtable}


\vskip1cm
From Table \ref{table2} and Table \ref{table3-1} we can list the candidates for Gorenstein orbits in terms of conditions on multiplicities of indecomposables. We express these orbits in the shape of the AR quiver for easy reading:
\vskip1cm
   \begin{center}
    \includegraphics[scale=0.75, clip]{sec3/Gorenstein1.pdf}
   \end{center}
\vskip0.7cm
  
  
 
We repeat this procedure for the remaining 6 cases. We state only the sub-case $a \neq 0, e\neq 0, f \neq 0$ each time (the remaining subcases can be derived from the above) and the possible candidates for Gorenstein orbits. \par
\newpage
\noindent \textbf{Case 2:} $b=0, ~c\neq0, ~d=0$ 
  
      \renewcommand{\arraystretch}{1.5}
      \begin{table}[h]
      \begin{tabular}{|c|c|c|}     
      \hline
      Condition & Weight of $\wedge^{max}\xi$  & Summand in $F_{top}$ \\
                      
      \hline

      $a \leq f$& $\big( (a+b)^f;~~0^c,(a+c)^a,a^{e-a};~~(-a-f)^c,(-e-f)^{a} \big)$ &  $S_{((a+b)^f)}V_1 \otimes 
      S_{(a^{c+e})}V_2 $\\
       && $\otimes S_{((-a-f)^c,(-e-f)^{a})}V^*_3$ \\
      \hline
     
      \end{tabular} \caption{ $b=0, ~c\neq0, ~d=0$} \label{table3-2}
      \end{table}

   
   \begin{center}
    \includegraphics[scale=0.75, clip]{sec3/Gorenstein2.pdf}
   \end{center}
 \vskip2cm
  
   \noindent \textbf{Case 3:} $b=0,~ c=0,~ d\neq0$ \vskip0.5cm
      \renewcommand{\arraystretch}{1.5}
      \begin{table}[h]
      \begin{tabular}{|c|c|c|}     
      \hline
      Condition & Weight of $\wedge^{max}\xi$  & Summand in $F_{top}$ \\
                      
      \hline
     $d+e+f \leq a$ & $\big( a^{d+f};~ a^{e},(d+e+f)^d;$&  $S_{(a^{d+f})}V_1                
        \otimes S_{(a^{e},(d+e+f)^d)}V_2 $\\
      &$(-d-e-f)^{a-d-e-f},(-2d-e-f)^{d+e+f}, 0^d \big)$ & $\otimes S_{(-d-e-f^a)}V^*_3$ \\

      \hline
     
      \end{tabular} \caption{$b=0,~ c=0,~ d\neq0$} \label{table3-3}
      \end{table}
    
   \begin{center}
    \includegraphics[scale=0.75, clip]{sec3/Gorenstein3.pdf}
   \end{center}      

\newpage
\noindent \textbf{Case 4:} $b=0,~ c\neq 0,~ d\neq0$ \vskip0.5cm
  
      \renewcommand{\arraystretch}{1.5}
      \begin{table}[h]
      \begin{tabular}{|c|c|c|c|} 
    
      \hline
      Condition& cases & Weight of $\wedge^{max}\xi$  & Summand in $F_{top}$ \\
                      
      \hline
       $a \leq d+e,$ & $f \geq c$ & $\big(~(a+c)^{d+f};0^b, (a+c)^a,a^{d+e-a};$ & $S_{((a+c)^{d+f})}V_1 \otimes 
                                                                               S_{(a^{c+d+e})}V_2 $\\
       $ d+e+f \geq a+c$ &&$(-d-f-a)^{c},(-2d-e-f)^{a}, 0^d \big)$& $\otimes S_{((-a-c)^d,(-a-f)^c,(-d-e-f)^a)}V^*_3$ \\
      
      \hline
      &$f \leq c$ &$\big(~(a+c)^{d+f};0^c, (a+c)^a,a^{d+e-a};$ & $S_{((a+c)^{d+f})}V_1\otimes S_{(a^{c+d+e})}V_2 $\\
      &&$(-d-f-a)^{c},(-2d-e-f)^{a}, 0^d \big)$& $ \otimes S_{((-a-c)^d,(-a-f)^c,(-d-e-f)^a)}V^*_3$ \\
      
      \hline
      
      $a \geq d+e$& $f \geq c$ &$\big(~(a+c)^{d+f};0^c, (a+c)^e,(d+e+f)^d;$ & $S_{((a+c)^{d+f})}V_1  $\\
      $d+e+f \leq a+c$ &&$(-d-e-f)^{a+c-d-e-f},(-2d-e-f)^{d+e+f},0^d \big)$& $\otimes 
      S_{(a^e,(d+e+f-c)^d,(d+e)^c)}V_2$ \\
      &&&$\otimes S_{((-d-e-f)^{a+c+d})}V^*_3$\\
      \hline
      & $f \leq c$ &$\big(~(a+c)^{f},(d+e+f)^d;0^c, (a+c)^{d+e};$ & $S_{((a+c)^f,(d+e+f)^d)}V_1 $\\
      &&$(-d-e-f)^{a+c-d-e-f},(-2d-e-f)^{d+e+f}, 0^d \big)$& $\otimes  S_{(a^{d+e},(d+e)^c)}V_2$ \\
      &&&$\otimes S_{((-d-e-f)^{a+c+d})}V^*_3$\\
      \hline
       $a \leq d+e$& $f\leq c$ &$\big(~(a+c)^{f},(a+f)^d;0^c, (a+c)^a,(d+e-a)^d;$ & $S_{((a+c)^{f},(a+f)^d)}V_1 \otimes 
       S_{(a^{c+d+e})}V_2 $\\

      $d+e+f \leq a+c$ &&$(-a-f)^{c-f},(-d-f-a)^{f},(-2d-e-f)^{a},0^d \big)$&$\otimes(-a-f)^{c+d},(-d-e-f)^{a})}V^*_3$ \\
     
      \hline
      \end{tabular} \caption{$b=0,~ c\neq 0,~ d\neq0$} \label{table3-4}
      \end{table}

      
   \begin{center}
    \includegraphics[scale=0.75, clip]{sec3/Gorenstein4.pdf}
   \end{center} 
        
\newpage
\noindent \textbf{Case 5:} $b\neq0,~ c = 0,~ d\neq0$ \par
      \begin{center}
      \renewcommand{\arraystretch}{1.5}
      \begin{table}[h]
      \begin{tabular}{|c|c|c|c|}     
      \hline
      Condition& cases & Weight of $\wedge^{max}\xi$  & Summand in $F_{top}$ \\
                      
      \hline
      $a \leq d+f,$& $e \geq b$ & $\big(0^b, (a+b)^a,a^{d+f-a};~(a+b)^{d+e};$ & $S_{(a^{b+d+f})}V_1 \otimes   
       S_{((a+b)^{d+e})}V_2 $\\
       $ d+e+f \geq a+b$ &&$(-d-e-a)^{b},(-2d-e-f)^{a}, 0^d \big)$& $\otimes S_{((-a-b)^d,(-a-e)^b,(-d-e-f)^a)}V^*_3$ \\
      \hline

      & $e \leq b$ &$\big(0^b, (a+b)^a,a^{d+f-a};~(a+b)^{d+e};$ & $S_{(a^{b+d+f})}V_1 \otimes  
       S_{((a+b)^{d+e})}V_2 $\\
       &&$(-d-e-a)^{b},(-2d-e-f)^{a}, 0^d \big)$& $\otimes S_{((-a-b)^d,(-a-e)^b,(-d-e-f)^a)}V^*_3$ \\
       \hline
       
       $a \geq d+f$& $e \geq b$ &$\big(0^b, (a+b)^f,(d+e+f)^d;~(a+b)^{d+e};$ & $S_{(a^f,(d+e+f-b)^d,(d+f)^b)}V_1 $\\
       $d+e+f < a+b$ &&$(-d-e-f)^{a+b-d-e-f},(-2d-e-f)^{d+e+f},0^d \big)$& $\otimes S_{((a+b)^{d+e})}V_2$ \\
       &&&$\otimes S_{((-d-e-f)^{a+b+d})}V^*_3$\\
       \hline
       & $e \leq b$ &$\big(0^b, (a+b)^{d+f};~(a+b)^{e},(d+e+f)^d;$ & $S_{(a^{d+f},(d+f)^b)}V_1 $\\
       &&$(-d-e-f)^{a+b-d-e-f},(-2d-e-f)^{d+e+f}, 0^d \big)$& $\otimes S_{((a+b)^e,(d+e+f)^d)}V_2 $ \\
       &&&$\otimes  S_{((-d-e-f)^{a+b+d})}V^*_3$\\

       \hline
        $a \leq d+f$& $e \leq b$ &$\big(0^b, (a+b)^a,(d+f-a)^d;~(a+b)^{e},(a+e)^d;$ &  $S_{(a^{b+d+f})}V_1 \otimes 
        S_{((a+b)^{e}, (a+e)^d)}V_2 $\\
       $d+e+f \leq a+b$ &&$(-a-e)^{b-e},(-d-e-a)^{e},(-2d-e-f)^{a},0^d \big)$& $\otimes 
       S_{((-a-e)^{b+d},(-d-e-f)^{a})}V^*_3$ \\
     
      \hline
     
      \end{tabular} \caption{ $b\neq0,~ c = 0,~ d\neq0$} \label{table3-5}
      \end{table}
      \end{center}
      
   \begin{center}
    \includegraphics[scale=0.75, clip]{sec3/Gorenstein5.pdf}
   \end{center}    
     
\newpage
\noindent \textbf{Case 6:} $b\neq0,~ c \neq 0,~ d=0$ \par
      
      \renewcommand{\arraystretch}{1.5}
      \begin{table}[h]
      \begin{tabular}{|c|c|c|c|}     
      \hline
      Condition& cases & Weight of $\wedge^{max}\xi$  & Summand in $F_{top}$ \\
                      
      \hline
      $a+c \leq f$, && $0^b, (a+b+c)^{a+c},(a+c)^{f-a-c};$ & $S_{((a+c)^{b+f})}V_1 \otimes S_{((a+b)^{e},e^c)}V_2 $\\ 
       
      $a+b \geq e$ && $~0^c,(a+b+c)^{e};$ & $\otimes S_{(-a-c-e)^{b},(-e-f)^{a+c} )}V^*_3$\\
      &&$(-a-c-e)^{b},(-e-f)^{a+c} $ & \\
      \hline
      $a+c \geq f$,  && $0^b, (a+b+c)^f;$ & $S_{((a+c)^{f},f^b)}V_1 \otimes S_{((a+b)^{c+e})}V_2 $\\
      $ a+b \leq e$ &&$~0^c,(a+b+c)^{a+b},(a+b)^{e-a-b};$  & $\otimes S_{(-a-b-f)^{c},(-e-f)^{a+b} )}V^*_3$ \\
      && $(-a-b-f)^{c},(-e-f)^{a+b}$ &\\
      \hline
      $a+c \leq f,$ & $c \geq b$ & $ 0^b, (a+b+c)^{a+c},(a+c)^{f-a-c};$ &  
                                                 $S_{((a+c)^{b+f})}V_1 \otimes S_{((a+b)^{e},e^c)}V_2 $\\
      $ a+b \leq e$ &&$ 0^c,(a+b+c)^{a+b},(a+b)^{e-a-b};$& $\otimes 
      S_{((-2a-b-c)^{b},(-a-b-f)^{c-b},(-e-f)^{a+b} )}V^*_3$ \\
      &&$(-2a-b-c)^{b},(-a-b-f)^{c-b},(-e-f)^{a+b} $&\\
      \hline
      &$c \leq b$ & $ 0^b, (a+b+c)^{a+c},(a+c)^{f-a-c};$ & $S_{((a+c)^{b+f})}V_1 \otimes 
                                                                               S_{((a+b)^{e},e^c)}V_2 $\\
       & & $~0^c,(a+b+c)^{a+b},(a+b)^{e-a-b}; $& $\otimes 
      S_{((-2a-b-c)^{b},(-a-c-e)^{b-c},(-e-f)^{a+b} )}V^*_3$ \\ 
      & & $(-2a-b-c)^{b},(-a-c-e)^{b-c},(-e-f)^{a+b} $& \\ \hline
      \end{tabular} \caption{$b\neq0,~ c \neq 0,~ d=0$} \label{table3-6}
      \end{table}
      
   \begin{center}
    \includegraphics[scale=0.75, clip]{sec3/Gorenstein6.pdf}
   \end{center}      
 
\newpage      
\noindent \textbf{Case 7:} $b\neq0,~ c \neq 0,~ d \neq 0$ \par
      
      \renewcommand{\arraystretch}{1.5}
     
      \begin{longtable}{|c|c|c|c|}     
      \hline
      Condition& cases & Weight of $\wedge^{max}\xi$  & Summand in $F_{top}$ \\
      \hline
\endfirsthead
       \hline 
          \multicolumn{1}{|c|}{Condition} &
          \multicolumn{1}{|c|}{cases} &
          \multicolumn{1}{|c|}{Weight of $\wedge^{max}\xi$ }&
          \multicolumn{1}{|c|}{Summand in $F_{top}$}\\  
      \hline 
      \endhead
      \hline 
           \multicolumn{4}{|r|}{{Continued on next page}} \\ \hline
      \endfoot
      \endlastfoot 
      
                      
   
      $a+c \leq d+f$ & $e \geq b$& $0^b, (a+b+c)^{a+c},(a+c)^{d+f-a-c};$ & $S_{((a+c)^{b+d+f})}V_1 \otimes 
      S_{((a+b)^{d+e},(d+e)^c)}V_2 $\\ 
      $a+b \geq d+e$ && $~0^c,(a+b+c)^{d+e};$ & $\otimes S_{(-a-b-c)^d,(-a-c-e)^{b},(-d-e-f)^{a+c} )}V^*_3$\\
      $d+e+f \geq a+b+c$ &&$(-d-a-c-e)^{b},(-2d-e-f)^{a+c},0^d $ & \\
      \hline
      
      &$e \leq b$ & $0^b, (a+b+c)^{a+c},(a+c)^{d+f-a-c};$ & $S_{((a+c)^{b+d+f})}V_1 $\\
      &$a \geq d$&$~0^c,(a+b+c)^{e},(a+c+e)^{d};$  & $ \otimes 
      S_{((a+b)^{e},(a+e)^d,(d+e)^c)}V_2$ \\
      && $(-a-c-e)^{b-e},(-d-e-a-c)^{e},$ &$\otimes S_{(-a-c-e)^{b+d},(-d-e-f)^{a+c} )}V^*_3$\\
      &&$(-2d-e-f)^{a+c},0^d$&\\
      \hline
      
      &$e \leq b$ & $0^b, (a+b+c)^{a+c},(a+c)^{d+f-a-c};$ & $S_{((a+c)^{b+d+f})}V_1  $\\
      &$a \leq d$&$~0^c,(a+b+c)^{e},(a+c+e)^{a},(a+e)^{d-a};$  & $\otimes S_{((a+b)^{e},(a+e)^{c+d})}V_2$ \\
      && $(-a-c-e)^{b-e},(-d-e-a-c)^{e},$ & $\otimes  
      S_{(-a-c-e)^{b+d},(-a-e-f)^{c},(-d-e-f)^{a})}V^*_3$\\
      &&$(-a-d-e-f)^{c},(-2d-e-f)^{a},0^d$&\\
      \hline
      $a+c \geq d+f$  & $e \geq b$ & $0^b,(a+b+c)^{f},(d+e+f)^d;$ & $S_{(a+c)^{f},(d+e+f-b)^d,(d+f)^b}V_1$ \\
      $a+b \geq d+e$ & $f \leq c$ & $0^c,(a+b+c)^{d+e};$ & $\otimes S_{(a+b)^{d+e},(d+e)^c}V_2$ \\
      $d+e+f \leq a+b+c$ &  & $(-d-e-f)^{a+b+c-d-e-f},(-2d-e-f)^{d+e+f},0^d$ & $\otimes S_{(-d-e-f)^{a+b+c+d}}V^*_3$ \\
      \hline
      & $e \leq b$ & $0^b,(a+b+c)^{d+f};$ & $S_{(a+c)^{d+f},(d+f)^b}V_1$ \\
      & $f \geq c$ & $0^c,(a+b+c)^{e},(d+e+f)^d$ & $\otimes S_{(a+b)^{e},(d+e+f-c)^d,(d+e)^c}V_2$ \\
      & & $(-d-e-f)^{a+b+c-d-e-f},(-2d-e-f)^{d+e+f},0^d$ & $S_{(-d-e-f)^{a+b+c+d}}V^*_3$ \\
      \hline
      & $e \leq b$ & $0^b,(a+b+c)^f,(a+b+f)^d;$ & $S_{(a+c)^f,(a+f)^{b+d}}V_1$ \\
      & $f \leq c$ & $0^c,(a+b+c)^{e},(c+d+e)^{d}$ & $\otimes S_{(a+b)^{e},(d+e)^{c+d}}V_2$ \\
      & $a \geq d$& $(-d-e-f)^{a+b+c-d-e-f},(-2d-e-f)^{d+e+f},0^d$ & $S_{(-d-e-f)^{a+b+c+d}}V^*_3$  \\
      \hline
      & $e \leq b$ & $0^b,(a+b+c)^f,(a+b+f)^a,(a+f)^{d-a};$ & $S_{(a+c)^f,(a+f)^{b+d}}V_1$ \\
      & $f \leq c$ & $0^c,(a+b+c)^{e},(a+c+e)^{a},(a+e)^{d-a}$ & $\otimes S_{(a+b)^{e},(a+e)^{c+d}}V_2$ \\
      & $a \leq d$& $(-a-e-f)^{b+c-e-f},(-d-e-f-a)^{e+f},(-2d-e-f)^{a},0^d$ & $S_{(-a-e-f)^{b+c+d},(-d-e-f)^{a}}V^*_3$\\
      \hline

      $a+c \leq d+f$  & $a \geq d$ & $0^b,(a+b+c)^{a+c},(a+c)^{d+f-a-c};$ & $S_{(a+c)^{b+d+f}}V_1$ \\
      $a+b \geq d+e$ &  & $0^c,(a+b+c)^{e},(a+c+e)^{d};$ & $\otimes S_{(a+b)^{e},(a+e)^{d},(d+e)^{c}}V_2$ \\
      $d+e+f \leq a+b+c$ &  & $(-a-c-e)^{b-e},(-d-a-c-e)^{e},(-2d-e-f)^{a+c},0^d$ & $\otimes 
      S_{(-a-c-e)^{a+b+c},(-d-e-f)^{d}}V^*_3$ \\
      \hline
      & $a \leq d$ & $0^b,(a+b+c)^f,(a+b+f)^a,(a+f)^{d-a};$ & $S_{(a+c)^f,(a+f)^d,(d+f)^b}V_1$ \\
      & $f \leq c$ & $0^c,(a+b+c)^{e},(a+c+e)^a,(a+e)^{d-a}$ & $\otimes S_{(a+b)^e,(a+e)^{c+d}}V_2$ \\
      & & $(-a-e-f)^{b+c-e-f},(-d-e-f-a)^{e+f},(-2d-e-f)^{a},0^d$ & $S_{(-a-e-f)^{b+c+d},(-d-e-f)^{a}}V^*_3$ \\
      \hline
      & $a \leq d$ & $0^b,(a+b+c)^{a+c},(a+c)^{d+f-a-c};$ & $S_{(a+c)^{b+d+f}}V_1$ \\
      & $f \geq c$ & $0^c,(a+b+c)^{e},(a+c+e)^{a},(a+e)^{d-a}$ & $\otimes S_{(a+b)^{e},(a+e)^{c+d}}V_2$ \\
      & & $(-a-c-e)^{b-e},(-d-a-c-e)^{e},$ & $S_{(-a-c-e)^{b+d},(-a-e-f)^{c},(-d-e-f)^{a}}V^*_3$ \\
      & &$(-d-e-f-a)^{c},(-2d-e-f)^{a},0^d$  &\\
      \hline

      $a+c \geq d+f$  & $a \geq d$ & $0^b,(a+b+c)^{f},(a+b+f)^{d};$ & $S_{(a+c)^{f},(a+f)^d,(d+f)^b}V_1$ \\
      $a+b \leq d+e$ &  & $0^c,(a+b+c)^{a+b},(a+b)^{d+e-a-b};$ & $\otimes S_{(a+b)^{c+d+e}}V_2$ \\
      $d+e+f \leq a+b+c$ &  & $(-a-b-f)^{c-f},(-d-a-b-f)^{f},(-2d-e-f)^{a+b},0^d$ & $\otimes 
      S_{(-a-b-f)^{c+d},(-d-e-f)^{a+b}}V^*_3$ \\
      \hline
      & $a \leq d$ & $0^b,(a+b+c)^f,(a+b+f)^a,(a+f)^{d-a};$ & $S_{(a+c)^f,(a+f)^{b+d}}V_1$ \\
      & $e \leq b$ & $0^c,(a+b+c)^{e},(a+c+e)^a,(a+e)^{d-a}$ & $\otimes S_{(a+b)^e,(a+e)^{c+d}}V_2$ \\
      & & $(-a-e-f)^{b+c-e-f},(-d-e-f-a)^{e+f},(-2d-e-f)^{a},0^d$ & $S_{(-a-e-f)^{b+c+d},(-d-e-f)^{a}}V^*_3$ \\
      \hline
      & $a \leq d$ & $0^b,(a+b+c)^{f},(a+b+f)^a,(a+f)^{d-a};$  & $S_{(a+c)^{f},(a+f)^{b+d}}V_1$ \\
      & $e \geq b$ & $0^c,(a+b+c)^{a+b},(a+b)^{d+e-a-b}$ & $\otimes S_{(a+b)^{c+d+e}}V_2$ \\
      & & $(-a-b-f)^{c-f},(-d-a-b-f)^{f},$ & $S_{(-a-b-f)^{c+d},(-a-e-f)^{b},(-d-e-f)^{a}}V^*_3$ \\
      &&$(-d-e-f-a)^{b},(-2d-e-f)^{a},0^d$  &\\
      \hline

      $a+c \leq d+f$  & $a \geq d$ & $0^b,(a+b+c)^{a+c},(a+c)^{d+f-a-c};$ & $S_{(a+c)^{b+d+f}}V_1$ \\
      $a+b \leq d+e$ & $c \geq b$ & $0^c,(a+b+c)^{a+b},(a+b)^{d+e-a-b};$ & $\otimes S_{(a+b)^{c+d+e}}V_2$ \\
      $d+e+f \geq a+b+c$ &  & $(-2a-b-c)^{b},(-d-a-b-f)^{c-b},(-2d-e-f)^{a+b},0^d$ & $\otimes         
      S_{(-a-b-c)^{d},(-2a-b-c-d)^{b},(-a-b-f)^{c-b},(-d-e-f)^{a+c}}V^*_3$ \\
      \hline
      & $a \geq d$ & $0^b,(a+b+c)^{a+c},(a+c)^{d+f-a-c};$ & $S_{(a+c)^{b+d+f}}V_1$ \\
      & $c \leq b$ & $0^c,(a+b+c)^{a+b},(a+b)^{d+e-a-b};$ & $\otimes S_{(a+b)^{c+d+e}}V_2$ \\
      &  & $(-2a-b-c)^{c},(-d-a-c-e)^{b-c},(-2d-e-f)^{a+b},0^d$ & $\otimes 
      S_{(-a-b-c)^{d},(-2a-b-c-d)^{c},(-a-c-e)^{b-c},(-d-e-f)^{a+c}}V^*_3$ \\
      \hline
      & $a \leq d$ & $0^b,(a+b+c)^f,(a+b+f)^a,(a+f)^{d-a};$ & $S_{(a+c)^f,(a+f)^{b+d}}V_1$ \\
      & $e \leq b$ & $0^c,(a+b+c)^{e},(a+c+e)^a,(a+e)^{d-a}$ & $\otimes S_{(a+b)^e,(a+e)^{c+d}}V_2$ \\
      & & $(-a-e-f)^{b+c-e-f},(-d-e-f-a)^{e+f},(-2d-e-f)^{a},0^d$ & $S_{(-a-e-f)^{b+c+d},(-d-e-f)^{a}}V^*_3$ \\
      \hline
      & $a \leq d$ & $0^b,(a+b+c)^{f},(a+b+f)^a,(a+f)^{d-a};$  & $S_{(a+c)^{f},(a+f)^{b+d}}V_1$ \\
      & $e \geq b$ & $0^c,(a+b+c)^{a+b},(a+b)^{d+e-a-b}$ & $\otimes S_{(a+b)^{c+d+e}}V_2$ \\
      & & $(-a-b-f)^{c-f},(-d-a-b-f)^{f},$ & $S_{(-a-b-f)^{c+d},(-a-e-f)^{b},(-d-e-f)^{a}}V^*_3$ \\
      &&$(-d-e-f-a)^{b},(-2d-e-f)^{a},0^d$  &\\
      \hline

      \caption{$b\neq0,~ c \neq 0,~ d\neq 0$} \label{table3-7}
      \end{longtable} 
      
      
   \begin{center}
    \includegraphics[scale=0.75, clip]{sec3/Gorenstein7.pdf}
   \end{center}
     
\begin{center}
\begin{table}[h]
\caption{Candidates for Gorenstein orbits}  \label{table4}
\begin{tabular}{|c|c|c|c|c|c|}
\hline
$a$  & $b$  & $c$ &  $d$  &  $e$  &  $f$ \\
\hline
$*$  & $*$  & $0$ &  $0$  &  $*$  &  $a$ \\
$0$  & $*$  & $0$ &  $0$  &  $*$  &  $*$ \\
$*$  & $*$  & $0$ &  $0$  &  $*$  &  $0$ \\
%$0$  & $*$  & $0$ &  $0$  &  $*$  &  $0$ \\
\hline
$*$  & $0$  & $*$ &  $0$  &  $a$  &  $*$ \\
$0$  & $0$  & $*$ &  $0$  &  $*$  &  $*$ \\
$*$  & $0$  & $*$ &  $0$  &  $0$  &  $*$ \\
%$0$  & $0$  & $*$ &  $0$  &  $*$  &  $*$ \\
\hline
$d+e+f$  & $0$  & $0$ &  $*$  &  $*$  &  $*$ \\
$*$      & $0$  & $0$ &  $*$  &  $0$  &  $*$ \\
$*$      & $0$  & $0$ &  $*$  &  $*$  &  $0$ \\
\hline
$d+e$  & $0$  & $*$ &  $*$  &  $*$  &  $c$ \\
$d+e$  & $0$  & $*$ &  $*$  &  $*$  &  $0$ \\
$0$  & $0$  & $*$ &  $*$  &  $*$  &  $c$ \\
$*$  & $0$  & $*$ &  $*$  &  $0$  &  $c$ \\
$d$  & $0$  & $*$ &  $*$  &  $0$  &  $0$ \\
%$0$  & $0$  & $*$ &  $*$  &  $0$  &  $c$ \\
\hline
$d+f$  & $*$  & $0$ &  $*$  &  $b$  &  $*$ \\
$d+f$  & $*$  & $0$ &  $*$  &  $0$  &  $*$ \\
$0$  & $*$  & $0$ &  $*$  &  $b$  &  $*$ \\
$*$  & $*$  & $0$ &  $*$  &  $b$  &  $0$ \\
$d$  & $*$  & $0$ &  $*$  &  $0$  &  $0$ \\
%$0$  & $*$  & $0$ &  $*$  &  $b$  &  $0$ \\
\hline
$*$  & $*$  & $*$ &  $0$  &  $a+b$  &  $a+c$ \\
$*$  & $*$  & $*$ &  $0$  &  $b$  &  $c$ \\
$*$  & $*$  & $*$ &  $0$  &  $0$  &  $a+c$ \\
$*$  & $*$  & $*$ &  $0$  &  $a+b$  &  $0$ \\
\hline
$0$  & $*$  & $*$ &  $*$  &  $b$  &  $c$ \\
%$*$  & $*$  & $*$ &  $a$  &  $0$  &  $c$ \\
%$*$  & $*$  & $*$ &  $a$  &  $b$  &  $0$ \\
$*$  & $*$  & $*$ &  $a$  &  $b$  &  $c$ \\
%$0$  & $*$  & $*$ &  $*$  &  $b$  &  $0$ \\
%$0$  & $*$  & $*$ &  $*$  &  $0$  &  $c$ \\
\hline
\end{tabular}
\end{table}
\end{center}
     
\bc{corollary3} For non-equioriented quiver $A_3$, let $V$ be a representation for which all indecomposables occur as summands of $V$ with non-zero multiplicities. The orbit closure $\overline{O_V}$ is Gorenstein iff the Coxeter orbits ($\tau$-orbits of the Auslander-Reiten quiver) are constant. 
\ec
\bpr
Sufficiency follows from Proposition \ref{Prop6}. Necessity follows from Case $7$.
\qed 
\newpage



==> subsec3.tex <==
%-------------------------------------------------------------------------------------------------------------------
\subsection{$F_{top}$ and classification of Gorenstein orbits}
%In this section, we investigate classes of orbit closures that are Gorenstein. For the case of non-equioriented A_3, we also give a description of the last (top) term occuring in the resolution. 
%By \cite{MR1988690}, an orbit closure is Gorenstein if and only if the top module occuring in its resolution is irreducible and 1-dimensional. \par

Lets consider a Dynkin quiver $Q$. The top exterior power of $\xi(a)$ is 
\begin{eqnarray}  S_{[0^{d_1(ta)}, d_1(ha)^{d_2(ta)}, \cdots, (d_1(ha)+\cdots+d_{s-1}(ha))^{d_s(ta)}]}(ta) \\ \nonumber \otimes S_{[(-d_2(ta)-\cdots-d_s(ta))^{d_1(ha)}, \cdots, -d_s(ta)^{d_{s-1}(ha)}, 0^{d_s(ha)}]}(ha)^*\end{eqnarray}
%\[ S_{[0^{d_1(ta)}, d_1(ha)^{d_2(ta)}, \cdots, (d_1(ha)+\cdots+d_{s-1}(ha))^{d_s(ta)}]}(ta) \otimes S_{[(-d_2(ta)-\cdots-d_s(ta))^{d_1(ha)}, \cdots, -d_s(ta)^{d_{s-1}(ha)}, 0^{d_s(ha)}]}(ha) \]
Thus the top exterior power of $\xi$ is given by 
   \begin{equation} \bigwedge^{top} \xi= \bigotimes_{x \in Q_0} S(x)(k_1(x)^{d_1(x)},\cdots,k_s(x)^{d_s(x)} )   
   \label{topterm}
   \end{equation}
where 
   \begin{equation} k_t(x)= \sum_{a \in Q_1; ta=x} \sum_{u<t} d_u(ha)-\sum_{a \in Q_1; ha=x} \sum_{u>t} d_u(ta)
   \end{equation} \par

First, we give a sufficient condition for the orbit closure $\overline{O}_V$ to be Gorenstein in case of any Dynkin quiver $Q$. 
By \cite{MR1988690}, we have that if for every $x \in Q_0$, the number 
   \begin{equation} k_t(x)-\sum_{u<t}d_u(x)+\sum_{u>t}d_u(x) \label{condition}
   \end{equation} 
is independent of $t$, $(t=1,2, \cdots, s)$, then the corresponding orbit closure is Gorenstein.
The following lemma shows that this condition means that the $\tau$-orbits in the Auslander-Reiten quiver are constant- 
\bl{lemma3.4.1} Let $\tau$ denote the Auslander-Reiten translate and suppose $\underline{d}(x)=(d_u(x))_{u=1,2,\cdots, s}$ are dimensions of the flag at vertex $x$ in the desingularization $Z$. Then
\[ \langle \underline{e}_x, \underline{d}_t(x) \rangle = -\langle \underline{d}_{t+1}(x), \underline{e}_x \rangle  \] 
for all $x \in Q_0$ and $t=1,2,\cdots, s-1$, where $\underline{e}_x$ is the dimension vector of the simple representation supported at $x$.
\el 
\bpr (\ref{condition}) translates to the equations- 
   \begin{equation} k_{t+1}(x)-k_t(x)=d_t(x)+d_{t+1}(x)
   \end{equation}
for $x \in Q_0$ and $t=1,2,\cdots, s-1$. This is equivalent to-   
   \begin{equation} \sum_{a \in Q_1;ta=x}d_t(ha)+\sum_{a \in Q_1; ha=x}d_{t+1}(ta)=d_{t+1}(x)+d_t(x)
   \end{equation}
for all $x \in Q_0$ and $t=1,2,\cdots, s-1$. These conditions can be expressed in terms of Euler form as follows-
   \begin{eqnarray} \nonumber
   \langle \underline{e}_x, \underline{d}_t \rangle &=& d_t(x)-\sum_{a \in Q_1;ta=x}d_t(ha) \\ \nonumber
   &=& \sum_{a \in Q_1;ha=x}d_{t+1}(ta)-d_{t+1}(x) \\ \nonumber
   &=& -\langle \underline{d}_{t+1}, \underline{e}_x \rangle
   \end{eqnarray} 
   Thus, 
   \begin{equation} \langle \underline{e}_x, \underline{d}_t \rangle = -\langle \underline{d}_{t+1}, \underline{e}_x
    \rangle \label{euler}
   \end{equation}
where $\underline{e}_x$ is the dimension vector of the simple representation supported at $x$.    \qed   


\bp{Prop3.4.2} Assume that for each $t=1,2, \cdots, s-1$ we have $\underline{d}_{t+1}=\tau^+ \underline{d}_t$. Then the complex $F_{\bullet}$ is self-dual. If the incidence variety comes from Reineke desingularization and the corresponding orbit closure is normal with rational singularities, then it is also Gorenstein. 
\ep
\bpr 
\qed

Next, we investigate necessary conditions for for the orbit closure $\overline{O}_V$ to be Gorenstein in case of non-equioriented $A_3$. 
First we prove that the top exterior power if $\xi$ contributes to the last term of the resolution.

\noindent \textbf{Notation}: We will denote the topmost exterior power of $\xi$ by $\bigwedge^{top} \xi$. %In cases when $\bigwedge^{top} \xi$ does not contribute to $F_{top}$, we denote the maximal contributing exterior power by $\bigwedge^{max} \xi$. \\

\noindent For the case of non-equioriented $A_3$, we investigate the following questions:
\begin{enumerate}
\item In what cases does $\bigwedge^{top}\xi$ contribute? To which term $F_i$ does $\bigwedge^{top}\xi$ contribute?  
\item In cases not covered by $(1)$ what is the $\bigwedge^{max}\xi$ which contributes? Does it contribute to $F_{top}$? 
\end{enumerate}

First we investigate the cases in which $\bigwedge^{top}\xi$ contributes. Observe that a contribution will occur whenever the Bott exchanges give a non-increasing sequence for every term of
\[\bigg( (0^b, (a+b+c)^{d+f}),~~(0^c, (a+b+c)^{d+e}),~((-2d-e-f)^{a+b+c},0^d) \bigg) \]
Also, note that if any of $b,c$ or $d$ are zero, then there are no exchanges for the corresponding term in the weight. We base our cases on this observation.
\bp{Prop3.4.3} $\bigwedge^{top}\xi$ contributes to $F_{top}$ in the following cases when the corresponding conditions are satisfied:
\begin{table}[h]
\centering
      \renewcommand{\arraystretch}{1.3}
\begin{tabular}{|c|ccc|}
\hline
Cases & \multicolumn{3}{|c|}{Conditions}\\
\hline
$b=0, ~c=0, ~d=0$ &   no condition &&      \\
\hline
$b\neq 0, ~c=0, ~d=0$ &  $a+c \geq d+f$ &  &      \\
\hline
$b=0, ~c\neq0, ~d=0$ &  & $a+b \geq d+e$ &  \\
\hline
$b=0,~ c=0,~ d\neq0$ &  &  &$ d+e+f \geq a+b+c  $      \\
\hline
$b=0, ~c\neq0,~ d\neq0$ &  & $a+b \geq d+e$ ,&~ $d+e+f \geq a+b+c$  \\
\hline
$b\neq 0, ~c=0, ~d\neq0$ & $a+c \geq d+f$ ,& & $ d+e+f \geq a+b+c $       \\
\hline
$b\neq 0,~ c\neq0, ~d=0$ &$ a+c \geq d+f$, &~$a+b \geq d+e$ & \\
\hline
$b\neq0,~c\neq0,~d\neq0$ & $a+c \geq d+f $, & ~$a+b \geq d+e $, &~$ d+e+f \geq a+b+c$ \\
\hline
\end{tabular}
\caption{}
\label{table1}
\end{table}
\ep
In each case, we give a description of $F_{top}$. Recall that for our case of non-equioriented $A_3$, we have desingularization-
  \begin{center}
  \includegraphics[scale=0.5, clip]{sec3/desing.pdf}
  \end{center}
As before, let $V=a(0K0)+b(0KK)+c(KK0)+d(KKK)+e(K00)+f(00K)$ be a representation of $A_3$.   
Then \[d_1=(b, ~a+b+c,~ c) ;~~ d_2=(d+f, ~d,~ d+e)\]  
From (\ref{topterm}) the weights for $\bigwedge^{top}\xi$ are:
\[(0^b, (a+b+c)^{d+f}),~~(0^c, (a+b+c)^{d+e}),~((-2d-e-f)^{a+b+c},0^d) \]  
\bl{lemma3} For a weight $(0^b, \lambda;~ 0^c, \mu;-\nu, 0^d)$ of $\bigwedge^{|\lambda|+|\mu|}\xi$, $D(\lambda,\mu)=$ codim $\overline{O}_V$ implies that the partition (if any) arising from $(0^b, \lambda; ~0^c, \mu; -\nu, 0^d)$ corresponds to a summand of $F_{top}$.
\el
\bpr...
\qed \par

Next we show that a contribution from $\bigwedge^{top}\xi$ always goes to $F_{top}$.
\bl{lemma3.4.4} If the weight of the $\bigwedge^{top}\xi$ gives a non-zero partition after Bott exchanges, then the corresponding representation is a $1$ -dimensional summand of $F_{top}$. 
%If $\bigwedge^{top} \xi$ contributes, it always contributes to $F_{top}$. 
\el
\bpr Suppose  
We apply Bott's algorithm to each weight to get:
 \[[0^b, (a+b+c)^{d+f}] = ((a+c)^{d+f}, (d+f)^b) ~\hbox{after}~  b(d+f) ~\hbox{Bott exchanges}\]
 \[[0^c, (a+b+c)^{d+e}] = ((a+b)^{d+e}, (d+e)^c) ~\hbox{after}~ c(d+e) ~\hbox{Bott exchanges}\]
 \[[(-2d-e-f)^{a+b+c},0^d] = ((-a-b-c)^d, (-d-e-f)^{a+b+c}) ~\hbox{after}~ d(a+b+c) ~\hbox{Bott exchanges}\]
 
   \begin{eqnarray} \nonumber
   D(\lambda, \mu)&=&[(d+f)(a+b+c)]+[(d+e)(a+b+c)]\\ \nonumber
   &&-[b(d+f)+c(d+e)+d(a+b+c)] \\ \nonumber
   &=&ad+ae+af+be+cf \\ \nonumber
   &=&\hbox{codim}~ \overline{O}_V 
   \end{eqnarray} 
\qed


In the case $b \neq 0, ~c \neq 0,~ d\neq 0$, if the condition on the right is satisfied, then applying Bott exchanges to 
\[\bigg( (0^b, (a+b+c)^{d+f}),~~(0^c, (a+b+c)^{d+e}),~((-2d-e-f)^{a+b+c},0^d) \bigg) \] gives the partitions -
\[\bigg( ((a+c)^{d+f}, (d+f)^b),~~((a+b)^{d+e}, (d+e)^c),~((-a-b-c)^{d},(-d-e-f)^{a+b+c}) \bigg) \]
If the orbit closure is Gorenstein, then $F_{top}$ is $1$-dimensional. This implies that the above partitions are rectangles, which means 
\[a+c=d+f, ~~a+b=d+e, ~~ a+b+c=d+e+f\]
When  $a \neq 0, ~e \neq 0,~ f\neq 0$, these conditions imply that $a=d, ~b=e$ and $c=f$.
Applying the same logic to each of the above cases, we get necessary conditions for the orbit closure to be Gorenstein. We list these conditions in the following table. \par \vskip0.5cm


%\advance\leftskip-3.5cm
\begin{center}
      \renewcommand{\arraystretch}{1.2}
\begin{longtable}{|c|cc|c|}
 \hline
Cases & \multicolumn{2}{|c|}{$\bigwedge^{top}\xi$ contributes if..}  & $\overline{O}_V$ is  \\
                                   &&& Gorenstein implies... \\ 
\hline 
\endfirsthead
       \hline 
          \multicolumn{1}{|c|}{Cases} &          
          \multicolumn{2}{|c|}{$\bigwedge^{top}\xi$ contributes if..} &
          \multicolumn{1}{|c|}{ $\overline{O}_V$ is Gorenstein implies..} \\
      \hline 
      \endhead
      \hline 
           \multicolumn{4}{|r|}{{Continued on next page}} \\ \hline
      \endfoot
      \endlastfoot
     
\multirow{3}{*}{$b=0, ~c=0, ~d=0$} & $a \neq 0, ~ e\neq 0, ~ f \neq0 $ &always & no condition     \\
                                                          & $a \neq 0, ~ e= 0, ~ f \neq0 $ &always & no condition     \\   
                                                          & $a \neq 0, ~ e\neq 0, ~ f = 0 $ &always & no condition     \\
 \hline
\multirow{4}{*}{$b\neq 0, ~c=0, ~d=0$}  &  $a \neq 0, ~ e\neq 0, ~ f \neq0 $ & $a \geq f$ & $a=f$     \\
                                                                &  $a \neq 0, ~ e= 0, ~ f \neq0 $ & $a \geq f$ & $a=f$     \\
                                                                &  $a \neq 0, ~ e\neq0, ~ f =0 $ & always & no condition     \\
                                                                &  $a = 0, ~ e\neq 0, ~ f =0 $ & always & no condition     \\
\hline

\multirow{4}{*}{$b=0, ~c\neq0, ~d=0$} &  $a \neq 0, ~ e\neq 0, ~ f \neq0 $ & $a \geq e$ & $a=e$     \\
                                                                &  $a \neq 0, ~ e\neq 0, ~ f =0 $ & $a \geq e$ & $a=e$     \\
                                                                &  $a \neq 0, ~ e=0, ~ f \neq0 $ & always & no condition     \\
                                                                &  $a = 0, ~ e = 0, ~ f \neq 0 $ & always & no condition     \\
\hline
\multirow{4}{*}{$b=0,~ c=0,~ d\neq0$ } &  $a \neq 0, ~ e\neq 0, ~ f \neq0 $ & $d+e+f \geq a$ & $d+e+f=a$     \\
                                                                &  $a \neq 0, ~ e\neq 0, ~ f =0 $ & $d+e \geq a$ & $d+e=a$     \\
                                                                &  $a \neq 0, ~ e=0, ~ f \neq0 $ & $d+f \geq a$ & $d+f=a$     \\
                                                                &  $a \neq 0, ~ e = 0, ~ f = 0 $ & $d \geq a$ & $d=a$   \\
\hline

\multirow{3}{*}{$b=0, ~c\neq0,~ d\neq0$}   & $a \neq 0, ~e \neq 0,~ f\neq 0$ & $a \geq d+e, ~ d+e+f \geq a+c$ & $a=d+e, ~c=f$ \\
                                                                   & $a = 0, ~e \neq 0,~ f\neq 0$ & $f \geq c$ & $c=f$     \\
                                                                   &  $a \neq 0, ~e = 0,~ f \neq 0$ & $a \geq d,~d+f \geq a+c$ & $a=d, ~c=f$    \\
                                                                   
\hline
\multirow{3}{*}{$b\neq 0, ~c=0, ~d\neq0$} & $a \neq 0, ~e \neq 0,~ f\neq 0$ & $a \geq d+f, ~ d+e+f \geq a+b$ & $a=d+f, ~b=e$ \\
                                                                   & $a = 0, ~e \neq 0,~ f\neq 0$ & $e \geq b$ & $b=e$     \\
                                                                   &  $a \neq 0, ~e \neq 0,~ f= 0$ & $a \geq d,~d+e \geq a+b$ & $a=d, ~b=e$    \\
                                                                   
\hline

\multirow{6}{*}{$b\neq 0,~ c\neq0, ~d=0$ }&  $a \neq 0, ~ e\neq 0, ~ f \neq0 $ & $a+b\geq e,~a+c \geq f$ & $a+b=e, ~a+c=f$  \\
                                                                   &  $a =0, ~ e\neq 0, ~ f \neq0 $ & $ b \geq e,~ c \geq f$ & $b=e,~c=f$     \\
                                                                   &  $a \neq 0, ~ e= 0, ~ f \neq0 $ & $a+c \geq f$ & $a+c=f$      \\
                                                                   &  $a \neq 0, ~ e\neq 0, ~ f =0 $ & $a+b\geq e$ & $a+b=e$      \\
                                                                   &  $a = 0, ~ e = 0, ~ f \neq0 $ & $c\geq f$ & $c=f$      \\
                                                                   &  $a = 0, ~ e\neq 0, ~ f =0 $ & $b\geq e$ & $b=e$      \\
\hline
$b\neq0,~c\neq0,~d\neq0$ &  $a \neq 0, ~e \neq 0,~ f\neq 0$ &  $a+c \geq d+f $, ~$a+b \geq d+e $,&  $a=d, ~b=e, ~c=f$   \\
             &&             ~$ d+e+f  \geq a+b+c$ &\\
\hline 

\caption{Cases} \label{table2}
\end{longtable}
\end{center}

\vskip1cm

Now we consider what happens if the conditions on the right are not satisfied in the cases listed in Proposition \ref{Prop4}. In this event, the top exterior power $\bigwedge^{top}\xi$ does not contribute any term to $F_{top}$. For each case, we obtain a description of the term that does contribute to $F_{top}$ (we denote the corresponding exterior power by $\bigwedge^{max}\xi$) and state the necessary condition for the orbit closure to be Gorenstein. \par

\noindent \textbf{Case 1:} $b\neq 0, ~c=0, ~d=0$ - in this case dim $\xi = (a+b)(e+f)$ and codim $\overline{O}_V = ae+af+be$. \par If $a \neq  
   0, ~ e \neq 0, ~f \neq 0$, the weight in $\bigwedge^{top}\xi$ is of the form
   \[ \big( 0^b,(a+b)^f ;~ (a+b)^e ;~(-e-f)^{a+b} \big) \] 
   If $a \geq f$, the above term gives the summand $S_{(a^f,f^b)}V_1 \otimes S_{(a+b)^e}V_2 \otimes S_{(e+f)^{a+b}}V^*_3$ of 
   $F_{top}$ (as noted in Proposition \ref{Prop4}). However, if $a \leq f$, the above term contributes nothing. In this case, it follows from 
   Remark \ref{} that $\bigwedge^{max}\xi$ has a weight of the form  \[ \big( 0^b,(a+b)^k,k^{f-k} ;~(a+b)^e 
   ; - \nu  \big) \] where $k < f$. By Lemma \ref{lemma3} this weight must satisfy the condition $D(\lambda,\mu) = ae+af+be$. Substitution   
   gives
   \begin{eqnarray} \nonumber
   k(a+b+f-k)+(a+b)e-bk&=&ae+af+be \\ \nonumber
   i.e. ~~k^2-k(a+f)+af&=&0   
   \end{eqnarray}  This implies $k=a$ (since $k<f$). So the weight for $\bigwedge^{max}\xi$ is  \[ \big(  
   0^b,(a+b)^a,a^{f-a};~ (a+b)^e ; ~(-a-e)^b,(-e-f)^a  \big) \]  Using this weight it is easy to derive the corresponding weights for remaining 
    cases in the following table  
      \vskip0.5cm
 
      \renewcommand{\arraystretch}{1.5}
      \begin{longtable}[c]{|p{0.08cm}p{0.08cm}p{0.08cm}|p{2cm}|p{6.1cm}|p{6.5cm}|}     
      \hline
      $a$ & $e$ & $f$ &Condition & Weight of $\bigwedge^{max}\xi$& Corresponding summand in $F_{top}$ \\
                                        
      \hline
      \endfirsthead
       \hline 
          \multicolumn{1}{|c}{$a$} &
          \multicolumn{1}{c}{$e$} &
          \multicolumn{1}{c|}{$f$} &
          \multicolumn{1}{|c|}{Condition} &
          \multicolumn{1}{|c|}{Weight of $\wedge^{max}\xi$ }&
          \multicolumn{1}{|c|}{Corresponding summand in  $F_{top}$}\\  
      \hline 
      \endhead
      \hline 
           \multicolumn{6}{|r|}{{Continued on next page}} \\ \hline
      \endfoot
      \endlastfoot

      $*$ & $*$ & $*$ & $a < f$&$\big(0^b, (a+b)^a, a^{f-a};~(a+b)^e;$ &  
      $S_{(a^{b+f})}V_1 \otimes S_{((a+b)^e)}V_2 $\\
      &&&&$(-a-e)^b,(-e-f)^{a} \big)$& $\otimes S_{((-e-a)^b,(-e-f)^{a})}V^*_3$ \\
      \hline
      $0$ & $*$ & $*$ & $a < f$ & $\big( 0^{b+f};~b^e;~-e^b  \big)$ &$S_{(b^e)}V_2 \otimes 
      S_{(-e^b)}V^*_3$ \\
      \hline
      $*$ & $0$ & $*$ & $a < f$ & $\big( 0^b, (a+b)^a,a^{f-a}; ~\phi ;~-a^b,-f^a  \big)$ &$S_{(a^{b+d+f})}V_1 
       \otimes S_{(-a^b,-f^a)}V^*_3$ \\
      \hline
      $*$ & $*$ & $0$ & \multicolumn{2}{|c|}{in this case $\wedge^{top}\xi$ contributes}&$S_{((a+b)^e)}V_2 \otimes 
      S_{(e^{a+b})}V^*_3$  \\
      \hline
      $0$ & $0$ & $*$ & \multicolumn{2}{|c|}{in this case codim $\overline{O}_V = 0$  }& $0$  \\
      \hline
      $0$ & $*$ & $0$ & \multicolumn{2}{|c|}{in this case $\wedge^{top}\xi$ contributes}&$S_{(b^e)}V_2 \otimes 
      S_{(e^b)}V^*_3$ 
      \\
      \hline
      $*$ & $0$ & $0$ & \multicolumn{3}{|c|}{in this case dim $\xi = 0$ } \\
      \hline
      \caption{$b\neq 0, ~c=0, ~d=0$}\label{table3-1}
      \end{longtable}


\vskip1cm
From Table \ref{table2} and Table \ref{table3-1} we can list the candidates for Gorenstein orbits in terms of conditions on multiplicities of indecomposables. We express these orbits in the shape of the AR quiver for easy reading:
\vskip1cm
   \begin{center}
    \includegraphics[scale=0.75, clip]{sec3/Gorenstein1.pdf}
   \end{center}
\vskip0.7cm
  
  
 
We repeat this procedure for the remaining 6 cases. We state only the sub-case $a \neq 0, e\neq 0, f \neq 0$ each time (the remaining subcases can be derived from the above) and the possible candidates for Gorenstein orbits. \par
\newpage
\noindent \textbf{Case 2:} $b=0, ~c\neq0, ~d=0$ 
  
      \renewcommand{\arraystretch}{1.5}
      \begin{table}[h]
      \begin{tabular}{|c|c|c|}     
      \hline
      Condition & Weight of $\wedge^{max}\xi$  & Summand in $F_{top}$ \\
                      
      \hline

      $a \leq f$& $\big( (a+b)^f;~~0^c,(a+c)^a,a^{e-a};~~(-a-f)^c,(-e-f)^{a} \big)$ &  $S_{((a+b)^f)}V_1 \otimes 
      S_{(a^{c+e})}V_2 $\\
       && $\otimes S_{((-a-f)^c,(-e-f)^{a})}V^*_3$ \\
      \hline
     
      \end{tabular} \caption{ $b=0, ~c\neq0, ~d=0$} \label{table3-2}
      \end{table}

   
   \begin{center}
    \includegraphics[scale=0.75, clip]{sec3/Gorenstein2.pdf}
   \end{center}
 \vskip2cm
  
   \noindent \textbf{Case 3:} $b=0,~ c=0,~ d\neq0$ \vskip0.5cm
      \renewcommand{\arraystretch}{1.5}
      \begin{table}[h]
      \begin{tabular}{|c|c|c|}     
      \hline
      Condition & Weight of $\wedge^{max}\xi$  & Summand in $F_{top}$ \\
                      
      \hline
     $d+e+f \leq a$ & $\big( a^{d+f};~ a^{e},(d+e+f)^d;$&  $S_{(a^{d+f})}V_1                
        \otimes S_{(a^{e},(d+e+f)^d)}V_2 $\\
      &$(-d-e-f)^{a-d-e-f},(-2d-e-f)^{d+e+f}, 0^d \big)$ & $\otimes S_{(-d-e-f^a)}V^*_3$ \\

      \hline
     
      \end{tabular} \caption{$b=0,~ c=0,~ d\neq0$} \label{table3-3}
      \end{table}
    
   \begin{center}
    \includegraphics[scale=0.75, clip]{sec3/Gorenstein3.pdf}
   \end{center}      

\newpage
\noindent \textbf{Case 4:} $b=0,~ c\neq 0,~ d\neq0$ \vskip0.5cm
  
      \renewcommand{\arraystretch}{1.5}
      \begin{table}[h]
      \begin{tabular}{|c|c|c|c|} 
    
      \hline
      Condition& cases & Weight of $\wedge^{max}\xi$  & Summand in $F_{top}$ \\
                      
      \hline
       $a \leq d+e,$ & $f \geq c$ & $\big(~(a+c)^{d+f};0^b, (a+c)^a,a^{d+e-a};$ & $S_{((a+c)^{d+f})}V_1 \otimes 
                                                                               S_{(a^{c+d+e})}V_2 $\\
       $ d+e+f \geq a+c$ &&$(-d-f-a)^{c},(-2d-e-f)^{a}, 0^d \big)$& $\otimes S_{((-a-c)^d,(-a-f)^c,(-d-e-f)^a)}V^*_3$ \\
      
      \hline
      &$f \leq c$ &$\big(~(a+c)^{d+f};0^c, (a+c)^a,a^{d+e-a};$ & $S_{((a+c)^{d+f})}V_1\otimes S_{(a^{c+d+e})}V_2 $\\
      &&$(-d-f-a)^{c},(-2d-e-f)^{a}, 0^d \big)$& $ \otimes S_{((-a-c)^d,(-a-f)^c,(-d-e-f)^a)}V^*_3$ \\
      
      \hline
      
      $a \geq d+e$& $f \geq c$ &$\big(~(a+c)^{d+f};0^c, (a+c)^e,(d+e+f)^d;$ & $S_{((a+c)^{d+f})}V_1  $\\
      $d+e+f \leq a+c$ &&$(-d-e-f)^{a+c-d-e-f},(-2d-e-f)^{d+e+f},0^d \big)$& $\otimes 
      S_{(a^e,(d+e+f-c)^d,(d+e)^c)}V_2$ \\
      &&&$\otimes S_{((-d-e-f)^{a+c+d})}V^*_3$\\
      \hline
      & $f \leq c$ &$\big(~(a+c)^{f},(d+e+f)^d;0^c, (a+c)^{d+e};$ & $S_{((a+c)^f,(d+e+f)^d)}V_1 $\\
      &&$(-d-e-f)^{a+c-d-e-f},(-2d-e-f)^{d+e+f}, 0^d \big)$& $\otimes  S_{(a^{d+e},(d+e)^c)}V_2$ \\
      &&&$\otimes S_{((-d-e-f)^{a+c+d})}V^*_3$\\
      \hline
       $a \leq d+e$& $f\leq c$ &$\big(~(a+c)^{f},(a+f)^d;0^c, (a+c)^a,(d+e-a)^d;$ & $S_{((a+c)^{f},(a+f)^d)}V_1 \otimes 
       S_{(a^{c+d+e})}V_2 $\\

      $d+e+f \leq a+c$ &&$(-a-f)^{c-f},(-d-f-a)^{f},(-2d-e-f)^{a},0^d \big)$&$\otimes(-a-f)^{c+d},(-d-e-f)^{a})}V^*_3$ \\
     
      \hline
      \end{tabular} \caption{$b=0,~ c\neq 0,~ d\neq0$} \label{table3-4}
      \end{table}

      
   \begin{center}
    \includegraphics[scale=0.75, clip]{sec3/Gorenstein4.pdf}
   \end{center} 
        
\newpage
\noindent \textbf{Case 5:} $b\neq0,~ c = 0,~ d\neq0$ \par
      \begin{center}
      \renewcommand{\arraystretch}{1.5}
      \begin{table}[h]
      \begin{tabular}{|c|c|c|c|}     
      \hline
      Condition& cases & Weight of $\wedge^{max}\xi$  & Summand in $F_{top}$ \\
                      
      \hline
      $a \leq d+f,$& $e \geq b$ & $\big(0^b, (a+b)^a,a^{d+f-a};~(a+b)^{d+e};$ & $S_{(a^{b+d+f})}V_1 \otimes   
       S_{((a+b)^{d+e})}V_2 $\\
       $ d+e+f \geq a+b$ &&$(-d-e-a)^{b},(-2d-e-f)^{a}, 0^d \big)$& $\otimes S_{((-a-b)^d,(-a-e)^b,(-d-e-f)^a)}V^*_3$ \\
      \hline

      & $e \leq b$ &$\big(0^b, (a+b)^a,a^{d+f-a};~(a+b)^{d+e};$ & $S_{(a^{b+d+f})}V_1 \otimes  
       S_{((a+b)^{d+e})}V_2 $\\
       &&$(-d-e-a)^{b},(-2d-e-f)^{a}, 0^d \big)$& $\otimes S_{((-a-b)^d,(-a-e)^b,(-d-e-f)^a)}V^*_3$ \\
       \hline
       
       $a \geq d+f$& $e \geq b$ &$\big(0^b, (a+b)^f,(d+e+f)^d;~(a+b)^{d+e};$ & $S_{(a^f,(d+e+f-b)^d,(d+f)^b)}V_1 $\\
       $d+e+f < a+b$ &&$(-d-e-f)^{a+b-d-e-f},(-2d-e-f)^{d+e+f},0^d \big)$& $\otimes S_{((a+b)^{d+e})}V_2$ \\
       &&&$\otimes S_{((-d-e-f)^{a+b+d})}V^*_3$\\
       \hline
       & $e \leq b$ &$\big(0^b, (a+b)^{d+f};~(a+b)^{e},(d+e+f)^d;$ & $S_{(a^{d+f},(d+f)^b)}V_1 $\\
       &&$(-d-e-f)^{a+b-d-e-f},(-2d-e-f)^{d+e+f}, 0^d \big)$& $\otimes S_{((a+b)^e,(d+e+f)^d)}V_2 $ \\
       &&&$\otimes  S_{((-d-e-f)^{a+b+d})}V^*_3$\\

       \hline
        $a \leq d+f$& $e \leq b$ &$\big(0^b, (a+b)^a,(d+f-a)^d;~(a+b)^{e},(a+e)^d;$ &  $S_{(a^{b+d+f})}V_1 \otimes 
        S_{((a+b)^{e}, (a+e)^d)}V_2 $\\
       $d+e+f \leq a+b$ &&$(-a-e)^{b-e},(-d-e-a)^{e},(-2d-e-f)^{a},0^d \big)$& $\otimes 
       S_{((-a-e)^{b+d},(-d-e-f)^{a})}V^*_3$ \\
     
      \hline
     
      \end{tabular} \caption{ $b\neq0,~ c = 0,~ d\neq0$} \label{table3-5}
      \end{table}
      \end{center}
      
   \begin{center}
    \includegraphics[scale=0.75, clip]{sec3/Gorenstein5.pdf}
   \end{center}    
     
\newpage
\noindent \textbf{Case 6:} $b\neq0,~ c \neq 0,~ d=0$ \par
      
      \renewcommand{\arraystretch}{1.5}
      \begin{table}[h]
      \begin{tabular}{|c|c|c|c|}     
      \hline
      Condition& cases & Weight of $\wedge^{max}\xi$  & Summand in $F_{top}$ \\
                      
      \hline
      $a+c \leq f$, && $0^b, (a+b+c)^{a+c},(a+c)^{f-a-c};$ & $S_{((a+c)^{b+f})}V_1 \otimes S_{((a+b)^{e},e^c)}V_2 $\\ 
       
      $a+b \geq e$ && $~0^c,(a+b+c)^{e};$ & $\otimes S_{(-a-c-e)^{b},(-e-f)^{a+c} )}V^*_3$\\
      &&$(-a-c-e)^{b},(-e-f)^{a+c} $ & \\
      \hline
      $a+c \geq f$,  && $0^b, (a+b+c)^f;$ & $S_{((a+c)^{f},f^b)}V_1 \otimes S_{((a+b)^{c+e})}V_2 $\\
      $ a+b \leq e$ &&$~0^c,(a+b+c)^{a+b},(a+b)^{e-a-b};$  & $\otimes S_{(-a-b-f)^{c},(-e-f)^{a+b} )}V^*_3$ \\
      && $(-a-b-f)^{c},(-e-f)^{a+b}$ &\\
      \hline
      $a+c \leq f,$ & $c \geq b$ & $ 0^b, (a+b+c)^{a+c},(a+c)^{f-a-c};$ &  
                                                 $S_{((a+c)^{b+f})}V_1 \otimes S_{((a+b)^{e},e^c)}V_2 $\\
      $ a+b \leq e$ &&$ 0^c,(a+b+c)^{a+b},(a+b)^{e-a-b};$& $\otimes 
      S_{((-2a-b-c)^{b},(-a-b-f)^{c-b},(-e-f)^{a+b} )}V^*_3$ \\
      &&$(-2a-b-c)^{b},(-a-b-f)^{c-b},(-e-f)^{a+b} $&\\
      \hline
      &$c \leq b$ & $ 0^b, (a+b+c)^{a+c},(a+c)^{f-a-c};$ & $S_{((a+c)^{b+f})}V_1 \otimes 
                                                                               S_{((a+b)^{e},e^c)}V_2 $\\
       & & $~0^c,(a+b+c)^{a+b},(a+b)^{e-a-b}; $& $\otimes 
      S_{((-2a-b-c)^{b},(-a-c-e)^{b-c},(-e-f)^{a+b} )}V^*_3$ \\ 
      & & $(-2a-b-c)^{b},(-a-c-e)^{b-c},(-e-f)^{a+b} $& \\ \hline
      \end{tabular} \caption{$b\neq0,~ c \neq 0,~ d=0$} \label{table3-6}
      \end{table}
      
   \begin{center}
    \includegraphics[scale=0.75, clip]{sec3/Gorenstein6.pdf}
   \end{center}      
 
\newpage      
\noindent \textbf{Case 7:} $b\neq0,~ c \neq 0,~ d \neq 0$ \par
      
      \renewcommand{\arraystretch}{1.5}
     
      \begin{longtable}{|c|c|c|c|}     
      \hline
      Condition& cases & Weight of $\wedge^{max}\xi$  & Summand in $F_{top}$ \\
      \hline
\endfirsthead
       \hline 
          \multicolumn{1}{|c|}{Condition} &
          \multicolumn{1}{|c|}{cases} &
          \multicolumn{1}{|c|}{Weight of $\wedge^{max}\xi$ }&
          \multicolumn{1}{|c|}{Summand in $F_{top}$}\\  
      \hline 
      \endhead
      \hline 
           \multicolumn{4}{|r|}{{Continued on next page}} \\ \hline
      \endfoot
      \endlastfoot 
      
                      
   
      $a+c \leq d+f$ & $e \geq b$& $0^b, (a+b+c)^{a+c},(a+c)^{d+f-a-c};$ & $S_{((a+c)^{b+d+f})}V_1 \otimes 
      S_{((a+b)^{d+e},(d+e)^c)}V_2 $\\ 
      $a+b \geq d+e$ && $~0^c,(a+b+c)^{d+e};$ & $\otimes S_{(-a-b-c)^d,(-a-c-e)^{b},(-d-e-f)^{a+c} )}V^*_3$\\
      $d+e+f \geq a+b+c$ &&$(-d-a-c-e)^{b},(-2d-e-f)^{a+c},0^d $ & \\
      \hline
      
      &$e \leq b$ & $0^b, (a+b+c)^{a+c},(a+c)^{d+f-a-c};$ & $S_{((a+c)^{b+d+f})}V_1 $\\
      &$a \geq d$&$~0^c,(a+b+c)^{e},(a+c+e)^{d};$  & $ \otimes 
      S_{((a+b)^{e},(a+e)^d,(d+e)^c)}V_2$ \\
      && $(-a-c-e)^{b-e},(-d-e-a-c)^{e},$ &$\otimes S_{(-a-c-e)^{b+d},(-d-e-f)^{a+c} )}V^*_3$\\
      &&$(-2d-e-f)^{a+c},0^d$&\\
      \hline
      
      &$e \leq b$ & $0^b, (a+b+c)^{a+c},(a+c)^{d+f-a-c};$ & $S_{((a+c)^{b+d+f})}V_1  $\\
      &$a \leq d$&$~0^c,(a+b+c)^{e},(a+c+e)^{a},(a+e)^{d-a};$  & $\otimes S_{((a+b)^{e},(a+e)^{c+d})}V_2$ \\
      && $(-a-c-e)^{b-e},(-d-e-a-c)^{e},$ & $\otimes  
      S_{(-a-c-e)^{b+d},(-a-e-f)^{c},(-d-e-f)^{a})}V^*_3$\\
      &&$(-a-d-e-f)^{c},(-2d-e-f)^{a},0^d$&\\
      \hline
      $a+c \geq d+f$  & $e \geq b$ & $0^b,(a+b+c)^{f},(d+e+f)^d;$ & $S_{(a+c)^{f},(d+e+f-b)^d,(d+f)^b}V_1$ \\
      $a+b \geq d+e$ & $f \leq c$ & $0^c,(a+b+c)^{d+e};$ & $\otimes S_{(a+b)^{d+e},(d+e)^c}V_2$ \\
      $d+e+f \leq a+b+c$ &  & $(-d-e-f)^{a+b+c-d-e-f},(-2d-e-f)^{d+e+f},0^d$ & $\otimes S_{(-d-e-f)^{a+b+c+d}}V^*_3$ \\
      \hline
      & $e \leq b$ & $0^b,(a+b+c)^{d+f};$ & $S_{(a+c)^{d+f},(d+f)^b}V_1$ \\
      & $f \geq c$ & $0^c,(a+b+c)^{e},(d+e+f)^d$ & $\otimes S_{(a+b)^{e},(d+e+f-c)^d,(d+e)^c}V_2$ \\
      & & $(-d-e-f)^{a+b+c-d-e-f},(-2d-e-f)^{d+e+f},0^d$ & $S_{(-d-e-f)^{a+b+c+d}}V^*_3$ \\
      \hline
      & $e \leq b$ & $0^b,(a+b+c)^f,(a+b+f)^d;$ & $S_{(a+c)^f,(a+f)^{b+d}}V_1$ \\
      & $f \leq c$ & $0^c,(a+b+c)^{e},(c+d+e)^{d}$ & $\otimes S_{(a+b)^{e},(d+e)^{c+d}}V_2$ \\
      & $a \geq d$& $(-d-e-f)^{a+b+c-d-e-f},(-2d-e-f)^{d+e+f},0^d$ & $S_{(-d-e-f)^{a+b+c+d}}V^*_3$  \\
      \hline
      & $e \leq b$ & $0^b,(a+b+c)^f,(a+b+f)^a,(a+f)^{d-a};$ & $S_{(a+c)^f,(a+f)^{b+d}}V_1$ \\
      & $f \leq c$ & $0^c,(a+b+c)^{e},(a+c+e)^{a},(a+e)^{d-a}$ & $\otimes S_{(a+b)^{e},(a+e)^{c+d}}V_2$ \\
      & $a \leq d$& $(-a-e-f)^{b+c-e-f},(-d-e-f-a)^{e+f},(-2d-e-f)^{a},0^d$ & $S_{(-a-e-f)^{b+c+d},(-d-e-f)^{a}}V^*_3$\\
      \hline

      $a+c \leq d+f$  & $a \geq d$ & $0^b,(a+b+c)^{a+c},(a+c)^{d+f-a-c};$ & $S_{(a+c)^{b+d+f}}V_1$ \\
      $a+b \geq d+e$ &  & $0^c,(a+b+c)^{e},(a+c+e)^{d};$ & $\otimes S_{(a+b)^{e},(a+e)^{d},(d+e)^{c}}V_2$ \\
      $d+e+f \leq a+b+c$ &  & $(-a-c-e)^{b-e},(-d-a-c-e)^{e},(-2d-e-f)^{a+c},0^d$ & $\otimes 
      S_{(-a-c-e)^{a+b+c},(-d-e-f)^{d}}V^*_3$ \\
      \hline
      & $a \leq d$ & $0^b,(a+b+c)^f,(a+b+f)^a,(a+f)^{d-a};$ & $S_{(a+c)^f,(a+f)^d,(d+f)^b}V_1$ \\
      & $f \leq c$ & $0^c,(a+b+c)^{e},(a+c+e)^a,(a+e)^{d-a}$ & $\otimes S_{(a+b)^e,(a+e)^{c+d}}V_2$ \\
      & & $(-a-e-f)^{b+c-e-f},(-d-e-f-a)^{e+f},(-2d-e-f)^{a},0^d$ & $S_{(-a-e-f)^{b+c+d},(-d-e-f)^{a}}V^*_3$ \\
      \hline
      & $a \leq d$ & $0^b,(a+b+c)^{a+c},(a+c)^{d+f-a-c};$ & $S_{(a+c)^{b+d+f}}V_1$ \\
      & $f \geq c$ & $0^c,(a+b+c)^{e},(a+c+e)^{a},(a+e)^{d-a}$ & $\otimes S_{(a+b)^{e},(a+e)^{c+d}}V_2$ \\
      & & $(-a-c-e)^{b-e},(-d-a-c-e)^{e},$ & $S_{(-a-c-e)^{b+d},(-a-e-f)^{c},(-d-e-f)^{a}}V^*_3$ \\
      & &$(-d-e-f-a)^{c},(-2d-e-f)^{a},0^d$  &\\
      \hline

      $a+c \geq d+f$  & $a \geq d$ & $0^b,(a+b+c)^{f},(a+b+f)^{d};$ & $S_{(a+c)^{f},(a+f)^d,(d+f)^b}V_1$ \\
      $a+b \leq d+e$ &  & $0^c,(a+b+c)^{a+b},(a+b)^{d+e-a-b};$ & $\otimes S_{(a+b)^{c+d+e}}V_2$ \\
      $d+e+f \leq a+b+c$ &  & $(-a-b-f)^{c-f},(-d-a-b-f)^{f},(-2d-e-f)^{a+b},0^d$ & $\otimes 
      S_{(-a-b-f)^{c+d},(-d-e-f)^{a+b}}V^*_3$ \\
      \hline
      & $a \leq d$ & $0^b,(a+b+c)^f,(a+b+f)^a,(a+f)^{d-a};$ & $S_{(a+c)^f,(a+f)^{b+d}}V_1$ \\
      & $e \leq b$ & $0^c,(a+b+c)^{e},(a+c+e)^a,(a+e)^{d-a}$ & $\otimes S_{(a+b)^e,(a+e)^{c+d}}V_2$ \\
      & & $(-a-e-f)^{b+c-e-f},(-d-e-f-a)^{e+f},(-2d-e-f)^{a},0^d$ & $S_{(-a-e-f)^{b+c+d},(-d-e-f)^{a}}V^*_3$ \\
      \hline
      & $a \leq d$ & $0^b,(a+b+c)^{f},(a+b+f)^a,(a+f)^{d-a};$  & $S_{(a+c)^{f},(a+f)^{b+d}}V_1$ \\
      & $e \geq b$ & $0^c,(a+b+c)^{a+b},(a+b)^{d+e-a-b}$ & $\otimes S_{(a+b)^{c+d+e}}V_2$ \\
      & & $(-a-b-f)^{c-f},(-d-a-b-f)^{f},$ & $S_{(-a-b-f)^{c+d},(-a-e-f)^{b},(-d-e-f)^{a}}V^*_3$ \\
      &&$(-d-e-f-a)^{b},(-2d-e-f)^{a},0^d$  &\\
      \hline

      $a+c \leq d+f$  & $a \geq d$ & $0^b,(a+b+c)^{a+c},(a+c)^{d+f-a-c};$ & $S_{(a+c)^{b+d+f}}V_1$ \\
      $a+b \leq d+e$ & $c \geq b$ & $0^c,(a+b+c)^{a+b},(a+b)^{d+e-a-b};$ & $\otimes S_{(a+b)^{c+d+e}}V_2$ \\
      $d+e+f \geq a+b+c$ &  & $(-2a-b-c)^{b},(-d-a-b-f)^{c-b},(-2d-e-f)^{a+b},0^d$ & $\otimes         
      S_{(-a-b-c)^{d},(-2a-b-c-d)^{b},(-a-b-f)^{c-b},(-d-e-f)^{a+c}}V^*_3$ \\
      \hline
      & $a \geq d$ & $0^b,(a+b+c)^{a+c},(a+c)^{d+f-a-c};$ & $S_{(a+c)^{b+d+f}}V_1$ \\
      & $c \leq b$ & $0^c,(a+b+c)^{a+b},(a+b)^{d+e-a-b};$ & $\otimes S_{(a+b)^{c+d+e}}V_2$ \\
      &  & $(-2a-b-c)^{c},(-d-a-c-e)^{b-c},(-2d-e-f)^{a+b},0^d$ & $\otimes 
      S_{(-a-b-c)^{d},(-2a-b-c-d)^{c},(-a-c-e)^{b-c},(-d-e-f)^{a+c}}V^*_3$ \\
      \hline
      & $a \leq d$ & $0^b,(a+b+c)^f,(a+b+f)^a,(a+f)^{d-a};$ & $S_{(a+c)^f,(a+f)^{b+d}}V_1$ \\
      & $e \leq b$ & $0^c,(a+b+c)^{e},(a+c+e)^a,(a+e)^{d-a}$ & $\otimes S_{(a+b)^e,(a+e)^{c+d}}V_2$ \\
      & & $(-a-e-f)^{b+c-e-f},(-d-e-f-a)^{e+f},(-2d-e-f)^{a},0^d$ & $S_{(-a-e-f)^{b+c+d},(-d-e-f)^{a}}V^*_3$ \\
      \hline
      & $a \leq d$ & $0^b,(a+b+c)^{f},(a+b+f)^a,(a+f)^{d-a};$  & $S_{(a+c)^{f},(a+f)^{b+d}}V_1$ \\
      & $e \geq b$ & $0^c,(a+b+c)^{a+b},(a+b)^{d+e-a-b}$ & $\otimes S_{(a+b)^{c+d+e}}V_2$ \\
      & & $(-a-b-f)^{c-f},(-d-a-b-f)^{f},$ & $S_{(-a-b-f)^{c+d},(-a-e-f)^{b},(-d-e-f)^{a}}V^*_3$ \\
      &&$(-d-e-f-a)^{b},(-2d-e-f)^{a},0^d$  &\\
      \hline

      \caption{$b\neq0,~ c \neq 0,~ d\neq 0$} \label{table3-7}
      \end{longtable} 
      
      
   \begin{center}
    \includegraphics[scale=0.75, clip]{sec3/Gorenstein7.pdf}
   \end{center}
     
\begin{center}
\begin{table}[h]
\caption{Candidates for Gorenstein orbits}  \label{table4}
\begin{tabular}{|c|c|c|c|c|c|}
\hline
$a$  & $b$  & $c$ &  $d$  &  $e$  &  $f$ \\
\hline
$*$  & $*$  & $0$ &  $0$  &  $*$  &  $a$ \\
$0$  & $*$  & $0$ &  $0$  &  $*$  &  $*$ \\
$*$  & $*$  & $0$ &  $0$  &  $*$  &  $0$ \\
%$0$  & $*$  & $0$ &  $0$  &  $*$  &  $0$ \\
\hline
$*$  & $0$  & $*$ &  $0$  &  $a$  &  $*$ \\
$0$  & $0$  & $*$ &  $0$  &  $*$  &  $*$ \\
$*$  & $0$  & $*$ &  $0$  &  $0$  &  $*$ \\
%$0$  & $0$  & $*$ &  $0$  &  $*$  &  $*$ \\
\hline
$d+e+f$  & $0$  & $0$ &  $*$  &  $*$  &  $*$ \\
$*$      & $0$  & $0$ &  $*$  &  $0$  &  $*$ \\
$*$      & $0$  & $0$ &  $*$  &  $*$  &  $0$ \\
\hline
$d+e$  & $0$  & $*$ &  $*$  &  $*$  &  $c$ \\
$d+e$  & $0$  & $*$ &  $*$  &  $*$  &  $0$ \\
$0$  & $0$  & $*$ &  $*$  &  $*$  &  $c$ \\
$*$  & $0$  & $*$ &  $*$  &  $0$  &  $c$ \\
$d$  & $0$  & $*$ &  $*$  &  $0$  &  $0$ \\
%$0$  & $0$  & $*$ &  $*$  &  $0$  &  $c$ \\
\hline
$d+f$  & $*$  & $0$ &  $*$  &  $b$  &  $*$ \\
$d+f$  & $*$  & $0$ &  $*$  &  $0$  &  $*$ \\
$0$  & $*$  & $0$ &  $*$  &  $b$  &  $*$ \\
$*$  & $*$  & $0$ &  $*$  &  $b$  &  $0$ \\
$d$  & $*$  & $0$ &  $*$  &  $0$  &  $0$ \\
%$0$  & $*$  & $0$ &  $*$  &  $b$  &  $0$ \\
\hline
$*$  & $*$  & $*$ &  $0$  &  $a+b$  &  $a+c$ \\
$*$  & $*$  & $*$ &  $0$  &  $b$  &  $c$ \\
$*$  & $*$  & $*$ &  $0$  &  $0$  &  $a+c$ \\
$*$  & $*$  & $*$ &  $0$  &  $a+b$  &  $0$ \\
\hline
$0$  & $*$  & $*$ &  $*$  &  $b$  &  $c$ \\
%$*$  & $*$  & $*$ &  $a$  &  $0$  &  $c$ \\
%$*$  & $*$  & $*$ &  $a$  &  $b$  &  $0$ \\
$*$  & $*$  & $*$ &  $a$  &  $b$  &  $c$ \\
%$0$  & $*$  & $*$ &  $*$  &  $b$  &  $0$ \\
%$0$  & $*$  & $*$ &  $*$  &  $0$  &  $c$ \\
\hline
\end{tabular}
\end{table}
\end{center}
     
\bc{corollary3} For non-equioriented quiver $A_3$, let $V$ be a representation for which all indecomposables occur as summands of $V$ with non-zero multiplicities. The orbit closure $\overline{O_V}$ is Gorenstein iff the Coxeter orbits ($\tau$-orbits of the Auslander-Reiten quiver) are constant. 
\ec
\bpr
Sufficiency follows from Proposition \ref{Prop6}. Necessity follows from Case $7$.
\qed 
\newpage



==> subsec4.tex <==
%-------------------------------------------------------------------------------------------------------------------
\subsection{$F_{top}$ and classification of Gorenstein orbits}
%In this section, we investigate classes of orbit closures that are Gorenstein. For the case of non-equioriented A_3, we also give a description of the last (top) term occuring in the resolution. 
%By \cite{MR1988690}, an orbit closure is Gorenstein if and only if the top module occuring in its resolution is irreducible and 1-dimensional. \par

Lets consider a Dynkin quiver $Q$. The top exterior power of $\xi(a)$ is 
\begin{eqnarray}  S_{[0^{d_1(ta)}, d_1(ha)^{d_2(ta)}, \cdots, (d_1(ha)+\cdots+d_{s-1}(ha))^{d_s(ta)}]}(ta) \\ \nonumber \otimes S_{[(-d_2(ta)-\cdots-d_s(ta))^{d_1(ha)}, \cdots, -d_s(ta)^{d_{s-1}(ha)}, 0^{d_s(ha)}]}(ha)^*\end{eqnarray}
%\[ S_{[0^{d_1(ta)}, d_1(ha)^{d_2(ta)}, \cdots, (d_1(ha)+\cdots+d_{s-1}(ha))^{d_s(ta)}]}(ta) \otimes S_{[(-d_2(ta)-\cdots-d_s(ta))^{d_1(ha)}, \cdots, -d_s(ta)^{d_{s-1}(ha)}, 0^{d_s(ha)}]}(ha) \]
Thus the top exterior power of $\xi$ is given by 
   \begin{equation} \bigwedge^{top} \xi= \bigotimes_{x \in Q_0} S(x)(k_1(x)^{d_1(x)},\cdots,k_s(x)^{d_s(x)} )   
   \label{topterm}
   \end{equation}
where 
   \begin{equation} k_t(x)= \sum_{a \in Q_1; ta=x} \sum_{u<t} d_u(ha)-\sum_{a \in Q_1; ha=x} \sum_{u>t} d_u(ta)
   \end{equation} \par

First, we give a sufficient condition for the orbit closure $\overline{O}_V$ to be Gorenstein in case of any Dynkin quiver $Q$. 
By \cite{MR1988690}, we have that if for every $x \in Q_0$, the number 
   \begin{equation} k_t(x)-\sum_{u<t}d_u(x)+\sum_{u>t}d_u(x) \label{condition}
   \end{equation} 
is independent of $t$, $(t=1,2, \cdots, s)$, then the corresponding orbit closure is Gorenstein.
The following lemma shows that this condition means that the $\tau$-orbits in the Auslander-Reiten quiver are constant- 
\bl{lemma3.4.1} Let $\tau$ denote the Auslander-Reiten translate and suppose $\underline{d}(x)=(d_u(x))_{u=1,2,\cdots, s}$ are dimensions of the flag at vertex $x$ in the desingularization $Z$. Then
\[ \langle \underline{e}_x, \underline{d}_t(x) \rangle = -\langle \underline{d}_{t+1}(x), \underline{e}_x \rangle  \] 
for all $x \in Q_0$ and $t=1,2,\cdots, s-1$, where $\underline{e}_x$ is the dimension vector of the simple representation supported at $x$.
\el 
\bpr (\ref{condition}) translates to the equations- 
   \begin{equation} k_{t+1}(x)-k_t(x)=d_t(x)+d_{t+1}(x)
   \end{equation}
for $x \in Q_0$ and $t=1,2,\cdots, s-1$. This is equivalent to-   
   \begin{equation} \sum_{a \in Q_1;ta=x}d_t(ha)+\sum_{a \in Q_1; ha=x}d_{t+1}(ta)=d_{t+1}(x)+d_t(x)
   \end{equation}
for all $x \in Q_0$ and $t=1,2,\cdots, s-1$. These conditions can be expressed in terms of Euler form as follows-
   \begin{eqnarray} \nonumber
   \langle \underline{e}_x, \underline{d}_t \rangle &=& d_t(x)-\sum_{a \in Q_1;ta=x}d_t(ha) \\ \nonumber
   &=& \sum_{a \in Q_1;ha=x}d_{t+1}(ta)-d_{t+1}(x) \\ \nonumber
   &=& -\langle \underline{d}_{t+1}, \underline{e}_x \rangle
   \end{eqnarray} 
   Thus, 
   \begin{equation} \langle \underline{e}_x, \underline{d}_t \rangle = -\langle \underline{d}_{t+1}, \underline{e}_x
    \rangle \label{euler}
   \end{equation}
where $\underline{e}_x$ is the dimension vector of the simple representation supported at $x$.    \qed   


\bp{Prop3.4.2} Assume that for each $t=1,2, \cdots, s-1$ we have $\underline{d}_{t+1}=\tau^+ \underline{d}_t$. Then the complex $F_{\bullet}$ is self-dual. If the incidence variety comes from Reineke desingularization and the corresponding orbit closure is normal with rational singularities, then it is also Gorenstein. 
\ep
\bpr 
\qed

Next, we investigate necessary conditions for for the orbit closure $\overline{O}_V$ to be Gorenstein in case of non-equioriented $A_3$. 
First we prove that the top exterior power if $\xi$ contributes to the last term of the resolution.

\noindent \textbf{Notation}: We will denote the topmost exterior power of $\xi$ by $\bigwedge^{top} \xi$. %In cases when $\bigwedge^{top} \xi$ does not contribute to $F_{top}$, we denote the maximal contributing exterior power by $\bigwedge^{max} \xi$. \\

\noindent For the case of non-equioriented $A_3$, we investigate the following questions:
\begin{enumerate}
\item In what cases does $\bigwedge^{top}\xi$ contribute? To which term $F_i$ does $\bigwedge^{top}\xi$ contribute?  
\item In cases not covered by $(1)$ what is the $\bigwedge^{max}\xi$ which contributes? Does it contribute to $F_{top}$? 
\end{enumerate}

First we investigate the cases in which $\bigwedge^{top}\xi$ contributes. Observe that a contribution will occur whenever the Bott exchanges give a non-increasing sequence for every term of
\[\bigg( (0^b, (a+b+c)^{d+f}),~~(0^c, (a+b+c)^{d+e}),~((-2d-e-f)^{a+b+c},0^d) \bigg) \]
Also, note that if any of $b,c$ or $d$ are zero, then there are no exchanges for the corresponding term in the weight. We base our cases on this observation.
\bp{Prop3.4.3} $\bigwedge^{top}\xi$ contributes to $F_{top}$ in the following cases when the corresponding conditions are satisfied:
\begin{table}[h]
\centering
      \renewcommand{\arraystretch}{1.3}
\begin{tabular}{|c|ccc|}
\hline
Cases & \multicolumn{3}{|c|}{Conditions}\\
\hline
$b=0, ~c=0, ~d=0$ &   no condition &&      \\
\hline
$b\neq 0, ~c=0, ~d=0$ &  $a+c \geq d+f$ &  &      \\
\hline
$b=0, ~c\neq0, ~d=0$ &  & $a+b \geq d+e$ &  \\
\hline
$b=0,~ c=0,~ d\neq0$ &  &  &$ d+e+f \geq a+b+c  $      \\
\hline
$b=0, ~c\neq0,~ d\neq0$ &  & $a+b \geq d+e$ ,&~ $d+e+f \geq a+b+c$  \\
\hline
$b\neq 0, ~c=0, ~d\neq0$ & $a+c \geq d+f$ ,& & $ d+e+f \geq a+b+c $       \\
\hline
$b\neq 0,~ c\neq0, ~d=0$ &$ a+c \geq d+f$, &~$a+b \geq d+e$ & \\
\hline
$b\neq0,~c\neq0,~d\neq0$ & $a+c \geq d+f $, & ~$a+b \geq d+e $, &~$ d+e+f \geq a+b+c$ \\
\hline
\end{tabular}
\caption{}
\label{table1}
\end{table}
\ep
In each case, we give a description of $F_{top}$. Recall that for our case of non-equioriented $A_3$, we have desingularization-
  \begin{center}
  \includegraphics[scale=0.5, clip]{sec3/desing.pdf}
  \end{center}
As before, let $V=a(0K0)+b(0KK)+c(KK0)+d(KKK)+e(K00)+f(00K)$ be a representation of $A_3$.   
Then \[d_1=(b, ~a+b+c,~ c) ;~~ d_2=(d+f, ~d,~ d+e)\]  
From (\ref{topterm}) the weights for $\bigwedge^{top}\xi$ are:
\[(0^b, (a+b+c)^{d+f}),~~(0^c, (a+b+c)^{d+e}),~((-2d-e-f)^{a+b+c},0^d) \]  
\bl{lemma3} For a weight $(0^b, \lambda;~ 0^c, \mu;-\nu, 0^d)$ of $\bigwedge^{|\lambda|+|\mu|}\xi$, $D(\lambda,\mu)=$ codim $\overline{O}_V$ implies that the partition (if any) arising from $(0^b, \lambda; ~0^c, \mu; -\nu, 0^d)$ corresponds to a summand of $F_{top}$.
\el
\bpr...
\qed \par

Next we show that a contribution from $\bigwedge^{top}\xi$ always goes to $F_{top}$.
\bl{lemma3.4.4} If the weight of the $\bigwedge^{top}\xi$ gives a non-zero partition after Bott exchanges, then the corresponding representation is a $1$ -dimensional summand of $F_{top}$. 
%If $\bigwedge^{top} \xi$ contributes, it always contributes to $F_{top}$. 
\el
\bpr Suppose  
We apply Bott's algorithm to each weight to get:
 \[[0^b, (a+b+c)^{d+f}] = ((a+c)^{d+f}, (d+f)^b) ~\hbox{after}~  b(d+f) ~\hbox{Bott exchanges}\]
 \[[0^c, (a+b+c)^{d+e}] = ((a+b)^{d+e}, (d+e)^c) ~\hbox{after}~ c(d+e) ~\hbox{Bott exchanges}\]
 \[[(-2d-e-f)^{a+b+c},0^d] = ((-a-b-c)^d, (-d-e-f)^{a+b+c}) ~\hbox{after}~ d(a+b+c) ~\hbox{Bott exchanges}\]
 
   \begin{eqnarray} \nonumber
   D(\lambda, \mu)&=&[(d+f)(a+b+c)]+[(d+e)(a+b+c)]\\ \nonumber
   &&-[b(d+f)+c(d+e)+d(a+b+c)] \\ \nonumber
   &=&ad+ae+af+be+cf \\ \nonumber
   &=&\hbox{codim}~ \overline{O}_V 
   \end{eqnarray} 
\qed


In the case $b \neq 0, ~c \neq 0,~ d\neq 0$, if the condition on the right is satisfied, then applying Bott exchanges to 
\[\bigg( (0^b, (a+b+c)^{d+f}),~~(0^c, (a+b+c)^{d+e}),~((-2d-e-f)^{a+b+c},0^d) \bigg) \] gives the partitions -
\[\bigg( ((a+c)^{d+f}, (d+f)^b),~~((a+b)^{d+e}, (d+e)^c),~((-a-b-c)^{d},(-d-e-f)^{a+b+c}) \bigg) \]
If the orbit closure is Gorenstein, then $F_{top}$ is $1$-dimensional. This implies that the above partitions are rectangles, which means 
\[a+c=d+f, ~~a+b=d+e, ~~ a+b+c=d+e+f\]
When  $a \neq 0, ~e \neq 0,~ f\neq 0$, these conditions imply that $a=d, ~b=e$ and $c=f$.
Applying the same logic to each of the above cases, we get necessary conditions for the orbit closure to be Gorenstein. We list these conditions in the following table. \par \vskip0.5cm


%\advance\leftskip-3.5cm
\begin{center}
      \renewcommand{\arraystretch}{1.2}
\begin{longtable}{|c|cc|c|}
 \hline
Cases & \multicolumn{2}{|c|}{$\bigwedge^{top}\xi$ contributes if..}  & $\overline{O}_V$ is  \\
                                   &&& Gorenstein implies... \\ 
\hline 
\endfirsthead
       \hline 
          \multicolumn{1}{|c|}{Cases} &          
          \multicolumn{2}{|c|}{$\bigwedge^{top}\xi$ contributes if..} &
          \multicolumn{1}{|c|}{ $\overline{O}_V$ is Gorenstein implies..} \\
      \hline 
      \endhead
      \hline 
           \multicolumn{4}{|r|}{{Continued on next page}} \\ \hline
      \endfoot
      \endlastfoot
     
\multirow{3}{*}{$b=0, ~c=0, ~d=0$} & $a \neq 0, ~ e\neq 0, ~ f \neq0 $ &always & no condition     \\
                                                          & $a \neq 0, ~ e= 0, ~ f \neq0 $ &always & no condition     \\   
                                                          & $a \neq 0, ~ e\neq 0, ~ f = 0 $ &always & no condition     \\
 \hline
\multirow{4}{*}{$b\neq 0, ~c=0, ~d=0$}  &  $a \neq 0, ~ e\neq 0, ~ f \neq0 $ & $a \geq f$ & $a=f$     \\
                                                                &  $a \neq 0, ~ e= 0, ~ f \neq0 $ & $a \geq f$ & $a=f$     \\
                                                                &  $a \neq 0, ~ e\neq0, ~ f =0 $ & always & no condition     \\
                                                                &  $a = 0, ~ e\neq 0, ~ f =0 $ & always & no condition     \\
\hline

\multirow{4}{*}{$b=0, ~c\neq0, ~d=0$} &  $a \neq 0, ~ e\neq 0, ~ f \neq0 $ & $a \geq e$ & $a=e$     \\
                                                                &  $a \neq 0, ~ e\neq 0, ~ f =0 $ & $a \geq e$ & $a=e$     \\
                                                                &  $a \neq 0, ~ e=0, ~ f \neq0 $ & always & no condition     \\
                                                                &  $a = 0, ~ e = 0, ~ f \neq 0 $ & always & no condition     \\
\hline
\multirow{4}{*}{$b=0,~ c=0,~ d\neq0$ } &  $a \neq 0, ~ e\neq 0, ~ f \neq0 $ & $d+e+f \geq a$ & $d+e+f=a$     \\
                                                                &  $a \neq 0, ~ e\neq 0, ~ f =0 $ & $d+e \geq a$ & $d+e=a$     \\
                                                                &  $a \neq 0, ~ e=0, ~ f \neq0 $ & $d+f \geq a$ & $d+f=a$     \\
                                                                &  $a \neq 0, ~ e = 0, ~ f = 0 $ & $d \geq a$ & $d=a$   \\
\hline

\multirow{3}{*}{$b=0, ~c\neq0,~ d\neq0$}   & $a \neq 0, ~e \neq 0,~ f\neq 0$ & $a \geq d+e, ~ d+e+f \geq a+c$ & $a=d+e, ~c=f$ \\
                                                                   & $a = 0, ~e \neq 0,~ f\neq 0$ & $f \geq c$ & $c=f$     \\
                                                                   &  $a \neq 0, ~e = 0,~ f \neq 0$ & $a \geq d,~d+f \geq a+c$ & $a=d, ~c=f$    \\
                                                                   
\hline
\multirow{3}{*}{$b\neq 0, ~c=0, ~d\neq0$} & $a \neq 0, ~e \neq 0,~ f\neq 0$ & $a \geq d+f, ~ d+e+f \geq a+b$ & $a=d+f, ~b=e$ \\
                                                                   & $a = 0, ~e \neq 0,~ f\neq 0$ & $e \geq b$ & $b=e$     \\
                                                                   &  $a \neq 0, ~e \neq 0,~ f= 0$ & $a \geq d,~d+e \geq a+b$ & $a=d, ~b=e$    \\
                                                                   
\hline

\multirow{6}{*}{$b\neq 0,~ c\neq0, ~d=0$ }&  $a \neq 0, ~ e\neq 0, ~ f \neq0 $ & $a+b\geq e,~a+c \geq f$ & $a+b=e, ~a+c=f$  \\
                                                                   &  $a =0, ~ e\neq 0, ~ f \neq0 $ & $ b \geq e,~ c \geq f$ & $b=e,~c=f$     \\
                                                                   &  $a \neq 0, ~ e= 0, ~ f \neq0 $ & $a+c \geq f$ & $a+c=f$      \\
                                                                   &  $a \neq 0, ~ e\neq 0, ~ f =0 $ & $a+b\geq e$ & $a+b=e$      \\
                                                                   &  $a = 0, ~ e = 0, ~ f \neq0 $ & $c\geq f$ & $c=f$      \\
                                                                   &  $a = 0, ~ e\neq 0, ~ f =0 $ & $b\geq e$ & $b=e$      \\
\hline
$b\neq0,~c\neq0,~d\neq0$ &  $a \neq 0, ~e \neq 0,~ f\neq 0$ &  $a+c \geq d+f $, ~$a+b \geq d+e $,&  $a=d, ~b=e, ~c=f$   \\
             &&             ~$ d+e+f  \geq a+b+c$ &\\
\hline 

\caption{Cases} \label{table2}
\end{longtable}
\end{center}

\vskip1cm

Now we consider what happens if the conditions on the right are not satisfied in the cases listed in Proposition \ref{Prop4}. In this event, the top exterior power $\bigwedge^{top}\xi$ does not contribute any term to $F_{top}$. For each case, we obtain a description of the term that does contribute to $F_{top}$ (we denote the corresponding exterior power by $\bigwedge^{max}\xi$) and state the necessary condition for the orbit closure to be Gorenstein. \par

\noindent \textbf{Case 1:} $b\neq 0, ~c=0, ~d=0$ - in this case dim $\xi = (a+b)(e+f)$ and codim $\overline{O}_V = ae+af+be$. \par If $a \neq  
   0, ~ e \neq 0, ~f \neq 0$, the weight in $\bigwedge^{top}\xi$ is of the form
   \[ \big( 0^b,(a+b)^f ;~ (a+b)^e ;~(-e-f)^{a+b} \big) \] 
   If $a \geq f$, the above term gives the summand $S_{(a^f,f^b)}V_1 \otimes S_{(a+b)^e}V_2 \otimes S_{(e+f)^{a+b}}V^*_3$ of 
   $F_{top}$ (as noted in Proposition \ref{Prop4}). However, if $a \leq f$, the above term contributes nothing. In this case, it follows from 
   Remark \ref{} that $\bigwedge^{max}\xi$ has a weight of the form  \[ \big( 0^b,(a+b)^k,k^{f-k} ;~(a+b)^e 
   ; - \nu  \big) \] where $k < f$. By Lemma \ref{lemma3} this weight must satisfy the condition $D(\lambda,\mu) = ae+af+be$. Substitution   
   gives
   \begin{eqnarray} \nonumber
   k(a+b+f-k)+(a+b)e-bk&=&ae+af+be \\ \nonumber
   i.e. ~~k^2-k(a+f)+af&=&0   
   \end{eqnarray}  This implies $k=a$ (since $k<f$). So the weight for $\bigwedge^{max}\xi$ is  \[ \big(  
   0^b,(a+b)^a,a^{f-a};~ (a+b)^e ; ~(-a-e)^b,(-e-f)^a  \big) \]  Using this weight it is easy to derive the corresponding weights for remaining 
    cases in the following table  
      \vskip0.5cm
 
      \renewcommand{\arraystretch}{1.5}
      \begin{longtable}[c]{|p{0.08cm}p{0.08cm}p{0.08cm}|p{2cm}|p{6.1cm}|p{6.5cm}|}     
      \hline
      $a$ & $e$ & $f$ &Condition & Weight of $\bigwedge^{max}\xi$& Corresponding summand in $F_{top}$ \\
                                        
      \hline
      \endfirsthead
       \hline 
          \multicolumn{1}{|c}{$a$} &
          \multicolumn{1}{c}{$e$} &
          \multicolumn{1}{c|}{$f$} &
          \multicolumn{1}{|c|}{Condition} &
          \multicolumn{1}{|c|}{Weight of $\wedge^{max}\xi$ }&
          \multicolumn{1}{|c|}{Corresponding summand in  $F_{top}$}\\  
      \hline 
      \endhead
      \hline 
           \multicolumn{6}{|r|}{{Continued on next page}} \\ \hline
      \endfoot
      \endlastfoot

      $*$ & $*$ & $*$ & $a < f$&$\big(0^b, (a+b)^a, a^{f-a};~(a+b)^e;$ &  
      $S_{(a^{b+f})}V_1 \otimes S_{((a+b)^e)}V_2 $\\
      &&&&$(-a-e)^b,(-e-f)^{a} \big)$& $\otimes S_{((-e-a)^b,(-e-f)^{a})}V^*_3$ \\
      \hline
      $0$ & $*$ & $*$ & $a < f$ & $\big( 0^{b+f};~b^e;~-e^b  \big)$ &$S_{(b^e)}V_2 \otimes 
      S_{(-e^b)}V^*_3$ \\
      \hline
      $*$ & $0$ & $*$ & $a < f$ & $\big( 0^b, (a+b)^a,a^{f-a}; ~\phi ;~-a^b,-f^a  \big)$ &$S_{(a^{b+d+f})}V_1 
       \otimes S_{(-a^b,-f^a)}V^*_3$ \\
      \hline
      $*$ & $*$ & $0$ & \multicolumn{2}{|c|}{in this case $\wedge^{top}\xi$ contributes}&$S_{((a+b)^e)}V_2 \otimes 
      S_{(e^{a+b})}V^*_3$  \\
      \hline
      $0$ & $0$ & $*$ & \multicolumn{2}{|c|}{in this case codim $\overline{O}_V = 0$  }& $0$  \\
      \hline
      $0$ & $*$ & $0$ & \multicolumn{2}{|c|}{in this case $\wedge^{top}\xi$ contributes}&$S_{(b^e)}V_2 \otimes 
      S_{(e^b)}V^*_3$ 
      \\
      \hline
      $*$ & $0$ & $0$ & \multicolumn{3}{|c|}{in this case dim $\xi = 0$ } \\
      \hline
      \caption{$b\neq 0, ~c=0, ~d=0$}\label{table3-1}
      \end{longtable}


\vskip1cm
From Table \ref{table2} and Table \ref{table3-1} we can list the candidates for Gorenstein orbits in terms of conditions on multiplicities of indecomposables. We express these orbits in the shape of the AR quiver for easy reading:
\vskip1cm
   \begin{center}
    \includegraphics[scale=0.75, clip]{sec3/Gorenstein1.pdf}
   \end{center}
\vskip0.7cm
  
  
 
We repeat this procedure for the remaining 6 cases. We state only the sub-case $a \neq 0, e\neq 0, f \neq 0$ each time (the remaining subcases can be derived from the above) and the possible candidates for Gorenstein orbits. \par
\newpage
\noindent \textbf{Case 2:} $b=0, ~c\neq0, ~d=0$ 
  
      \renewcommand{\arraystretch}{1.5}
      \begin{table}[h]
      \begin{tabular}{|c|c|c|}     
      \hline
      Condition & Weight of $\wedge^{max}\xi$  & Summand in $F_{top}$ \\
                      
      \hline

      $a \leq f$& $\big( (a+b)^f;~~0^c,(a+c)^a,a^{e-a};~~(-a-f)^c,(-e-f)^{a} \big)$ &  $S_{((a+b)^f)}V_1 \otimes 
      S_{(a^{c+e})}V_2 $\\
       && $\otimes S_{((-a-f)^c,(-e-f)^{a})}V^*_3$ \\
      \hline
     
      \end{tabular} \caption{ $b=0, ~c\neq0, ~d=0$} \label{table3-2}
      \end{table}

   
   \begin{center}
    \includegraphics[scale=0.75, clip]{sec3/Gorenstein2.pdf}
   \end{center}
 \vskip2cm
  
   \noindent \textbf{Case 3:} $b=0,~ c=0,~ d\neq0$ \vskip0.5cm
      \renewcommand{\arraystretch}{1.5}
      \begin{table}[h]
      \begin{tabular}{|c|c|c|}     
      \hline
      Condition & Weight of $\wedge^{max}\xi$  & Summand in $F_{top}$ \\
                      
      \hline
     $d+e+f \leq a$ & $\big( a^{d+f};~ a^{e},(d+e+f)^d;$&  $S_{(a^{d+f})}V_1                
        \otimes S_{(a^{e},(d+e+f)^d)}V_2 $\\
      &$(-d-e-f)^{a-d-e-f},(-2d-e-f)^{d+e+f}, 0^d \big)$ & $\otimes S_{(-d-e-f^a)}V^*_3$ \\

      \hline
     
      \end{tabular} \caption{$b=0,~ c=0,~ d\neq0$} \label{table3-3}
      \end{table}
    
   \begin{center}
    \includegraphics[scale=0.75, clip]{sec3/Gorenstein3.pdf}
   \end{center}      

\newpage
\noindent \textbf{Case 4:} $b=0,~ c\neq 0,~ d\neq0$ \vskip0.5cm
  
      \renewcommand{\arraystretch}{1.5}
      \begin{table}[h]
      \begin{tabular}{|c|c|c|c|} 
    
      \hline
      Condition& cases & Weight of $\wedge^{max}\xi$  & Summand in $F_{top}$ \\
                      
      \hline
       $a \leq d+e,$ & $f \geq c$ & $\big(~(a+c)^{d+f};0^b, (a+c)^a,a^{d+e-a};$ & $S_{((a+c)^{d+f})}V_1 \otimes 
                                                                               S_{(a^{c+d+e})}V_2 $\\
       $ d+e+f \geq a+c$ &&$(-d-f-a)^{c},(-2d-e-f)^{a}, 0^d \big)$& $\otimes S_{((-a-c)^d,(-a-f)^c,(-d-e-f)^a)}V^*_3$ \\
      
      \hline
      &$f \leq c$ &$\big(~(a+c)^{d+f};0^c, (a+c)^a,a^{d+e-a};$ & $S_{((a+c)^{d+f})}V_1\otimes S_{(a^{c+d+e})}V_2 $\\
      &&$(-d-f-a)^{c},(-2d-e-f)^{a}, 0^d \big)$& $ \otimes S_{((-a-c)^d,(-a-f)^c,(-d-e-f)^a)}V^*_3$ \\
      
      \hline
      
      $a \geq d+e$& $f \geq c$ &$\big(~(a+c)^{d+f};0^c, (a+c)^e,(d+e+f)^d;$ & $S_{((a+c)^{d+f})}V_1  $\\
      $d+e+f \leq a+c$ &&$(-d-e-f)^{a+c-d-e-f},(-2d-e-f)^{d+e+f},0^d \big)$& $\otimes 
      S_{(a^e,(d+e+f-c)^d,(d+e)^c)}V_2$ \\
      &&&$\otimes S_{((-d-e-f)^{a+c+d})}V^*_3$\\
      \hline
      & $f \leq c$ &$\big(~(a+c)^{f},(d+e+f)^d;0^c, (a+c)^{d+e};$ & $S_{((a+c)^f,(d+e+f)^d)}V_1 $\\
      &&$(-d-e-f)^{a+c-d-e-f},(-2d-e-f)^{d+e+f}, 0^d \big)$& $\otimes  S_{(a^{d+e},(d+e)^c)}V_2$ \\
      &&&$\otimes S_{((-d-e-f)^{a+c+d})}V^*_3$\\
      \hline
       $a \leq d+e$& $f\leq c$ &$\big(~(a+c)^{f},(a+f)^d;0^c, (a+c)^a,(d+e-a)^d;$ & $S_{((a+c)^{f},(a+f)^d)}V_1 \otimes 
       S_{(a^{c+d+e})}V_2 $\\

      $d+e+f \leq a+c$ &&$(-a-f)^{c-f},(-d-f-a)^{f},(-2d-e-f)^{a},0^d \big)$&$\otimes(-a-f)^{c+d},(-d-e-f)^{a})}V^*_3$ \\
     
      \hline
      \end{tabular} \caption{$b=0,~ c\neq 0,~ d\neq0$} \label{table3-4}
      \end{table}

      
   \begin{center}
    \includegraphics[scale=0.75, clip]{sec3/Gorenstein4.pdf}
   \end{center} 
        
\newpage
\noindent \textbf{Case 5:} $b\neq0,~ c = 0,~ d\neq0$ \par
      \begin{center}
      \renewcommand{\arraystretch}{1.5}
      \begin{table}[h]
      \begin{tabular}{|c|c|c|c|}     
      \hline
      Condition& cases & Weight of $\wedge^{max}\xi$  & Summand in $F_{top}$ \\
                      
      \hline
      $a \leq d+f,$& $e \geq b$ & $\big(0^b, (a+b)^a,a^{d+f-a};~(a+b)^{d+e};$ & $S_{(a^{b+d+f})}V_1 \otimes   
       S_{((a+b)^{d+e})}V_2 $\\
       $ d+e+f \geq a+b$ &&$(-d-e-a)^{b},(-2d-e-f)^{a}, 0^d \big)$& $\otimes S_{((-a-b)^d,(-a-e)^b,(-d-e-f)^a)}V^*_3$ \\
      \hline

      & $e \leq b$ &$\big(0^b, (a+b)^a,a^{d+f-a};~(a+b)^{d+e};$ & $S_{(a^{b+d+f})}V_1 \otimes  
       S_{((a+b)^{d+e})}V_2 $\\
       &&$(-d-e-a)^{b},(-2d-e-f)^{a}, 0^d \big)$& $\otimes S_{((-a-b)^d,(-a-e)^b,(-d-e-f)^a)}V^*_3$ \\
       \hline
       
       $a \geq d+f$& $e \geq b$ &$\big(0^b, (a+b)^f,(d+e+f)^d;~(a+b)^{d+e};$ & $S_{(a^f,(d+e+f-b)^d,(d+f)^b)}V_1 $\\
       $d+e+f < a+b$ &&$(-d-e-f)^{a+b-d-e-f},(-2d-e-f)^{d+e+f},0^d \big)$& $\otimes S_{((a+b)^{d+e})}V_2$ \\
       &&&$\otimes S_{((-d-e-f)^{a+b+d})}V^*_3$\\
       \hline
       & $e \leq b$ &$\big(0^b, (a+b)^{d+f};~(a+b)^{e},(d+e+f)^d;$ & $S_{(a^{d+f},(d+f)^b)}V_1 $\\
       &&$(-d-e-f)^{a+b-d-e-f},(-2d-e-f)^{d+e+f}, 0^d \big)$& $\otimes S_{((a+b)^e,(d+e+f)^d)}V_2 $ \\
       &&&$\otimes  S_{((-d-e-f)^{a+b+d})}V^*_3$\\

       \hline
        $a \leq d+f$& $e \leq b$ &$\big(0^b, (a+b)^a,(d+f-a)^d;~(a+b)^{e},(a+e)^d;$ &  $S_{(a^{b+d+f})}V_1 \otimes 
        S_{((a+b)^{e}, (a+e)^d)}V_2 $\\
       $d+e+f \leq a+b$ &&$(-a-e)^{b-e},(-d-e-a)^{e},(-2d-e-f)^{a},0^d \big)$& $\otimes 
       S_{((-a-e)^{b+d},(-d-e-f)^{a})}V^*_3$ \\
     
      \hline
     
      \end{tabular} \caption{ $b\neq0,~ c = 0,~ d\neq0$} \label{table3-5}
      \end{table}
      \end{center}
      
   \begin{center}
    \includegraphics[scale=0.75, clip]{sec3/Gorenstein5.pdf}
   \end{center}    
     
\newpage
\noindent \textbf{Case 6:} $b\neq0,~ c \neq 0,~ d=0$ \par
      
      \renewcommand{\arraystretch}{1.5}
      \begin{table}[h]
      \begin{tabular}{|c|c|c|c|}     
      \hline
      Condition& cases & Weight of $\wedge^{max}\xi$  & Summand in $F_{top}$ \\
                      
      \hline
      $a+c \leq f$, && $0^b, (a+b+c)^{a+c},(a+c)^{f-a-c};$ & $S_{((a+c)^{b+f})}V_1 \otimes S_{((a+b)^{e},e^c)}V_2 $\\ 
       
      $a+b \geq e$ && $~0^c,(a+b+c)^{e};$ & $\otimes S_{(-a-c-e)^{b},(-e-f)^{a+c} )}V^*_3$\\
      &&$(-a-c-e)^{b},(-e-f)^{a+c} $ & \\
      \hline
      $a+c \geq f$,  && $0^b, (a+b+c)^f;$ & $S_{((a+c)^{f},f^b)}V_1 \otimes S_{((a+b)^{c+e})}V_2 $\\
      $ a+b \leq e$ &&$~0^c,(a+b+c)^{a+b},(a+b)^{e-a-b};$  & $\otimes S_{(-a-b-f)^{c},(-e-f)^{a+b} )}V^*_3$ \\
      && $(-a-b-f)^{c},(-e-f)^{a+b}$ &\\
      \hline
      $a+c \leq f,$ & $c \geq b$ & $ 0^b, (a+b+c)^{a+c},(a+c)^{f-a-c};$ &  
                                                 $S_{((a+c)^{b+f})}V_1 \otimes S_{((a+b)^{e},e^c)}V_2 $\\
      $ a+b \leq e$ &&$ 0^c,(a+b+c)^{a+b},(a+b)^{e-a-b};$& $\otimes 
      S_{((-2a-b-c)^{b},(-a-b-f)^{c-b},(-e-f)^{a+b} )}V^*_3$ \\
      &&$(-2a-b-c)^{b},(-a-b-f)^{c-b},(-e-f)^{a+b} $&\\
      \hline
      &$c \leq b$ & $ 0^b, (a+b+c)^{a+c},(a+c)^{f-a-c};$ & $S_{((a+c)^{b+f})}V_1 \otimes 
                                                                               S_{((a+b)^{e},e^c)}V_2 $\\
       & & $~0^c,(a+b+c)^{a+b},(a+b)^{e-a-b}; $& $\otimes 
      S_{((-2a-b-c)^{b},(-a-c-e)^{b-c},(-e-f)^{a+b} )}V^*_3$ \\ 
      & & $(-2a-b-c)^{b},(-a-c-e)^{b-c},(-e-f)^{a+b} $& \\ \hline
      \end{tabular} \caption{$b\neq0,~ c \neq 0,~ d=0$} \label{table3-6}
      \end{table}
      
   \begin{center}
    \includegraphics[scale=0.75, clip]{sec3/Gorenstein6.pdf}
   \end{center}      
 
\newpage      
\noindent \textbf{Case 7:} $b\neq0,~ c \neq 0,~ d \neq 0$ \par
      
      \renewcommand{\arraystretch}{1.5}
     
      \begin{longtable}{|c|c|c|c|}     
      \hline
      Condition& cases & Weight of $\wedge^{max}\xi$  & Summand in $F_{top}$ \\
      \hline
\endfirsthead
       \hline 
          \multicolumn{1}{|c|}{Condition} &
          \multicolumn{1}{|c|}{cases} &
          \multicolumn{1}{|c|}{Weight of $\wedge^{max}\xi$ }&
          \multicolumn{1}{|c|}{Summand in $F_{top}$}\\  
      \hline 
      \endhead
      \hline 
           \multicolumn{4}{|r|}{{Continued on next page}} \\ \hline
      \endfoot
      \endlastfoot 
      
                      
   
      $a+c \leq d+f$ & $e \geq b$& $0^b, (a+b+c)^{a+c},(a+c)^{d+f-a-c};$ & $S_{((a+c)^{b+d+f})}V_1 \otimes 
      S_{((a+b)^{d+e},(d+e)^c)}V_2 $\\ 
      $a+b \geq d+e$ && $~0^c,(a+b+c)^{d+e};$ & $\otimes S_{(-a-b-c)^d,(-a-c-e)^{b},(-d-e-f)^{a+c} )}V^*_3$\\
      $d+e+f \geq a+b+c$ &&$(-d-a-c-e)^{b},(-2d-e-f)^{a+c},0^d $ & \\
      \hline
      
      &$e \leq b$ & $0^b, (a+b+c)^{a+c},(a+c)^{d+f-a-c};$ & $S_{((a+c)^{b+d+f})}V_1 $\\
      &$a \geq d$&$~0^c,(a+b+c)^{e},(a+c+e)^{d};$  & $ \otimes 
      S_{((a+b)^{e},(a+e)^d,(d+e)^c)}V_2$ \\
      && $(-a-c-e)^{b-e},(-d-e-a-c)^{e},$ &$\otimes S_{(-a-c-e)^{b+d},(-d-e-f)^{a+c} )}V^*_3$\\
      &&$(-2d-e-f)^{a+c},0^d$&\\
      \hline
      
      &$e \leq b$ & $0^b, (a+b+c)^{a+c},(a+c)^{d+f-a-c};$ & $S_{((a+c)^{b+d+f})}V_1  $\\
      &$a \leq d$&$~0^c,(a+b+c)^{e},(a+c+e)^{a},(a+e)^{d-a};$  & $\otimes S_{((a+b)^{e},(a+e)^{c+d})}V_2$ \\
      && $(-a-c-e)^{b-e},(-d-e-a-c)^{e},$ & $\otimes  
      S_{(-a-c-e)^{b+d},(-a-e-f)^{c},(-d-e-f)^{a})}V^*_3$\\
      &&$(-a-d-e-f)^{c},(-2d-e-f)^{a},0^d$&\\
      \hline
      $a+c \geq d+f$  & $e \geq b$ & $0^b,(a+b+c)^{f},(d+e+f)^d;$ & $S_{(a+c)^{f},(d+e+f-b)^d,(d+f)^b}V_1$ \\
      $a+b \geq d+e$ & $f \leq c$ & $0^c,(a+b+c)^{d+e};$ & $\otimes S_{(a+b)^{d+e},(d+e)^c}V_2$ \\
      $d+e+f \leq a+b+c$ &  & $(-d-e-f)^{a+b+c-d-e-f},(-2d-e-f)^{d+e+f},0^d$ & $\otimes S_{(-d-e-f)^{a+b+c+d}}V^*_3$ \\
      \hline
      & $e \leq b$ & $0^b,(a+b+c)^{d+f};$ & $S_{(a+c)^{d+f},(d+f)^b}V_1$ \\
      & $f \geq c$ & $0^c,(a+b+c)^{e},(d+e+f)^d$ & $\otimes S_{(a+b)^{e},(d+e+f-c)^d,(d+e)^c}V_2$ \\
      & & $(-d-e-f)^{a+b+c-d-e-f},(-2d-e-f)^{d+e+f},0^d$ & $S_{(-d-e-f)^{a+b+c+d}}V^*_3$ \\
      \hline
      & $e \leq b$ & $0^b,(a+b+c)^f,(a+b+f)^d;$ & $S_{(a+c)^f,(a+f)^{b+d}}V_1$ \\
      & $f \leq c$ & $0^c,(a+b+c)^{e},(c+d+e)^{d}$ & $\otimes S_{(a+b)^{e},(d+e)^{c+d}}V_2$ \\
      & $a \geq d$& $(-d-e-f)^{a+b+c-d-e-f},(-2d-e-f)^{d+e+f},0^d$ & $S_{(-d-e-f)^{a+b+c+d}}V^*_3$  \\
      \hline
      & $e \leq b$ & $0^b,(a+b+c)^f,(a+b+f)^a,(a+f)^{d-a};$ & $S_{(a+c)^f,(a+f)^{b+d}}V_1$ \\
      & $f \leq c$ & $0^c,(a+b+c)^{e},(a+c+e)^{a},(a+e)^{d-a}$ & $\otimes S_{(a+b)^{e},(a+e)^{c+d}}V_2$ \\
      & $a \leq d$& $(-a-e-f)^{b+c-e-f},(-d-e-f-a)^{e+f},(-2d-e-f)^{a},0^d$ & $S_{(-a-e-f)^{b+c+d},(-d-e-f)^{a}}V^*_3$\\
      \hline

      $a+c \leq d+f$  & $a \geq d$ & $0^b,(a+b+c)^{a+c},(a+c)^{d+f-a-c};$ & $S_{(a+c)^{b+d+f}}V_1$ \\
      $a+b \geq d+e$ &  & $0^c,(a+b+c)^{e},(a+c+e)^{d};$ & $\otimes S_{(a+b)^{e},(a+e)^{d},(d+e)^{c}}V_2$ \\
      $d+e+f \leq a+b+c$ &  & $(-a-c-e)^{b-e},(-d-a-c-e)^{e},(-2d-e-f)^{a+c},0^d$ & $\otimes 
      S_{(-a-c-e)^{a+b+c},(-d-e-f)^{d}}V^*_3$ \\
      \hline
      & $a \leq d$ & $0^b,(a+b+c)^f,(a+b+f)^a,(a+f)^{d-a};$ & $S_{(a+c)^f,(a+f)^d,(d+f)^b}V_1$ \\
      & $f \leq c$ & $0^c,(a+b+c)^{e},(a+c+e)^a,(a+e)^{d-a}$ & $\otimes S_{(a+b)^e,(a+e)^{c+d}}V_2$ \\
      & & $(-a-e-f)^{b+c-e-f},(-d-e-f-a)^{e+f},(-2d-e-f)^{a},0^d$ & $S_{(-a-e-f)^{b+c+d},(-d-e-f)^{a}}V^*_3$ \\
      \hline
      & $a \leq d$ & $0^b,(a+b+c)^{a+c},(a+c)^{d+f-a-c};$ & $S_{(a+c)^{b+d+f}}V_1$ \\
      & $f \geq c$ & $0^c,(a+b+c)^{e},(a+c+e)^{a},(a+e)^{d-a}$ & $\otimes S_{(a+b)^{e},(a+e)^{c+d}}V_2$ \\
      & & $(-a-c-e)^{b-e},(-d-a-c-e)^{e},$ & $S_{(-a-c-e)^{b+d},(-a-e-f)^{c},(-d-e-f)^{a}}V^*_3$ \\
      & &$(-d-e-f-a)^{c},(-2d-e-f)^{a},0^d$  &\\
      \hline

      $a+c \geq d+f$  & $a \geq d$ & $0^b,(a+b+c)^{f},(a+b+f)^{d};$ & $S_{(a+c)^{f},(a+f)^d,(d+f)^b}V_1$ \\
      $a+b \leq d+e$ &  & $0^c,(a+b+c)^{a+b},(a+b)^{d+e-a-b};$ & $\otimes S_{(a+b)^{c+d+e}}V_2$ \\
      $d+e+f \leq a+b+c$ &  & $(-a-b-f)^{c-f},(-d-a-b-f)^{f},(-2d-e-f)^{a+b},0^d$ & $\otimes 
      S_{(-a-b-f)^{c+d},(-d-e-f)^{a+b}}V^*_3$ \\
      \hline
      & $a \leq d$ & $0^b,(a+b+c)^f,(a+b+f)^a,(a+f)^{d-a};$ & $S_{(a+c)^f,(a+f)^{b+d}}V_1$ \\
      & $e \leq b$ & $0^c,(a+b+c)^{e},(a+c+e)^a,(a+e)^{d-a}$ & $\otimes S_{(a+b)^e,(a+e)^{c+d}}V_2$ \\
      & & $(-a-e-f)^{b+c-e-f},(-d-e-f-a)^{e+f},(-2d-e-f)^{a},0^d$ & $S_{(-a-e-f)^{b+c+d},(-d-e-f)^{a}}V^*_3$ \\
      \hline
      & $a \leq d$ & $0^b,(a+b+c)^{f},(a+b+f)^a,(a+f)^{d-a};$  & $S_{(a+c)^{f},(a+f)^{b+d}}V_1$ \\
      & $e \geq b$ & $0^c,(a+b+c)^{a+b},(a+b)^{d+e-a-b}$ & $\otimes S_{(a+b)^{c+d+e}}V_2$ \\
      & & $(-a-b-f)^{c-f},(-d-a-b-f)^{f},$ & $S_{(-a-b-f)^{c+d},(-a-e-f)^{b},(-d-e-f)^{a}}V^*_3$ \\
      &&$(-d-e-f-a)^{b},(-2d-e-f)^{a},0^d$  &\\
      \hline

      $a+c \leq d+f$  & $a \geq d$ & $0^b,(a+b+c)^{a+c},(a+c)^{d+f-a-c};$ & $S_{(a+c)^{b+d+f}}V_1$ \\
      $a+b \leq d+e$ & $c \geq b$ & $0^c,(a+b+c)^{a+b},(a+b)^{d+e-a-b};$ & $\otimes S_{(a+b)^{c+d+e}}V_2$ \\
      $d+e+f \geq a+b+c$ &  & $(-2a-b-c)^{b},(-d-a-b-f)^{c-b},(-2d-e-f)^{a+b},0^d$ & $\otimes         
      S_{(-a-b-c)^{d},(-2a-b-c-d)^{b},(-a-b-f)^{c-b},(-d-e-f)^{a+c}}V^*_3$ \\
      \hline
      & $a \geq d$ & $0^b,(a+b+c)^{a+c},(a+c)^{d+f-a-c};$ & $S_{(a+c)^{b+d+f}}V_1$ \\
      & $c \leq b$ & $0^c,(a+b+c)^{a+b},(a+b)^{d+e-a-b};$ & $\otimes S_{(a+b)^{c+d+e}}V_2$ \\
      &  & $(-2a-b-c)^{c},(-d-a-c-e)^{b-c},(-2d-e-f)^{a+b},0^d$ & $\otimes 
      S_{(-a-b-c)^{d},(-2a-b-c-d)^{c},(-a-c-e)^{b-c},(-d-e-f)^{a+c}}V^*_3$ \\
      \hline
      & $a \leq d$ & $0^b,(a+b+c)^f,(a+b+f)^a,(a+f)^{d-a};$ & $S_{(a+c)^f,(a+f)^{b+d}}V_1$ \\
      & $e \leq b$ & $0^c,(a+b+c)^{e},(a+c+e)^a,(a+e)^{d-a}$ & $\otimes S_{(a+b)^e,(a+e)^{c+d}}V_2$ \\
      & & $(-a-e-f)^{b+c-e-f},(-d-e-f-a)^{e+f},(-2d-e-f)^{a},0^d$ & $S_{(-a-e-f)^{b+c+d},(-d-e-f)^{a}}V^*_3$ \\
      \hline
      & $a \leq d$ & $0^b,(a+b+c)^{f},(a+b+f)^a,(a+f)^{d-a};$  & $S_{(a+c)^{f},(a+f)^{b+d}}V_1$ \\
      & $e \geq b$ & $0^c,(a+b+c)^{a+b},(a+b)^{d+e-a-b}$ & $\otimes S_{(a+b)^{c+d+e}}V_2$ \\
      & & $(-a-b-f)^{c-f},(-d-a-b-f)^{f},$ & $S_{(-a-b-f)^{c+d},(-a-e-f)^{b},(-d-e-f)^{a}}V^*_3$ \\
      &&$(-d-e-f-a)^{b},(-2d-e-f)^{a},0^d$  &\\
      \hline

      \caption{$b\neq0,~ c \neq 0,~ d\neq 0$} \label{table3-7}
      \end{longtable} 
      
      
   \begin{center}
    \includegraphics[scale=0.75, clip]{sec3/Gorenstein7.pdf}
   \end{center}
     
\begin{center}
\begin{table}[h]
\caption{Candidates for Gorenstein orbits}  \label{table4}
\begin{tabular}{|c|c|c|c|c|c|}
\hline
$a$  & $b$  & $c$ &  $d$  &  $e$  &  $f$ \\
\hline
$*$  & $*$  & $0$ &  $0$  &  $*$  &  $a$ \\
$0$  & $*$  & $0$ &  $0$  &  $*$  &  $*$ \\
$*$  & $*$  & $0$ &  $0$  &  $*$  &  $0$ \\
%$0$  & $*$  & $0$ &  $0$  &  $*$  &  $0$ \\
\hline
$*$  & $0$  & $*$ &  $0$  &  $a$  &  $*$ \\
$0$  & $0$  & $*$ &  $0$  &  $*$  &  $*$ \\
$*$  & $0$  & $*$ &  $0$  &  $0$  &  $*$ \\
%$0$  & $0$  & $*$ &  $0$  &  $*$  &  $*$ \\
\hline
$d+e+f$  & $0$  & $0$ &  $*$  &  $*$  &  $*$ \\
$*$      & $0$  & $0$ &  $*$  &  $0$  &  $*$ \\
$*$      & $0$  & $0$ &  $*$  &  $*$  &  $0$ \\
\hline
$d+e$  & $0$  & $*$ &  $*$  &  $*$  &  $c$ \\
$d+e$  & $0$  & $*$ &  $*$  &  $*$  &  $0$ \\
$0$  & $0$  & $*$ &  $*$  &  $*$  &  $c$ \\
$*$  & $0$  & $*$ &  $*$  &  $0$  &  $c$ \\
$d$  & $0$  & $*$ &  $*$  &  $0$  &  $0$ \\
%$0$  & $0$  & $*$ &  $*$  &  $0$  &  $c$ \\
\hline
$d+f$  & $*$  & $0$ &  $*$  &  $b$  &  $*$ \\
$d+f$  & $*$  & $0$ &  $*$  &  $0$  &  $*$ \\
$0$  & $*$  & $0$ &  $*$  &  $b$  &  $*$ \\
$*$  & $*$  & $0$ &  $*$  &  $b$  &  $0$ \\
$d$  & $*$  & $0$ &  $*$  &  $0$  &  $0$ \\
%$0$  & $*$  & $0$ &  $*$  &  $b$  &  $0$ \\
\hline
$*$  & $*$  & $*$ &  $0$  &  $a+b$  &  $a+c$ \\
$*$  & $*$  & $*$ &  $0$  &  $b$  &  $c$ \\
$*$  & $*$  & $*$ &  $0$  &  $0$  &  $a+c$ \\
$*$  & $*$  & $*$ &  $0$  &  $a+b$  &  $0$ \\
\hline
$0$  & $*$  & $*$ &  $*$  &  $b$  &  $c$ \\
%$*$  & $*$  & $*$ &  $a$  &  $0$  &  $c$ \\
%$*$  & $*$  & $*$ &  $a$  &  $b$  &  $0$ \\
$*$  & $*$  & $*$ &  $a$  &  $b$  &  $c$ \\
%$0$  & $*$  & $*$ &  $*$  &  $b$  &  $0$ \\
%$0$  & $*$  & $*$ &  $*$  &  $0$  &  $c$ \\
\hline
\end{tabular}
\end{table}
\end{center}
     
\bc{corollary3} For non-equioriented quiver $A_3$, let $V$ be a representation for which all indecomposables occur as summands of $V$ with non-zero multiplicities. The orbit closure $\overline{O_V}$ is Gorenstein iff the Coxeter orbits ($\tau$-orbits of the Auslander-Reiten quiver) are constant. 
\ec
\bpr
Sufficiency follows from Proposition \ref{Prop6}. Necessity follows from Case $7$.
\qed 
\newpage


